Introduction to speech recognition

This document contains lectures and practical experimentations using Matlab and implementing a system which is actually correctly classifying three words (one, two and three) with the help of a very small database. To achieve this performance, it uses speech modeling specificities, powerful computer algorithms (dynamic time warping and Dijktra's algorithm) and machine learning (nearest neighbor). This document introduces also some machine learning evaluation metrics.

==> annexe_son.tex <==


\appendix 

\chapter{Onde sonore stationnaire à une dimension}
\label{app:onde_stationnaire_1D}

L'application~\footnote{Cette annexe est inspirée de~\cite{DIsrael10ch5}} 
du principe fondamental de la dynamique et de la thermodynamique des fluides 
permettent d'écrire 
\beqn
\frac{1}{c^2}\frac{\partial^2 p(x,t)}{\partial t^2}-\frac{\partial^2 p(x,t)}{\partial x^2}=0
\eeqn
où $c$ est la vitesse du son. 

Les solutions de cette équation différentielle sont de la forme 
\beqn
p(x,t)=p_0+f_1(t-\frac{x}{c})+f_2(t+\frac{x}{c})
\eeqn

On considère une onde avec une seule fréquence $f_0$.
L'équation~(\ref{eq:p_onde_freq1}) définie page~\pageref{eq:p_onde_freq1} est recopiée ici. 
\beqns%\label{eq:p_onde_freq1}
p(x,t)=P_0+\Delta P_1\cos\left [2\pi f_0\left(t-\frac{x}{c}\right )+\varphi-\psi\right]
+\Delta P_2\cos\left[2\pi f_0\left (t+\frac{x}{c}\right )+\varphi+\psi\right]
\eeqns 

On considère ici un tuyau fermé de longueur L. 
On suppose $x=0$ à son extrêmité gauche et $x=L$ à son extrêmité droite. 
Il n'y a pas de déplacement de l'air là où le tube est fermé et cela se traduit par 
\beqn
\left .\frac{\partial p}{\partial x}\right |_{x=0}=0\quad \mbox{et}\quad 
\left .\frac{\partial p}{\partial x}\right |_{x=L}=0
\eeqn
Le calcul de ces expressions à partir de $p(x,t)$ 
aboutit à 
\beqn
\left .\frac{\partial p}{\partial x}\right |_{x=0}=
\frac{2\pi  f_0}{c}\Delta P_1\sin\left [2\pi f_0\left(t-\frac{0}{c}\right )+\varphi-\psi\right]
-\frac{2\pi f_0}{c}\Delta P_2\sin\left [2\pi f_0\left(t+\frac{0}{c}\right )+\varphi+\psi\right]
\eeqn
Le fait que cette expression est nulle montre que $\Delta P_1=\Delta P_2$ qui est noté $\Delta P$ et 
que $\psi=0$. 
\beqn
\left .\frac{\partial p}{\partial x}\right |_{x=L}=
\frac{2\pi f_0}{c}\Delta P\sin\left [2\pi f_0\left(t-\frac{L}{c}\right )+\varphi\right]
-\frac{2\pi f_0}{c}\Delta P\sin\left [2\pi f_0\left(t+\frac{L}{c}\right )+\varphi\right]
\eeqn
Une relation trigonométrique permet d'écrire 
\beqn
\cos(a+b)-\cos(a-b)=-2\sin(a)\sin(b)
\eeqn



Une  relation trigonométrique similaire montre que 
\beqn
\sin(a+b)-\sin(a-b)=2\sin(b)\cos(a)
\eeqn
Aussi 
\beqn
\left .\frac{\partial p}{\partial x}\right |_{x=L}=
-\frac{4\pi f_0}{c}\Delta P
\cos\left [2\pi f_0 t+\varphi\right]
\sin\left (\frac{2\pi f_0L}{c}\right )
\eeqn
Cette expression est bien nulle si et seulement si 
\beqn
\sin\left (\frac{2\pi f_0L}{c}\right )=0
\eeqn
Ce qui est vrai lorsque 
\beqn
f_0=k\frac{c}{L}
\eeqn
\underline{Plus la longueur augmente plus la fréquence de base diminue. }


\bibliographystyle{plain}
%\bibliographystyle{plain}
%\bibliography{L:/t1/TNS/TNS/BIBLIO/biblio}
\include{poly_son.bbl}
%\bibliography{biblio/bibtex_son}


==> sedRYbD7V <==

\newcommand{\msm}{$\mbox{m}.\mbox{s}^{-1}$}
\newcommand{\de}{{({\mbox{\small de}})}}
\newcommand{\moy}{{({ \mbox{\small moy})}}}
\newcommand{\der}{{({ \mbox{\small fin}})}}
\newcommand{\ce}{{({ \mbox{\small ce}})}}
\newcommand{\PMCT}{{\mbox{PMCT}}}
\newcommand{\arr}[1]{\rotatebox[origin=c]{#1}{$\xrightarrow{\hspace{1cm}}$}}
\newcommand{\fr}[1]{\framebox{#1}}
\newcommand{\bz}{{\mathbf z}}
\newcommand{\deux}{{\text{\tiny{|2}}}}     


\DeclareMathOperator{\OA}{OA}

\title{
Introduction à la reconnaissance de la parole  \\
}
\author{{\small Gabriel Dauphin}}


\begin{document}




%\pagenumbering{Alph}

%\pagenumbering{arabic}

\maketitle
\tableofcontents


\chapter*{Introduction}

Ce cours présente un ensemble de techniques qui sont utilisées en travaux pratiques 
pour distinguer les sons correspondant aux mots {\tt un}, {\tt deux} et {\tt trois}. 
Ces techniques utilisent la notion de description temps-fréquence qui est implicite dans la 
décomposition d'un son en trames, explicite dans la notion de {\tt spectrogramme} et qui est 
utilisée dans les différents descripteurs présentés dans le chapitre~\ref{ch:desc}.
Le chapitre~\ref{ch:traitement_son} a pour objectif de décrire la façon des sons sont représentées, cela amène 
à décrire brièvement les organes humains de la perception et le prétraitement qui est appliqué 
aux données associées aux sons. 
Le chapitre~\ref{ch:classification_par_descripteurs} a pour objectif de présenter la classification, à savoir son objectif, la façon dont on l'évalue et 
la manière dont elle utilise des valeurs calculées pour chaque son  que l'on appelle ici {\em descripteur}. 
Le chapitre~\ref{ch:desc} présente différentes techniques permettant de calculer les valeurs de descripteurs à partir des données 
associés aux sons. Cela amène à décrire brièvement les organes humains de la génération d'un son car cela explique 
l'intérêt porté à l'utilisation d'une description fréquentielle de portions de signaux temporels. 

En tant que document de cours, il a pour objectif de préciser les notions à connaître. Les notions 
à connaître le plus précisément sont la compréhension et la connaissance des {\em formules encadrées}, la compréhension 
des {\em graphiques et schémas} présentés et la connaissance et la signification des {\em termes techniques}. 





\chapter{Représentation d'un son}
\label{ch:traitement_son}

Pour décrire et discuter de la façon dont les sons sont représentées, la 
section~\ref{sec:questce_quun_son} discute de ce qu'est physiquement un son et donne 
une brève description des organes humains utilisées pour la perception d'un son. 
La section~\ref{sec:son_temps} rappelle comment le traitement numérique du signal permet 
de représenter un son.
La section~\ref{sec:N:son_trames} montre une façon un peu différente de représenter le son au moyens 
de {\em trames}, c'est-à-dire de petites portions du signal sonore. 
La section~\ref{sec:detection_silence} montre une façon simplifiée de détecter les phases de silence et de paroles, 
il se trouve que ceci était un des objectifs de ce cours. Cette détection est utilisée pour réaliser un 
prétraitement permettant d'améliorer la performance de la classification. 
La section~\ref{sec:implementation} donne quelques indications sur la façon dont les techniques proposées sont implémentées
dans les travaux pratiques qui illustre ce cours. 



\section{Qu'est-ce qu'un son~?}
\label{sec:questce_quun_son}


La section~\ref{ssec:model_physique} présente une description du son en tant qu'onde sonore se propageant 
dans l'air. 
La section~\ref{ssec:oreille} présente une très brève description du fonctionnement de l'oreille 
en tant qu'organe de perception des sons. 
La section~\ref{ssec:audibilite} présente des courbes d'audibilité, c'est-à-dire les seuils hauts et bas 
de perception du son. 


\subsection{Modélisation physique}
\label{ssec:model_physique}
Un son est généralement décrit comme plus ou moins aigu ou plus ou moins fort. Nous allons voir
que la première notion correspond à une fréquence et la deuxième à un niveau sonore. 

Le son est une variation de la pression de l'air.~\footnote{Un son peut aussi se propager à travers d'autres matériaux et dans ce cas 
c'est le matériau traversé qui se met à vibrer, en revanche le son ne peut pas se propager à travers le vide.}
Cette variation se propage sous la forme d'une onde. Une modélisation sphérique de cette onde est décrite par 
\beqn\label{eq:propag_onde}
P(r,t)=P_0+\frac{1}{r}\left [g_1(t-\frac{r}{c})+g_2(t+\frac{r}{c})\right ]
\eeqn
\begin{itemize}
\item $P_0$ est la pression atmosphérique moyenne. L'unité dans laquelle elle s'exprime est le Pa (Pascal). La pression de l'air est environ $10^5$Pa.
\item $r$ est la distance en mètres (m) entre le point où on mesure la pression et la  source de ce signal sonore. 
\item $t$ est l'instant en secondes~(s) pour lequel on mesure la pression $P(r,t)$. 
\item $c$ est la vitesse ($\mbox{m}.\mbox{s}^{-1}$) de propagation du son à travers l'air. C'est environ de $340$\msm. 
\item $g_1$ et $g_2$ peuvent a priori être des fonctions quelconques. Pour modéliser la propagation d'un signal sonore, on 
considère $g_2=0$ et pour un son stationnaire par exemple dans une caisse de résonnance, $g_1$ et $g_2$ sont similaires. 
\end{itemize}

Pour modéliser une note de musique qui dure un temps infini, on utilise 
\beqn
\boxed{
g_1(\tau)=\cos(2\pi f_0\tau)
}
\eeqn
Cette note est caractérisée par sa fréquence $f_0$ en Hz. 
En effet, avec cette modélisation on observe que $P(r,t+\frac{1}{f_0})=P(r,t)$, 
c'est-à-dire qu'en chaque point la pression évolue dans le temps avec une périodicité de $\frac{1}{f_0}$. 
{\small 
\beqns
P(r,t+\frac{1}{f_0})=P_0+\frac{1}{r}\cos(2\pi f_0(t+\frac{1}{f_0}-\frac{r}{c}))
=P_0+\frac{1}{r}\cos(2\pi f_0(t-\frac{r}{c}))=P(r,t)
\eeqns
}
Et $f_0$ est reliée à une longueur d'onde notée $\lambda_0$ mesurée en mètres.
\beqn\label{eq:long_onde}
\boxed{
\lambda =\frac{c}{f_0}
}
\eeqn
Ceci traduit une évolution quasi-périodique du signal dans l'espace $P(r+\lambda,t)\approx P(r,t)$. 
{\small 
\beqns
P(r+\lambda,t)=P_0+\frac{1}{r+\lambda}\cos(2\pi f_0(t-\frac{r}{c}-\frac{\lambda}{c}))
=P_0+\frac{1}{r+\lambda}\cos(2\pi f_0(t-\frac{r}{c}))\approx P(r,t)
\eeqns
}
\`A l'oreille, ce son apparaît comme une note de musique. Il s'agit d'un La lorsque $f_0=440$Hz. 
Cette fréquence est donc liée au caractère plus ou moins aigu du son. 

L'intensité sonore d'un son correspond au produit de la surpression par la vitesse. Dans le cadre de ce cours, 
on considère qu'il s'agit du carré de la partie variable de la pression. 
\beqns
I=\left (P(r,t)-P_0\right )^2
\eeqns
Cette intensité sonore est en Watt par mètres carrés ($\mbox{W}.\mbox{m}^{-2}$).
Dans le cadre de ce cours, on attache de l'importance au fait que cette intensité sonore est proportionnelle à $\frac{1}{r^2}$. 
\beqn
\boxed{
I=\frac{I_e}{r^2}
}
\eeqn
$I_e$ étant une quantité inconnue à estimer. 
Aussi lorsqu'on s'éloigne de la source en doublant la distance, l'intensité sonore est divisée par $4$. 

On appelle niveau sonore, le fait d'utiliser une échelle en décibel pour mesurer l'intensité sonore. 
\beqn\label{eq:N:niveau_sonore}
\boxed{
L=10\log_{10}\left (\frac{I}{I_0}\right )
}
\eeqn
où $I_0$ est une intensité sonore de référence. On peut remarquer que dans l'équation~(\ref{eq:N:niveau_sonore}), 
l'échelle en décibel n'est pas calculé avec un facteur multiplicatif de $20$ mais de $10$, parce que l'intensité sonore est 
déjà un terme carré. Et en effet lorsqu'on s'éloigne d'une source sonore en multipliant par deux la distance, 
le niveau sonore est diminué de $10\log_{10}(4)=6$dB.~\footnote{C'est en effet la même diminution que pour 
le rapport signal sur bruit, si on divisait par deux le bruit sans modifier le signal source.}

\subsection{Fonctionnement schématique de l'oreille}
\label{ssec:oreille}

\begin{figure}
\begin{center}
\begin{tabular}{c}
\includegraphics[width=0.5\linewidth]{oreille.png}
\end{tabular}
\end{center}
\caption{Schéma détaillé de l'oreille.}
\label{fig:N:oreille}
\end{figure}
	

La figure~\ref{fig:N:oreille} (extraite d'une publication) 
représente un schéma détaillé de l'oreille. Schématiquement, le son s'introduit dans le conduit auditif, 
fait vibrer le tympan qui actionne le marteau, l'enclume et l'étrier qui à son tour fait vibrer le liquide présent dans la cochlée. 
Cette cochlée est tapissée de cellules ciliées qui transmettent les vibrations vers des nerfs auditifs. Les cellules au début 
de la cochlée sont sensibles aux sons aigus tandis que celles en fin de cochlée sont sensibles aux sons graves. 

\subsection{Courbes d'audibilité humaine}
\label{ssec:audibilite}

\begin{figure}
\begin{center}
\begin{tabular}{c}
\includegraphics[width=0.5\linewidth]{courbe_audibilite.png}
\end{tabular}
\end{center}
\caption{Courbe d'audibilité humaine.}
\label{fig:N:courbe_audibilite}
\end{figure}
	
Dans la figure~\ref{fig:N:courbe_audibilite} (extraite d'une publication), l'échelle des ordonnées est le niveau sonore d'un son écouté. L'échelle 
des abscisses est une échelle de fréquences (Hz) mais avec une distribution logarithmique. \`A gauche ce sont les infrasons qui
correspondent aux sons qu'on ne peut entendre parce que leur fréquence est trop basse. \`A droite ce sont les ultrasons 
qu'on ne peut pas non plus entendre parce que leur fréquence est trop haute. Entre ces deux fréquences, il y a deux courbes, 
si le niveau sonore d'un son est supérieur à la limite donnée par la courbe inférieure alors on peut l'entendre et s'il 
est supérieur à la limite donnée par la courbe supérieure alors ce son peut abîmer l'oreille. 
Ces courbes sont obtenues en expérimentant sur un grand nombre de patients, elles indiquent un sensibilité moyenne, mais 
il y a en réalité des différences importantes d'un individu à un autre. 
Ces courbes nous amènent à affirmer qu'une assez grande partie de l'information sonore est obtenue en ne considérant 
que les fréquences inférieures à $4$kHz et qu'a priori la totalité de l'information sonore est obtenue en 
ne considérant que les fréquences inférieures à $20$kHz. 


\section{Représentation temporelle d'un son}
\label{sec:son_temps}


\begin{figure}
\begin{center}
\begin{tabular}{c}
\includegraphics[width=0.5\linewidth]{son_temps.png}
\end{tabular}
\end{center}
\caption{Représentation temporelle du signal sonore.}
\label{fig:N:son_temps}
\end{figure}
	
	
En tant qu'onde sonore, un son est un signal temps continu à valeurs continus. Mais lorsqu'il est 
converti en signal électrique avec un capteur acoustique appelé microphone puis converti en signal numérique avec 
échantillonnage et quantification, le signal devient temps discret. 
Du fait du critère de Shannon-Nyquist, la fréquence d'échantillonnage $f_e$ est entre $40$kHz et $50$kHz (en général 
$44.1$kHz mais, 
elle peut parfois être de $8$kHz. Le signal est souvent quantifié sur $8$ bits, mais cela peut être $10$ ou $12$ bits. 
Le signal échantillonné est noté $x_n$, chaque indique $n$ correspondant à un instant $t_n=nT_e$ où $T_e=\frac{1}{f_e}$.
La figure~\ref{fig:N:son_temps} (extraite d'une publication), indique l'évolution au cours du temps de l'intensité sonore. 
En ordonnée, il n'y a pas d'unité, c'est a priori une fraction de la valeur maximale. Mais le carré du signal est proportionnel à l'intensité sonore. 
Le signal représenté est celui obtenu en enregistrant la phrase {\em Le metteur en scène termine le scénario.} 



On appelle {\em durée} du signal, le temps qui s'écoule entre le début 
du signal sonore et la fin. Cette durée est égale à $NT_e$ où ici $N$ est 
le nombre d'échantillons~\footnote{\'Etant donné 
la valeur de $f_e$, il est tout à fait satisfaisant d'approcher cette durée 
à un multiple de $T_e$.} représenté sur la figure~\ref{fig:N:son_temps}. 
\'Etant donné la valeur élevée de $f_e$, on a en fait un très grand nombre d'échantillons, 
bien plus qu'il n'est possible de distinguer à l'oeil en observant la figure. L'allure générale permet aussi de distinguer les
 moments où il y a du silence, des moments où 
il y a un signal sonore important~: le silence correspond à des valeurs très faibles en valeur absolues et le signal sonore important correspond à des 
valeurs importantes du signal. 
Comme chaque intervalle de temps dans le graphe correspond aussi à un intervalle de 
temps durant lequel un son est prononcé, il est possible de faire correspondre chaque syllabe à un morceau du signal. On peut ainsi visualiser pour certaines sons des particularités, le premier {\em t} et les deux {\em s} correspondent à des parties très foncées du graphe. 

Bref, cette représentation temporelle du signal suggère l'étude séparée de chaque morceau de signal correspondant à un son ou à une syllabe. Mais comme on ne connaît 
pas a priori quand commence et quand finit le son ou la syllabe, la 
section~\ref{sec:N:son_trames} montre que l'on découpe le signal en une succession
de trames. 

Les notations utilisées pour décrire l'ensemble du signal sont les suivantes. 
\begin{itemize}
\item $T$ durée du signal en secondes.
\item $N$ nombre total d'échantillons.
\item $t_n=nT_e$ échelle de temps du signal pour $n\in\{0\ldots N-1\}$. 
\end{itemize}
On a la relation entre durée du signal et période d'échantillonnage. 
\beqn
\boxed{
T=NT_e
}
\eeqn
On a aussi l'échantillonnage du signal.
\beqn
\boxed{
x_n=x(t_n)
}
\eeqn


Pour illustrer des notions traitement du signal, on s'interroge ici sur la façon 
de rendre un son plus grave au moyen d'un traitement numérique du vecteur $x_n$. 
\begin{itemize}
\item En diminuant $f_e$, le son est plus grave. 
Mais sa durée est aussi diminuée d'autant puisqu'elle est égale à $\frac{N}{f_e}$. 
\item Si on effectue un sur-échantillonnage tout en conservant la fréquence 
d'échantillonnage alors le son devient plus grave mais sa durée est 
augmentée d'autant. 
\item Si on effectue une modulation, c'est-à-dire qu'on multiplie le graphe
par une sinusoïde d'une certaine fréquence alors on déplace effectivement 
le son à la fois en le rendant plus aigu et plus grave. Si ce son a un spectre
très étroit alors il est possible de supprimer la composante aigüe ou la composante grave. Et la durée est alors inchangée.  
\end{itemize}


\section{Représentation du signal sonore en une succession de trames}
\label{sec:N:son_trames}

\subsection{Découpage en trames sans chevauchement}

\begin{figure}
\begin{center}
\begin{tabular}{c}
\includegraphics[width=0.8\linewidth]{son_trames_simples.png}
\end{tabular}
\end{center}
\caption{Découpage d'une sinusoïde en trames qui ne se chevauchent pas.}
\label{fig:N:son_trames_simples}
\end{figure}
	
La figure~\ref{fig:N:son_trames_simples} donne quatre représentation 
d'un même signal défini par 
\beqns
x_n=\sin(20\pi nT_e)
\eeqns
C'est le signal représenté en haut à gauche de cette figure où sur une seconde, il
y $10$ périodes de la sinusoïde qui sont répétées et où donc, la fréquence de la 
sinusoïde est de $10$Hz et la période $T=0.1$s. L'échelle des ordonnées est 
une fraction de l'amplitude maximale. L'échelle des abscisses est la seconde. 

Dans cet exemple, on découpe le signal d'une seconde en $10$ trames chacune 
dure ici $0.1$s. La figure en haut à droite représente chaque trame avec une couleur 
différente~: bleu pour la première trame, vert pour la deuxième, rouge pour la troisième, cyan pour la quatrième, violet pour la cinquième, etc...

Le graphe en bas à gauche est une autre représentation de ces trames. L'axe pointant vers la droite est le temps écoulé depuis le début de chaque trame. 
L'axe pointant vers la gauche et commençant à zéro au milieu indique le numéro 
de la trame considérée. L'axe vers le haut indique la valeur du signal pour la trame considérée à l'instant de la trame considérée. La valeur zéro est ici à mi-hauteur. Ici la couleur ne distingue plus les trames entre elles, elle dépend de la valeur prise par le signal. Dans cet exemple le signal est identique sur chaque trame, c'est pour cela qu'on retrouve exactement le même signal sur chaque courbe. 

La courbe en noir du graphe en bas à droite est la même que le graphe en haut à gauche, il s'agit du signal $x_n$ représenté en fonction du temps. Sur ce graphe, il y a en plus des traits horizontaux de couleurs et de hauteurs différentes
qui permettent d'identifier chaque trame. Ce sont ces traits qui permettent de lire 
les instants associés au début et à la fin de chaque trame en trouvant l'abscisse 
du début et de la fin du trait horizontal. 

\subsection{Notations pour définir les trames}

On utilise ici les notations suivantes. Ces notations ne sont pas 
universelles, il est donc nécessaire de les redéfinir quand on les utilise. 
\begin{itemize}
\item $K$ désigne le nombre de trames. 
\item $T_K$ est la durée d'une trame. 
\item $N_K$ est le nombre d'échantillons dans une trame, il est identique pour toutes les trames d'un même son.
\item $k\in \{0\ldots K-1\}$ est un indice qui identifie la trame. 
\item $t_k^\de$ instant associé au premier échantillon de la trame $k$.
\item $t_k^\der$ instant associé au dernier échantillon de la trame $k$. 
\item $t_k^\ce$ instant associé au centre de la trame $k$. 
\item $t_{k,n}$ échelle de temps associée à la trame $k$ donnant 
les instants associées aux échantillons $n=0$ jusqu'à $n=N_K-1$. 
\end{itemize}

Du fait qu'il n'y a pas de chevauchement, on a
\beqn\label{eq:N:T_K}
\boxed{
T_K=\frac{T}{K}\mbox{ et }N_K=\frac{N}{K}
}
\eeqn

D'une façon générale, le début, le centre et la fin d'une trame 
$k$
sont définies par
\beqn\label{eq:N:t_k_de}
\boxed{
\mbox{Pour }k\in\{0\ldots K-1\},\quad\left \{
\begin{array}{l}
t_k^\de=k\frac{T}{K}\\[0.2cm]
 t_k^\der=t_k^\de+T_K-T_e\\[0.2cm]
t_k^\ce=\frac{1}{2}\left (t_k^\de+t_k^\der\right )
\end{array}
\right. 
}\eeqn

Avec ces définitions et pour une trame $k$, on peut définir une échelle de temps et déterminer les valeurs du signal
\beqn\label{eq:N:ech_temps_trame}
\boxed{
\begin{array}{c}
\mbox{Pour }k\in\{0\ldots\}\mbox{ et }n\in \{0\ldots N_K-1\}\\[0.5cm]
t_{k,n}=t_k^\de+nT_e \mbox{ et }x_{k,n}=x(t_{k,n})=x\left[\frac{t_{k,n}}{T_e}\right ]
\end{array}
}
\eeqn
Dans la dernière expression en bas à droite de l'équation~(\ref{eq:N:ech_temps_trame}), l'expression entre crochet est un indice 
\beqns
n'=\frac{t_{k,n}}{T_e}=k\frac{N}{K}+n
\eeqns
et cet indice est utilisé pour retrouver dans le signal $x_n$ la valeur recherchée 
$x_{k,n}=x_{n'}$. 


\subsection{Découpage en trames avec chevauchement}

\begin{figure}
\begin{center}
\begin{tabular}{c}
\includegraphics[width=0.8\linewidth]{son_trames_chevauchement.png}
\end{tabular}
\end{center}
\caption{Découpage d'une sinusoïde en trames qui se chevauchent.}
\label{fig:N:son_trames_chevauchement}
\end{figure}


\`Etant donné un nombre total d'échantillons $N$, un nombre de trames $K$ et 
du choix de chevauchement utilisé, on a les deux propriétés suivantes. 
\begin{itemize}
\item Les instants de débuts des trames ne sont pas modifiées.
\beqn
\boxed{
t_k^\de=k\frac{T}{K}
}
\eeqn
\item La longueur des trames est augmenté d'un facteur $\frac{1}{1-\alpha}$. 
\beqn\label{eq:N:T_K_alpha}
\boxed{
T_K=\frac{T}{K}\frac{1}{1-\alpha}\mbox{ et }N_K=\frac{N}{K}\frac{1}{1-\alpha}
}
\eeqn
\item Hormis la première trame, toutes les trames partagent avec la précédente
$\alpha N_K$ échantillons. Et hormis la dernière trame, toutes les trames partagent avec la suivante $\alpha N_K$ échantillons. 
\end{itemize}


La dernière affirmation se calcule ainsi pour $k\in\{0\ldots K-1\}$
\beqns
t_k^\der-t_{k+1}^\de+T_e=\left (k\frac{T}{K}+\frac{T}{K}\frac{1}{1-\alpha}-T_e\right ) -(k+1)\frac{T}{K}+T_e=\frac{T}{K}\left (\frac{1}{1-\alpha}-1\right )
=\alpha T_K
\eeqns


Ainsi les équations (\ref{eq:N:t_k_de}) et (\ref{eq:N:ech_temps_trame})
ne sont pas modifiées quand on met un chevauchement. En revanche l'équation~(\ref{eq:N:T_K})
est remplacée par l'équation~(\ref{eq:N:T_K_alpha}).

Lors de l'implémentation, ces formules ont été un peu modifiées pour tenir 
compte de ce que le découpage en trames ne tombe pas exactement sur un échantillon 
et qu'il faut donc commencer à partir de l'échantillon le plus proche. 

\section{Signaux sonores et silences}
\label{sec:detection_silence}
\subsection{Puissance moyenne à court terme}
\label{ssec:PMCT}


\begin{figure}
\begin{center}
\begin{tabular}{c}
\includegraphics[width=0.8\linewidth]{son_puissance.png}
\end{tabular}
\end{center}
\caption{Signal temps discret représentant un signal sonore commençant et terminant par un silence.}
\label{fig:N:son_puissance}
\end{figure}

En traitement du signal, on définit une puissance moyenne qui évolue dans le temps
qui est appelée puissance moyenne à court terme. 
Cela se fait en introduisant une fenêtre notée $w_T$ qui est un signal temps 
continu de durée $T$ centré en zéro. 
La notion de fenêtre a déjà été présentée lors du cours sur la 
synthèse des filtres numérique à réponse impulsionnelle finie avec notamment la fenêtre rectangulaire et triangulaire. 
\`A temps continu, la fenêtre rectangulaire de largeur $T$ est ainsi définie.
\beqns
w_T(\tau)=\1_{\left [-\frac{T}{2},\frac{T}{2}\right]}(\tau)
\eeqns
La fenêtre triangulaire de largeur $T$ est ainsi définie.
\beqns
w'_T(\tau)=\left (1-\frac{2t}{T}\right)\1_{\left [-\frac{T}{2},\frac{T}{2}\right]}(\tau)
\eeqns
Ici la fenêtre est utilisée, non pour modifier une réponse impulsionnelle mais un signal, ici $x^2(t)$. L'action de la fenêtre 
porte sur l'intervalle de temps centré en $t$. Aussi elle est d'abord centrée en $t$ puis normalisée.
\beqns
w_T(\tau)\mapsto w_T(t-\tau)\mapsto \frac{1}{\int_\Rr w_T(t-\tau)\,d\tau}\,w_T(t-\tau)
\eeqns
Ainsi modifiée la fenêtre est ensuite multipliée par $x^2(\tau)$
\beqns
x^2(\tau)\mapsto x^2(\tau)\frac{1}{\int_\Rr w_T(t-\tau)\,d\tau}\,w_T(t-\tau)
\eeqns

Cette puissance moyenne à court terme, notée $\sm{PMCT}$~\footnote{{\tt PMCT}
est défini dans \cite{Camastra07} p.~41-42.}~\footnote{Une interprétation en terme d'énergie
existe dans page~3, section~2.1 dans~\cite{Peeters04}.}
 est 
\beqn\label{eq:PMCT_TC}
P(t)=\frac{{\int_\Rr {x^2(\tau)w_T(t-\tau)\,d\tau }}}{{\int_\Rr w_T(\tau)\,d\tau}}
\eeqn
Avec une fenêtre rectangulaire, $P(t)$ devient 
\beqn\label{eq:PMCT_TC_rect}
\boxed{
P(t)=\frac{1}{T}{\int_{t-\frac{T}{2}}^{t-\frac{T}{2}} x^2(\tau)\,d\tau}
}
\eeqn


Ici le découpage en trame du signal se prête justement à un calcul très similaire.
\begin{itemize}
\item $T$ est remplacée par la longueur de la trame $T_K$ qui compte $N_K$ échantillons. 
\item $t$ est remplacée par $t_k^\ce$, le milieu de la trame $k$ qui se trouve à peu près à l'échantillon $\frac{N_K}{2}$ de 
la trame $k$. 
\end{itemize} 
 Cela permet ainsi d'approcher la  discrétisation de l'équation~(\ref{eq:PMCT_TC}).
\beqn
\PMCT_k=\frac{{\sum_{n=0}^{N_K-1} x_k^2[n]w_{N_K}[n-\frac{N_K}{2}]}}{{\sum_{n=0}^{N_K-1} w_{N_K}[n-\frac{N_K}{2}]}}
\eeqn
où $w_{N_K}[n]$ est une fenêtre de support $\{-\frac{N_K}{2}\ldots \frac{N_K}{2}\}$ {\bf mais} avec des indices allant de $0$ à $N_K-1$.  

Avec une fenêtre rectangulaire, 
\beqn
\boxed{
\PMCT_k=\frac{1}{N_K}
{\sum_{n=0}^{N_K-1} x_k^2[n]}
}
\eeqn


\subsection{Détection du début et de la fin d'un signal sonore.}
\label{ssec:det_deb_fin_son}

La figure~\ref{fig:N:son_puissance} montre un exemple de signal sonore commençant et terminant par un silence. 
On souhaite dans cet exemple retrouver l'instant à partir duquel le signal sonore commence et l'instant auquel ce
 signal sonore s'arrête. 


On se donne un seuil, il est ici fixé à $10\%$ de la valeur maximale.
\beqn\label{eq:seuil}
\boxed{
s_e=\frac{1}{10}\max_k({\PMCT_k})
}
\eeqn
Ce seuil est utilisé pour déterminer deux numéros de trames~: $k^\de$ la première trame pour laquelle la puissance $\PMCT_k$ est supérieure 
$s_e$ et $k^\der$ la dernière  pour laquelle ceci est vrai. 
\beqn
\boxed{
k^{\de}=\underset{k}{\min}\,\{k|\,\PMCT_k>s_e\}
\mbox{ et }
k^{\der}=\underset{k}{\max}\,\{k|\,\PMCT_k>s_e\}
}
\eeqn
Les instants $t^\de$ et $t^\der$ associés au début et à la fin du signal sonore sont les centres des trames $k^\de$ et $k^\der$. 
\beqn
\boxed{
\left\{\begin{array}{l}
t^{\de}=t_{k}^{\ce}\mbox{ avec }k=k^{\de}\\[0.3cm]
t^{\der}=t_k^{\ce}\mbox{ avec }k=k^{\der}
\end{array}
\right . 
}
\eeqn
où $t_k^{\ce}$ désigne l'instant associé au centre de la trame $k$. 

\subsection{Normalisation d'un signal sonore}

La normalisation du signal a pour but de rendre comparable 
un son qui serait prononcé de façon forte et un son prononcé à voix plus basse. 
Cette normalisation consiste à imposer que la puissance moyenne soit fixe et en l'occurrence égale à $1$, mais 
cette étape se fait après avoir retiré les silences du signal.~\footnote{Si on effectuait cette normalisation du 
signal avant de retirer les silences, un son avec beaucoup de silences 
que l'on aurait normalisé  avec ses silences, aurait une 
puissance moyenne plus forte, une fois retirés les silences.}


Pour comparer les signaux, il est souhaitable que les signaux soient comparable en terme de puissance moyenne. Cette moyenne étant calculée sans considérer les silences. 
Pour obtenir que les signaux soient comparés, on effectue une {\em normalisation}, c'est-à-dire qu'on chacun des signaux par une valeur appropriée. 
Cette valeur est déterminée avec les étapes suivantes. 
\begin{itemize}
\item On utilise la technique de détection du début et de fin du signal sonore présentée en section~\ref{ssec:det_deb_fin_son}. 
\item On calcule la puissance moyenne en ne considérant que les trames qui se situent entre la première et la dernière des trames associées au signal sonore. 
On note $\bb{K}$ l'ensemble des trames où le son est plus fort que le seuil fixé par l'équation~(\ref{eq:seuil})
et $|\bb{K}|$ le nombre de ces trames. 
\beqns
\boxed{
P_\moy=\frac{1}{|\bb{K}|}{\sum\limits_{k\in \bb{K}} \sm{PMCT}_k}
}
\eeqns
\item La normalisation consiste à multiplier le signal par $\frac{1}{\sqrt{P_\moy}}$. 
\beqn
\boxed{
x_n\mapsto \frac{1}{\sqrt{P_\moy}} x_n
}
\eeqn
\end{itemize}


\section{Indications sur l'implémentation proposée}
\label{sec:implementation}

\begin{figure}
\begin{center}
\begin{tabular}{c}
\includegraphics[width=0.6\linewidth]{projet_son1.png}
\end{tabular}
\end{center}
\caption{Organisation des données dans l'implémentation}
\label{fig:N:projet_son1}
\end{figure}

Dans la simulation proposée, le répertoire principal est subdivisé en {\tt prg} contenant les programmes Matlab (fichiers {\tt .m} ou {\tt .p}) et {\tt donnee} qui contient 
les fichiers audio répartis en trois répertoires  {\tt un},  {\tt deux } et {\tt trois}. 
Cette organisation est schématisée sur la figure~\ref{fig:N:projet_son1}.


\chapter{Obtenir une classification grâce à des descripteurs}
\label{ch:classification_par_descripteurs}

L'objectif au cours de la séance de TP correspondante est de classer les sons à partir de descripteurs. Un descripteur peut 
soit être une valeur pour l'ensemble du signal, soit un ensemble de valeurs, une pour chaque trame.
On suppose dans cette partie qu'on dispose d'un certain nombre de descripteurs qui nous donnent des valeurs, une valeur par trame. 
La classification des sons est alors exposée en trois parties. 
La section~\ref{sec:distance_entre_sons} permet à partir de descripteurs d'évaluer numériquement 
une similarité entre deux sons. En fait on parle plutôt de distance entre sons, la distance correspondant ici à un défaut de similarité. 
une distance entre deux sons. 
La section~\ref{sec:knn} permet à partir de distances entre sons de prédire l'identité d'un son quelconque, 
c'est-à-dire s'il ressemble plus à un son de type {\tt un}, {\tt deux} ou {\tt trois}. 
Enfin la section~\ref{sec:evaluation_classification} montre comment on évalue généralement un classifieur. 


%\fbox{\begin{minipage}{0.8\linewidth}
%\imp
%Des descripteurs sont disponibles en utilisant la fonction {\tt traitement}. 
%\end{minipage}}

\section{Calcul d'une distance entre deux sons}
\label{sec:distance_entre_sons}



\begin{figure}
\begin{center}
\begin{tabular}{c}
\begin{tikzpicture}
[node distance = 10mm,thick, main/.style = {draw, circle},
  rect/.style={draw,rectangle,fill=green!50},rect_y/.style={draw,rectangle},
  minimum size=0mm]
	\node (H1) {};
	\node (L1)[below of=H1] {};
	\node (L11) [below of=L1] {};
		\node (L12) [below of=L11] {};
		\node (L13) [below of=L12] {};
		\node (L14) [below of=L13] {};
	  \node (sons) [right of=L1] {sons}; 
		\node[rect_y] (xn) [below of=sons] {$x_a[n]$};   
		\node (xmn) [below of=xn] {};  
		\node[rect_y] (xpn) [below of=xmn] {$x_b[n]$};  
		\node (L2) [right of=sons] {};
	  \node (trames) [right of=L2] {trames}; 
		\node[rect_y] (xkn) [below of=trames] {$x_a[k,n]$};   
		\node (xmkn) [below of=xkn] {};  
		\node[rect_y] (xpkn) [below of=xmkn] {$x_b[k,n]$};  
		\node (L3) [right of=trames] {};
		\node (sans_silence) [right of=L3] {$\begin{array}{c}\mbox{sans le}\\ \mbox{silence}\end{array}$}; 
		\node[rect_y] (xkn1) [below of=sans_silence] {$x_a[k,n]$};   
		\node (xmkn1) [below of=xkn1] {};  
		\node[rect_y] (xpkn1) [below of=xmkn1] {$x_b[k,n]$};  
		\node (L4) [right of=sans_silence] {};
		\node (normalisation) [right of=L4] {$\begin{array}{c}\mbox{normali-}\\ \mbox{sation}\end{array}$}; 
		\node[rect_y] (xkn2) [below of=normalisation] {$x_a[k,n]$};   
		\node (xmkn2) [below of=xkn2] {};  
		\node[rect_y] (xpkn2) [below of=xmkn2] {$x_b[k,n]$};  
		\node (L5) [right of=normalisation] {};
		\node (H5) [above of=L5] {};
		\node (L51) [below of=L5] {};
		\node (L52) [below of=L51] {};
		\node (L53) [below of=L52] {};
		\node (L54) [below of=L53] {};
		\node (descripteur) [right of=L5] {$\begin{array}{c}\mbox{calcul des}\\ \mbox{descripteurs}\end{array}$}; 
		\node[rect_y] (zkj) [below of=descripteur] {$z_{a}^{(j)}[k]$};   
		\node (zmkj) [below of=zkj] {};  
		\node[rect_y] (zpkj) [below of=zmkj] {${z}_{b}^{(j)}[k]$};  		
		\node (L6) [right of=descripteur] {};
		\node (distance) [right of=L6] {$\begin{array}{c}\mbox{calcul de la}\\ \mbox{distance}\end{array}$}; 
		\node (L67l) [below of=distance] {}; 
		\node[rect_y] (d) [below of=L67l] {$d(x_a,x_b)$};   
		
		\begin{scope}[-latex]
\draw[thick,->,blue] (xn) to   (xkn);
\draw[thick,->,blue] (xkn) to   (xkn1);
\draw[thick,->,blue] (xkn1) to   (xkn2);
\draw[thick,->,green] (xkn2) to   (zkj);
\draw[thick,->,blue] (xpn) to   (xpkn);
\draw[thick,->,blue] (xpkn) to   (xpkn1);
\draw[thick,->,blue] (xpkn1) to   (xpkn2);
\draw[thick,->,green] (xpkn2) to   (zpkj);
\draw[thick,->,red] (zpkj) to   (d);
\draw[thick,->,red] (zkj) to   (d);
\draw[gray,dashed,-] (H1) to   (H5);
\draw[gray,dashed,-] (H5) to   (L54);
\draw[gray,dashed,-] (L14) to   (L54);
\draw[gray,dashed,-] (H1) to   (L14);
\end{scope}
\end{tikzpicture}
\end{tabular}
\end{center}
\caption{Schéma décrivant la mise en oeuvre du calcul de la distance entre deux sons noté $x$ et $x'$. 
La partie encadrée en pointillé est la préparation des signaux
transformant $x_a[n]$ et $x_b[n]$ en $x_a[k,n]$ et $x_b[k,n]$, $n$ étant dans $x_a[n]$ et $x_b[n]$ l'indice de l'échantillon pour  l'ensemble du son 
et pour $x_a[k,n]$ et $x_b[k,n]$, l'indice dans la trame $k$. La lettre $j$ désigne un type de descripteur et celui-ci est calculé pour les deux sons et pour chaque 
%trame $k$, les valeurs obtenues sont rangées dans $z_{k}^{(j)}$ et ${z'}_{k}^{(j)}$. 
$d(x_a,x_b)$ désigne la valeur de la distance entre les deux sons.  }
\label{fig:dist_sons}
\end{figure}
 %\beqns
%\begin{array}{c@{}c@{}c@{}c@{}c@{}c@{}c}
%\mbox{sons} &  & \mbox{trames} && \hspace{-1cm}\mbox{descripteurs}\hspace{-1cm} && \mbox{distance}\\[0.3cm]
%\fr{$x_n$} &\arr{0}& \fr{$x_{k,n}$}& \arr{0}& \fr{$z_{k,j}$}\\[-0.4cm]
%&& && &\arr{-30} \\[-0.3cm]
%&& && &  &\fr{d(x,x')}\\[-0.3cm]
%&& && &\arr{+30} \\[-0.4cm]
%\fr{$x'_n$} &\arr{0}& \fr{$x'_{k,n}$}& \arr{0}& \fr{$z'_{k,j}$}\\[0.3cm]
%\end{array}
%\eeqns


La figure~\ref{fig:dist_sons} schématise la façon de calculer une distance (i.e. une non-similarité) entre deux sons. 
La partie encadrée en pointillé figure la préparation des signaux avec les tâches suivantes. 

\begin{minipage}{0.95\linewidth}
\begin{itemize}
\item Chaque signal sonore est décrit avec $x_a[n]$ et $x_b[n]$ par un signal temps discret échantillonné à la même fréquence d'échantillonnage, mais 
pas forcément de même durée. 
\item Chaque signal est découpé en trames, de longueur et de chevauchement identique, le nombre de trames est a priori différent d'un signal à l'autre. 
\item Les trames silencieuses en début et fin de son sont retirées. 
\item Les valeurs des signaux au sein de chaque trames sont normalisées globalement au niveau du son, c'est-à-dire que si une trame est 
en moyenne deux fois plus forte qu'une autre trame du même son, elle reste deux fois plus forte après la normalisation. 
Par contre quand on compare deux sons, le fait de multiplier par deux toutes les valeurs d'un des deux sons, ne modifie pas la distance entre les 
deux sons. 
\end{itemize}
\end{minipage}

On rajoute les notations suivantes~: 

\begin{minipage}{0.95\linewidth}
\begin{itemize}
\item $x_a$ et~$x_b$ désignent les sons~$a$ et~$b$. 
\item $x_a[n]$ et~$x_b[n]$ désignent les~$N_a$ et~$N_b$ valeurs des signaux associés aux sons~$a$ et~$b$. 
\item $x_a[kn]$ et~$x_b[kn]$ désignent les~$N_k$ valeurs des sons $a$ et $b$ pour la trame~$k$, c'est l'équivalent pour le son~$a$ de ce qui était noté précédemment~$x_k[n]$. 
\item $J$ désigne le nombre total de descripteur. 
\item $j\in\{1\ldots J\}$ désigne un descripteur spécifique. $\PMCT$ est un exemple de descripteur, les autres seront décrits dans le 
chapitre~\ref{ch:desc}. 
\item ${z}_a^{(j)}[k]$ et~${z}_b^{(j)}[k]$  désigne la valeur du descripteur~$j$ pour la trame~$k$ et les sons~$a$ et~$b$. 
\end{itemize}
\end{minipage}

Les calculs figurés par les flèches vertes joignant $x_a[kn]$ et $x_b[kn]$ à  ${z}_a^{(j)}[k]$ et ${z}^{(j)}_b[k]$ correspondent aux 
calculs des valeurs des descripteurs, 
Les flèches rouges joignant  ${z}_{a}^{(j)}[k]$ et ${z}_{b}^{(j)}[k]$ à $d(x_a,x_b)$ figurent les calculs permettant d'évaluer la distance à partir 
des valeurs des descripteurs, trois techniques sont proposées dans cette section. 

\subsection{Les descripteurs par trames sont transformés en descripteurs par son}
\label{ssec:mu_sigma}
On rajoute ici un autre sens au mot descripteur. Précédemment, il s'agissait d'un descripteur par trame, ici il s'agit d'un descripteur 
pour l'ensemble d'un son. Ce descripteur est identifié par $j$ correspondant aux valeurs du descripteur par trame qui sont 
résumés dans une seule valeur. Ce descripteur est aussi identifié par la façon de faire ce résumé~: $\mu$ pour la moyenne, $\sigma$ 
pour l'écart-type, $\gamma_1$ et $\gamma_2$ pour les coefficients d'asymétrie et d'aplatissement.

Ces quatre descripteurs de sons sont calculés à partir des valeurs d'un descripteur obtenu pour chaque trame d'un son. 

\begin{minipage}{0.95\linewidth}
\begin{itemize}
\item La moyenne d'un descripteur $j$ est la moyenne des valeurs de $z_k^{(j)}$ pour chaque trame $k$. 
\beqn\label{eq:mu}
\boxed{
\mu^{(j)}=\frac{1}{K}{\sum_{k=0}^{K-1} z_k^{(j)}}
}
\eeqn
\item 
L'écart-type d'un descripteur $j$ est la racine carré de la moyenne des variances.
\beqn\label{eq:sigma}
\boxed{
\sigma^{(j)}=\sqrt{\frac{1}{K}{\sum_{k=1}^K \left (z_k^{(j)} -\mu^{(j)}\right)^2}}
}
\eeqn
\item Le coefficient d'asymétrie d'un descripteur $j$ est 
\beqn
\gamma_1^{(j)}=\frac{1}{(\sigma^{(j)})^3}{\frac{1}{K}{\sum_{k=1}^K \left (z_k^{(j)} -\mu^{(j)}\right)^3}}
\eeqn
\item Le coefficient d'aplatissement d'un descripteur $j$ est 
\beqn
\gamma_2^{(j)}=\frac{1}{(\sigma^{(j)})^4}{\frac{1}{K}{\sum_{k=1}^K \left (z_k^{(j)} -\mu^{(j)}\right)^4}}
\eeqn
\end{itemize}
 \end{minipage}

Ces quatre descripteur de sons permettent de définir différentes distances entre sons suivant ce qui est pris en compte. 
Par exemple en prenant en compte la moyenne et l'écart-type des descripteur $j\in\{1\ldots J\}$, on a la distance suivante~: 
\beqn
\boxed{
d(x_a,x_b)=\sqrt{{\sum_{j=1}^J \left( \mu_a^{(j)}-\mu_b^{(j)}\right )^2+\left( \sigma_a^{(j)}-\sigma_b^{(j)}\right )^2}}
}
\eeqn

\subsection{La distance entre deux sons est obtenue en comparant trame par trame, les valeurs des descripteurs.}
\label{ssec:dist_trames}

Les sons $a$ et $b$ n'ont pas a priori la même durée et donc pas le même nombre de trames. On note $\min(K_a,K_b)$ le nombre de trames du son 
le plus court. On définit la distance comme la moyenne des distances entre les descripteurs trame par trame. Cette distance est 
en fait la racine carré de la somme des carrés des différences. Chaque son est décrit par $J{\times}K_a$ et $J{\times}K_b$ valeurs, 
on arrive à la définition suivante. 
\beqn
\boxed{
d(x_a,x_b)=\sqrt{\frac{1}{\min(K_a,K_b)}
{\sum_{k=0}^{\min(K_a,K_b)-1}{\sum_{j=1}^J\left (z_a^{(j)}[k]-z_b^{(j)}[k]\right )^2}}}
}
\eeqn

Un important défaut de cette technique est qu'elle amène à considérer un son comme différent, lorsqu'il est prononcé avec une vitesse différente ou simplement une vitesse qui varie différemment. 

\subsection{La distance entre deux sons est obtenue en cherchant la déformation temporelle minimisant la différence entre les deux sons.}
\label{ssec:dist_def_temp}

\subsubsection{Notion de déformation temporelle dynamique }


\begin{figure}
\begin{center}
\begin{tabular}{cc}
\includegraphics[width=0.5\linewidth]{fig_def_temp1.png}
\includegraphics[width=0.5\linewidth]{fig_def_temp2.png}\\
\includegraphics[width=0.5\linewidth]{fig_def_temp4.png}
\includegraphics[width=0.5\linewidth]{fig_def_temp3.png}
\end{tabular}
\end{center}
\caption{Quatre déformations possibles d'un même signal sinusoïdal représenté sur les quatre figures en vert. 
Le temps est représenté sur l'axe horizontal et les valeurs des signaux sont représentées sur l'axe vertical. En haut à gauche, le signal bleu 
est perturbé par un bruit additif, en haut à droite, il est perturbé par une bruit additif de moindre ampleur ajouté à la fois sur les valeurs du signal 
et celles du temps~; en bas à gauche, il est perturbé par un bruit additif ajouté seulement sur les valeurs de temps~; en bas à droite, le bruit 
additif ajouté seulement sur les valeurs de temps est corrigé par le fait qu'un évènement postérieur à un autre évènement doit rester postérieur après 
la perturbation.}
\label{fig:def_temp_1}
\end{figure}

La figure~\ref{fig:def_temp_1} représente un même signal sinusoïdal colorié en vert $x_v(t)$ et 
différentes déformations de ce signal sinusoïdal, $x_b(t)$, colorées en 
bleu. 

Il est d'usage lorsqu'on évalue la distance entre deux courbes définies sur un même intervalle de temps $[0,T]$, de calculer la 
moyenne quadratique de la différence entre $x_v(t)$ et $x_b(t)$. 
\beqn
\boxed{
d_1(x_v,x_b)=\sqrt{\frac{1}{T}{\int_0^T \left(x_v(t)-x_b(t)\right )^2\,dt}}
}
\eeqn
Cette évaluation est souvent choisie pour sa simplicité, elle a une interprétation pertinente lorsque le signal déformé $x_b(t)$ resulte 
d'un bruit blanc gaussien centré additif, car dans ce cas $d_1(x_v,x_b)$ est une estimation de l'écart-type de cette gaussienne. Le graphe en haut à gauche 
de la figure~\ref{fig:def_temp_1} montre en bleu un signal déformé par un bruit blanc additif, on y observe que parfois la courbe bleue est au dessus 
de la courbe verte et parfois elle est en dessous. 

Il existe dans la littérature scientifique une technique permettant d'évaluer la distance avec les différences en hauteur entre les signaux mais
avec les distances euclidienne entre les courbes, c'est-à-dire pour chaque point de la courbe $x_b(t)$, on utilise la distance entre ce point et 
le point le plus proche de $x_v(t)$. Cette évaluation est pertinente lorsqu'on considère que la déformation de $x_b(t)$ résulte d'une part 
d'un variation de  la valeur du signal $x_b(t^b_n)-x_v(t^v_n)$ mais aussi une variation de la base de temps $t^b_n-t^v_n$. Le graphe en haut à droite est obtenu en ajoutant deux bruits blancs 
gaussiens centrés additifs indépendants sur les valeurs du signal et sur les instants associés à ces valeurs. 

Le graphe en bas à gauche est obtenu en ne modifiant que les bases de temps $t^b_n$ par rapport à $t^v_n$, il s'agit d'un bruit blanc gaussien centré 
additif. C'est-à-dire qu'on a l'égalité entre les valeurs des signaux $x_b$ et $x_v$ mais les valeurs ont lieu à des instants différents. 
\beqns
x_b(t^b_n)=x_v(t^v_n)
\eeqns
Sur ce graphe, la courbe bleue présente des boucles suggérant que le temps s'inverse parfois. Ceci n'est pas une modélisation réaliste. 

Le graphe en bas à droite est obtenu aussi en ne modifiant que les bases de temps $t^b_n$ par rapport à $t^v_n$, mais pour plus de réalisme, l'ordre des 
évènements est respecté, il n'y a donc plus de boucles.
\beqns
t^v_n\leq t^v_{n'}\quad\Rightarrow\quad t^b_n\leq t^b_{n'}
\eeqns
Concrètement, les variations de $t^b_n$ sont limitées par la contrainte que $t^b_{n}\leq t^b_{n+1}$ doit toujours être vrai. 
C'est ce type de  déformation du signal que l'on cherche à prendre en compte. Quand on prononce un son plus lentement pour plus rapidement ou 
avec une vitesse qui varie au cours de la prononciation du son, il s'agit du même son. La distance devrait théoriquement ne pas 
être sensible à ce type de déformation. 
On appelle cette déformation, une déformation temporelle dynamique.~\footnote{Cette notion est présentée en détail dans~\cite{Cassisi12}.} 


\subsubsection{Table d'indexation}

\begin{figure}
\begin{center}
\begin{tabular}{c}
\includegraphics[width=0.5\linewidth]{fig_7.png}
\end{tabular}
\end{center}
\caption{En vert et bleu, deux signaux sont définis sur des intervalles de temps différents $(t_n,x_n)$, $(t'_n,y_n)$.
En rouge, le signal $(t_n,x_n)$ est transformé par une table d'indexation en 
$(t'_{\Phi_{y}[n]},x_{\Phi_x[n]})$ de façon à approcher le signal $(t'_n,y_n)$.}
\label{fig7}
\end{figure}

La figure~\ref{fig7} illustre ce que l'on cherche à faire avec deux tables d'indexation. 
Le trait bleu associé à $x_n$ est défini sur l'intervalle de temps $[0,20]$, tandis que la courbe verte associée à $y_n$ 
est définie sur l'intervalle de 
temps $[0,15]$. Le signal $x_{\Phi_x[n]}$ est défini pour les entiers $\{0\ldots 21\}$ et est à valeurs parmi les 
valeurs de $\{x_0\ldots x_{20}\}$, ce sont des points qui sont sur la courbe rouge. La courbe rouge est en fait 
obtenue avec reliant les points $(t_{\Phi_y[n]},x_{\Phi_x[n]})$.
\beqns
\begin{array}{llcl}
\Phi_x[0]=0 & \Phi_y[0]=0 & (t_{\Phi_y[0]},x_{\Phi_x[0]})=(t_0,x_0)=(0,0) & \mbox{position initiale en bas à gauche}\\
& & \vdots& \\
\Phi_x[3]=3 & \Phi_y[1]=0 & (t_{\Phi_y[3]},x_{\Phi_x[3]})=(t_0,x_3)=(0,3) & \mbox{déplacement vertical {\bf V}}\\
\Phi_x[4]=3 & \Phi_y[4]=1 & (t_{\Phi_y[4]},x_{\Phi_x[4]})=(t_1,x_3)=(1,3) & \mbox{déplacement horizontal {\bf H}}\\
\Phi_x[5]=4 & \Phi_y[5]=2 & (t_{\Phi_y[5]},x_{\Phi_x[5]})=(t_2,x_4)=(2,4) & \mbox{déplacement diagonal {\bf D}}\\
&&\vdots &
\end{array}
\eeqns 
Cet exemple illustre le fait que deux tables d'indexation permettent de modéliser un déplacement horizontal et vertical. 

En pratique, on n'utilise pas la base de temps, on modifie juste les indices avec les deux tables 
d'indexation de façon à minimiser le carré des différences entre $x_{\Phi_x[n]}$ et $y_{\Phi_y[n]}$. 
\beqn
y_{\Phi_y[n]}\approx x_{\Phi_x[n]}
\eeqn

On introduit de nouvelles notations. 
\begin{itemize}
\item $N_\Phi$: Les tables d'indexation sont définies sur une plage d'indices communs 
\beqns
n\in\{0\ldots N_\Phi-1\}
\eeqns
\item $N_x$ et $N_y$ sont le nombre d'indices pour $x_n$ et $y_n$. 
Chaque table d'indexation est à valeurs dans les indices sur lesquels $x_n$ et $y_n$ sont définis
\beqns
\Phi_x[n]\in \{0\ldots N_x-1\} \mbox{ et }\Phi_y[n]\in \{0\ldots N_y-1\}
\eeqns
\end{itemize}


En pratique, on impose que le premier indice de $\Phi_x$ corresponde au point de départ de $x_n$, le dernier de $\Phi_x$
avec le point d'arrivée de $x_n$ et de même pour $\Phi_y$ avec $y_n$. 
\beqn\label{eq:phi_contr1}
\left \{
\begin{array}{ll}
\Phi_x[0]=0,\,&\Phi_x[N_{\Phi}-1]=N_x-1\\[0.2cm]
\Phi_{y}[0]=0,\,&\Phi_{y}[N_{\Phi}-1]=N_y-1\\[0.2cm]
\end{array}
\right . 
\eeqn

On introduit la contrainte modélisant le non-retournement du temps 
\beqn\label{eq:phi_contr2}
\Phi_x[n]\leq \Phi_x[n+1] \mbox{ et }\Phi_{y}[n]\leq \Phi_{y}[n+1]
\eeqn


On rajoute une autre contrainte qui indique que la différence de temporalité entre les deux signaux ne doit pas 
être trop grande. 
Cette contrainte a aussi l'avantage de diminuer la complexité numérique de l'algorithme utilisé pour calculer cette nouvelle distance. 
\beqn\label{eq:phi_contr3}
\left |\Phi_x[n]-\Phi_{y}[n]\right |\leq \delta
\eeqn
$\delta$ étant un paramètre à définir pour calculer cette distance. 

\subsubsection{Distance définie au moyen d'un problème d'optimisation}


Pour chaque choix de $\Phi_x$ et $\Phi_y$, on a une valeur de distance qui est obtenue classiquement avec la moyenne quadratique. 
\beqn
\label{eq:tw_d1}
\boxed{
d_{\Phi_x,\Phi_{y}}(x,y)=\sqrt{\frac{1}{N_x+N_y}{\sum_{n=0}^{N_{\Phi}-1} \left(x_{\Phi_x[n]}-y_{\Phi_{y}[n]} \right )^2}}
}
\eeqn
La distance prenant  en compte de la déformation temporelle dynamique est alors défini en choisissant 
$\Phi_x$ et $\Phi_y$ de façon à respecter les contraintes définies par les équations~(\ref{eq:phi_contr1}),~(\ref{eq:phi_contr2}) et~(\ref{eq:phi_contr3}). 
et à minimiser $d_{\Phi_x,\Phi_{y}}(x,y)$.
\beqn\label{eq:prob_min}
\boxed{
d_\delta(x,y)=\underset{\Phi_x,\Phi_y}{\min}\,d_{\Phi_x,\Phi_{y}}(x,y)
}
\eeqn

\subsubsection{Algorithme résolvant ce problème d'optimisation}

\begin{figure}
\begin{center}
\begin{tabular}{c}
\includegraphics[width=0.5\linewidth]{fig_8c.png}
\includegraphics[width=0.5\linewidth]{fig_8d.png}
\end{tabular}
\end{center}
\caption{\`A gauche~: représentation temporelle des signaux $x_n$, $y_n$ et $x_n$ transformés par déformation temporelle. 
\`A droite~: représentation des tables d'indexation permettant de générer la déformation temporelle du signal $x_n$. 
}
\label{fig8}
\end{figure}

La gauche de la figure~\ref{fig8} est similaire à la figure~\ref{fig7} avec en bleu et vert deux signaux $(t_n,x_n)$ et $(t_n,y_n)$ et 
en rouge, la déformation du premier signal pour se rapprocher du second~: $(t_{\Phi_y[n]},x_{\Phi_x[n]})$. 
La droite de cette figure montre les valeurs prises par~$\Phi_x[n]$ et~$\Phi_y[n]$ en représentant ces deux tables 
comme une succession de points formant un chemin reliant au départ~$(0,0)$ au point d'arrivée~$(N_x,N_y)=(5,3)$.
Ces contraintes correspondent à  l'équation~(\ref{eq:phi_contr1}). 
On satisfait la contrainte de l'équation~(\ref{eq:phi_contr2}) en imposant que le chemin soit composé seulement de 
déplacement verticaux, horizontaux ou diagonaux et en l'occurrence seulement d'un pas à la fois. 
La contrainte indiquée par l'équation~(\ref{eq:phi_contr3}) est indiquée par les traits noirs hachurés à l'extérieur de la zone autorisée sur la 
droite de la figure~\ref{fig8}. 
 


Les valeurs utilisées pour les signaux représentés sur la figure~\ref{fig8} sont 
\beqns
\begin{array}{llllll}
x_0=0 & x_1=1 & x_2=2 & x_3=3 & x_4=4 & x_5=5\\[0.2cm]
y_0=0 & y_1=2 & y_2=4 & y_3=5\\[0.2cm]
\end{array}
\eeqns
Les tables d'indexations créées sont~: 
\beqns
\begin{array}{llllll}
\Phi_x[0]=0 & \Phi_x[1]=1 & \Phi_x[2]=2 & \Phi_x[3]=3 & \Phi_x[4]=4 & \Phi_x[5]=5 \\[0.2cm]
\Phi_y[0]=0 & \Phi_y[1]=0 & \Phi_y[2]=0 & \Phi_y[3]=1 & \Phi_y[4]=2 & \Phi_y[5]=3 \\[0.2cm]
\end{array}
\eeqns

On appelle arête ({\em edge}) les traits associés au déplacement sur le graphe de droite. On appelle noeud ({\em node}, {\em vertice}) les 
points indiqués par des ronds bleus sur le graphe de droite. 
La localisation du point $n$ est déterminé par $\Phi_x[n]$ et $\Phi_y[n]$, il se trouve que ces valeurs déterminent aussi 
\beqns
(x_{\Phi_x[n]}-y_{\Phi_y[n]})^2
\eeqns
Les nombres en bleus situés à côté de chaque noeud donnent la valeur de cette quantité. 
Ce sont les valeurs de $x_n$ et $y_n$ qui donnent à chaque point du graphe de droite une valeur pour $(x_{\Phi_x[n]}-y_{\Phi_y[n]})^2$
dépendant uniquement de la position du point. 
La distance entre les deux signaux telle que définie dans l'équation est à la somme des quantités inscrites à côté de chaque noeud. 
L'équation~(\ref{eq:prob_min}) indiquant que la distance est obtenue à partir du chemin minimisant $d_{\Phi_x,\Phi_y}(x,y)$
 définie par l'équation~(\ref{eq:tw_d1}). Il se trouve que le graphe à droite de la figure~\ref{fig8} donne une interprétation de cette minimisation. 
$d_{\Phi_x,\Phi_y}(x,y)$ est la somme des valeurs associées à chaque point et qui ne dépend que de la position des points. 
La minimisation consiste donc à trouver le chemin minisant la somme des valeurs de chaque noeud en utilisant que des déplacements verticaux, horizontaux ou diagonaux et menant d'un point de départ à un point d'arrivée tout en restant dans le domaine délimité par les zones hachurées. 

L'algorithme permettant cette minimisation s'appelle l'algorithme de Dijkstra. 
Il consiste dans un premier temps à découvrir tous les noeuds possibles.
\begin{itemize}
\item Le premier noeud regardé est le point de départ et on lui affecte la valeur associée $(x_0-y_0)^2$. 
\item On répète la tâche suivante
\begin{enumerate}
\item\label{it:vois} Aller au voisin et lui donner la valeur de la distance entre le point de départ et ce voisin. 
\item On indique aussi à ce voisin le noeud précédent où l'on était. 
\item Si sur ce voisin il y a déjà une valeur, alors cette valeur doit être diminuée si la distance trouvée est moindre et 
on lui change l'origine que si l'on change sa valeur. 
\item Revenir au noeud précédent. 
\item Aller à l'étape~\ref{it:vois} s'il y a un voisin disponible et non-exploré dans cette tâche. 
\item Revenir au premier voisin et s'autoriser à aller à une profondeur supplémentaire. 
\end{enumerate}
\end{itemize}
Lorsque ces tâches ne peuvent plus être répétés parce qu'on a été au maximum de la profondeur possible, alors 
on part du point d'arrivée et on remonte au point de départ en suivant les indications laissées à chaque noeud. 




\begin{figure}
\begin{center}
\begin{tabular}{c}
\includegraphics[width=\linewidth]{fig_dist_temp_bis.png}
\end{tabular}
\end{center}
\caption{\`A gauche~: représentation temporelle des signaux $x_n$, $y_n$ et $x_n$ transformés par déformation temporelle. 
\`A droite~: représentation des tables d'indexation permettant de générer la déformation temporelle du signal $x_n$. 
}
\label{fig8bis}
\end{figure}

La figure~\ref{fig8bis} est assez similaire à la figure~\ref{fig8} mais avec d'autres valeurs pour les signaux $x_n$, $y_n$, $\Phi_x[n]$ et $\Phi_y[n]$. 



\section{Prédiction par le plus proche voisin}
\label{sec:knn}
\subsection{Principe}

\begin{figure}
\begin{center}
\begin{tabular}{c}
\includegraphics[width=\linewidth]{knn_ex1.png}
\end{tabular}
\end{center}
\caption{Visualisation de sons à travers les valeurs des indicateurs $\mu_\sm{PMCT}$ et $\sigma_\sm{PMCT}$}
\label{fig_knn}
\end{figure}

On appelle {\bf classifieur} le programme ou le procédé par lequel il est estimé que le son appartient à telle classe. 

On appelle {\bf prédiction} le fait pour un classifieur d'estimer qu'un son appartient à une classe en utilisant uniquement les données 
numériques disponible pour ce son. 

La prédiction par le plus proche voisin est un cas particulier d'un classifieur appelé $k$-NN pour {\em Nearest Neighbor} ce qui signifie 
justement les $k$ plus proche voisins. Ce classifieur est performant mais très coûteux en terme de complexité numérique dès lors que la 
base de donnée est assez importante. Il est aussi particulièrement simple à implémenter, ce qui est la raison principal de son choix ici. 
Il est utilisé ici dans le cas où $k=1$. 

Ce classifieur consiste pour chaque son inconnu appelé requête, de parcourir tous les sons de la base de données et pour chaque son de 
calculer sa distance avec la requête. Le classifieur détermine la classe comme étant celle du son ayant la plus petite distance avec la requête. 
Cette classe est appelée la prédiction faite par le classifieur pour cette requête. 
Il est intéressant de remarquer que ce choix de faire une classification en fonction d'un seul élément (ou de $k$ éléments dans la version plus 
générale de cet algorithme) permet de s'adapter à une situation ou une classe regrouperait des éléments très hétérogènes. 


La figure~\ref{fig_knn} montre comment une vingtaine de sons peuvent être visualisés sur un graphe. Chaque point correspond à un son, sa couleur 
(bleu pour {\tt un}, vert pour {\tt deux}, rouge pour {\tt trois}) indique le mot que ce son vocalise. Cette information est ce que l'on cherche à prédire avec 
la prédiction par le plus proche voisin. La localisation de chaque point dépend des valeurs de deux indicateurs, $\mu_{\sm{PMCT}}$ et $\sigma_{\sm{PMCT}}$. 
Ces indicateurs ont été présentés dans les sections~\ref{ssec:PMCT} et~\ref{ssec:mu_sigma}, c'est un programme informatique qui à partir des
données enregistrées permet de calculer ces deux valeurs et ainsi de positionner ces points sur ce graphique.
Pour illustrer le fonctionnement de cette technique de prédiction, voici son fonctionnement. 
\begin{enumerate}
\item  Sélectionnez dix points que vous numérotez de $1$ à $10$. 
\item Considérer un autre 
point qui ne figure pas parmi ces points. Ce point est appelé requête. 
\item Mesurez avec une règle la distance entre ce point requête et chacun de ces 10 points numérotés. 
\item Regardez la couleur du point qui a la distance avec le point requête la plus faible (et qui est donc sur le graphique 
le plus proche du point requête parmi les 10 points numérotés).
\item La prédiction consiste à attribuer au point requête la couleur du point le plus proche et par suite la classe, {\tt un}, {\tt deux} ou 
{\tt trois} suivant la 
couleur observée. 
\end{enumerate}

\subsection{Formalisation de la technique du plus proche voisin}

 Pour formaliser cette technique du plus proche voisin, on adopte les notations suivantes. 
\begin{itemize}
\item $x$ désigne en général un son défini pour plus de généralité par ses valeurs  $x_n$. 
\item $\chi$ désigne un ensemble de sons. 
\item $y$ désigne la classe à laquelle le son $x$ appartient, ({\tt un}, {\tt deux} ou {\tt trois}), est indiqué par son appartenance respective à $\chi_1, \chi_2,\chi_3$. 
\item $\br{d}(x_a,x_b)$ est une valeur positive correspondant à 
la distance entre les sons $x_a$ et $x_b$. En fait pour plus de généralité, ce calcul repose sur la réalisation des 
étapes suvantes. 
\begin{itemize}
\item Découpage de $x_a$ et $x_b$ en trames décrit à la section~\ref{sec:N:son_trames}.
\item Calcul d'un indicateur par trame pour $x_a$ et $x_b$, illustré par $\sm{PMCT}$ décrite à la section~\ref{ssec:PMCT}.
\item Mise en  oeuvre d'une des trois distance présentées dans les sections~\ref{ssec:mu_sigma},~\ref{ssec:dist_trames},~\ref{ssec:dist_def_temp}. 
\end{itemize}
\item $\br{d}(x,\chi)$ désigne la distance entre le son $x$ et un ensemble de sons regroupés dans $\chi$. 
Du fait du choix de la technique du plus proche voisin, cette distance est ici définie par 
\beqn
\boxed{
\br{d}(x,\chi)=\min\limits_{x'\in \chi} \br{d}(x,x')
}
\eeqn
où $\min\limits_{x'\in \chi} \br{d}(x,x')$ désigne la valeur la plus faible parmi les distances mesurées entre un son donné $x$ et 
tous les sons $x'$ contenus dans $\chi$. 
\item $\ww{x}$ désigne la classe prédite. Cette classe est prédite de cette façon. 
\beqn
\boxed{
\ww{x}=\argmin_{c\in\{1,2,3\}}\br{d}(x,\chi_c)
}
\eeqn
où $\chi_1,\chi_2,\chi_3$ regroupent des sons dont on sait qu'ils sont respectivement associés à {\tt un}, {\tt deux} et {\tt trois}. 
et $\argmin\limits_{c\in\{1,2,3\}}\br{d}(x,\chi_c)$ est ainsi défini. 
\beqns
\argmin\limits_{c\in\{1,2,3\}}\br{d}(x,\chi_c)=\left \{
\begin{array}{lclcl}
1 & \mbox{si} & \br{d}(x,\chi_1)\leq \br{d}(x,\chi_2) &\mbox{et}& \br{d}(x,\chi_1)\leq \br{d}(x,\chi_3)\\
2 & \mbox{si} & \br{d}(x,\chi_2)\leq \br{d}(x,\chi_1) &\mbox{et}& \br{d}(x,\chi_2)\leq \br{d}(x,\chi_3)\\
3 & \mbox{si} & \br{d}(x,\chi_3)\leq \br{d}(x,\chi_1) &\mbox{et}& \br{d}(x,\chi_3)\leq \br{d}(x,\chi_2)\\
\end{array}
\right . 
\eeqns

\end{itemize}


\subsection{Illustration avec l'implémentation proposée en TP}

\begin{figure}
\begin{center}
\begin{tabular}{c}
\includegraphics[width=\linewidth]{fig_rep_req.png}
\end{tabular}
\end{center}
\caption{Schéma correspondant aux différents dossiers existant et créés pour réaliser la prédiction en utilisant la technique du plus proche voisin. 
}
\label{fig9bis}
\end{figure}

La figure~\ref{fig9bis} illustre la façon  dont l'algorithme est ici implémenté. Chaque bloc représente un répertoire 
contenant des fichiers. 
Les sons que l'on utilise pour tester et évaluer la performance d'un classifieur sont en réalité issus de la base de données. 
Il faudrait donc s'assurer qu'ils ne sont pas utilisés aussi pour l'apprentissage. 
La partie qui n'est pas encadré en pointillé n'est pas modifiée lors de la mise en oeuvre de la classification. Cette
mise en oeuvre consiste à tirer aléatoirement une partie des sons des répertoires {\tt un}, {\tt deux} et {\tt trois}, 
de les placer dans le
répertoire {\tt requête}, les autres sons sont placés dans trois nouveaux répertoires contenus dans le répertoire 
{\tt simulation} et appelé {\tt un}, {\tt deux} et {\tt trois}. 
L'information selon laquelle les sons placés dans {\tt requête} n'est pas disponible sur les fichiers sons, mais elle 
est stockée pour être utilisée ultérieurement lors de l'évaluation de l'algorithme. 

\section{\'Evaluation de la performance d'un classifieur}
\label{sec:evaluation_classification}

En pratique quand on utilise un procédé de reconnaissance vocal, on a besoin de savoir dans quelle mesure on peut lui faire confiance. 
Cette mesure est ce qu'on appelle l'{\bf évaluation de la performance}. Pour se faire, on utilise des sons dont on connaît la classe à laquelle 
ils appartiennent et on compare cette classe avec ce que le classifieur prédit. Il existe un très grand nombre de mesures de performance, on en présente 
trois types~: la sensibilité globale, la précision et le rappel. 

\subsection{Matrice de confusion}

Le rôle de la matrice de confusion est de résumer sous la forme d'une matrice les données utiles au calcul de l'évaluation de la performance. 
Ces données utiles consistent en le fait de connaître le nombre d'expérience où le son requête appartenait à telle classe et où la classe prédite est 
celle-là. Dans le cadre de cette étude, il s'agit d'une matrice $3{\times}3$ puisqu'il y a trois sons possibles. 

\begin{itemize}
\item Chaque {\bf ligne} est associée aux expérimentations sur les sons qui en réalité appartiennent à telle classe. 
\item Chaque {\bf colonne} est associée aux expérimentations sur les sons qui ont été prédit comme étant de telle classe. 
\item La somme de toutes les cases est égale au nombre total d'expérimentations. 
\item \`A la case $i,j$, il y a le nombre d'expérimentations pour lesquelles le son appartient en réalité à la classe~$i$ et 
le classifieur l'a prédit comme étant de la classe~$j$. 
\item $m$ est un indice faisant référence à un son $x$. 
\item $M$ est le nombre total de sons utilisés pour les différentes requêtes. 
\item $\1(\ldots)$ est la fonction caractéristique, elle prend la valeur $1$ si les trois points de suspension sont remplacés par 
une affirmation exacte et par $0$ si l'affirmation est fausse. 
\item $\1(y_m=c)$ vaut $1$ si  le son numéro $m$ est de la classe $c$ et $\1(y_m=c)$ vaut $0$ si ce n'est pas le cas. 
\item $\1(\ww{x}_m=c)$ vaut $1$ si le son numéro $m$ est prédit par le classifieur comme étant de classe $c$ et $\1(\ww{x}_m=c)$ vaut $0$ 
si ce n'est pas le cas. 
\item $\1(y_m=i)\1(\ww{x}_m=j)$ vaut $1$ is le son numéro $m$ est d'une part de la classe $i$ et d'autre part a été prédit par le classifieur 
comme étant de la classe $j$. 
\end{itemize}

Les composantes de la matrices de confusion sont~: 
\beqn\label{eq:matrice_confusion}
\boxed{
C_{ij}={\sum_{m=1}^M\1(y_m=i)\1(\ww{x}_m=j)}
}
\eeqn


\subsection{Sensibilité globale}

La sensibilité globale, notée $\OA$ pour {\em Overall Assessment}, est 
le rapport entre le nombre de classifications correctes sur le nombre totales de requêtes, noté $M$. 
Les classifications correctes sont celles pour lesquelles $y_m=\ww{x}_m$. 

\beqn
\label{eq:OA}
\boxed{
\OA=\frac{C_{11}+C_{22}+C_{33}}{3}
}
\eeqn

\subsection{Précision et rappel}

La précision et le rappel sont des notions très utilisées pour les classifieurs binaires, c'est-à-dire pour lesquels, il n'y a que deux classes. 
Mais ces notions sont parfois étendues au cas plus général où on considère un nombre plus important de classes, c'est ce que nous utilisons ici. 

Pour chaque classe~$c$, on calcule deux indicateurs. La {\bf précision} $\p{P}_c$ est le rapport entre le nombre de requête correctement attribuées à la classe~$c$
et le nombre de requêtes que le classifieur évalué a prédit comme étant de la classe~$c$. 
Le {\bf rappel} $\p{R}_c$  est le rapport entre le nombre de requête correctement attribué à la classe~$c$ 
et le nombre de requêtes qui dans la réalité correspondent à la classe~$c$. 
\beqn
\boxed{
\left\{
\begin{array}{l}
\p{P}_1=\frac{C_{11}}{C_{11}+C_{21}+C_{31}}\\[0.3cm]
\p{P}_2=\frac{C_{22}}{C_{12}+C_{22}+C_{32}}\\[0.3cm]
\p{P}_3=\frac{C_{33}}{C_{13}+C_{23}+C_{33}}\\[0.3cm]
\end{array}
\right.
\quad
\mbox{et} \quad 
\left\{
\begin{array}{l}
\p{R}_1=\frac{C_{11}}{C_{11}+C_{12}+C_{13}}\\[0.3cm]
\p{R}_2=\frac{C_{22}}{C_{21}+C_{22}+C_{23}}\\[0.3cm]
\p{R}_3=\frac{C_{33}}{C_{31}+C_{32}+C_{33}}\\[0.3cm]
\end{array}
\right.
}
\eeqn
Ainsi la précision indique la probabilité  qu'un échantillon, dont le classeur évalué indique qu'il s'agit de la classe~$i$, 
soit effectivement de la classe~$i$. 
Par contre,  le rappel indique la probabilité pour qu'un échantillon dont on sait qu'il est de la classe~$i$, soit détecté 
comme tel par le classifieur évalué. 


\subsection{Validation croisée}

\begin{figure}
\begin{center}
\begin{tabular}{c}
\includegraphics[width=0.8\linewidth]{illustration_validation_croisee.png}
\end{tabular}
\end{center}
\caption{Schéma décrivant ce qu'est une validation croisée.}
\label{fig:O:valid_croisee}
\end{figure}


La {\bf validation croisée} est une technique souvent utilisée pour la mise en oeuvre d'un algorithme de classification, 
elle n'est pas destinée à améliorer l'efficacité d'un classifieur, elle est destinée à évaluer plus précisément sa 
performance vis-à-vis d'une base de données en particulier  lorsqu'il est compliqué d'augmenter le nombre de sons dont on connaît la
classe à laquelle chacun appartient. 
La figure~\ref{fig:O:valid_croisee} illustre le fonctionnement de la validation croisée avec un schéma. 
En haut de cette figure se trouve 12 sons figurés par $x_1\ldots x_{12}$ et $12$ valeurs notées $y_1\ldots y_{12}$ indiquant les véritables classes à laquelle chaque son appartient.
Ici il s'agit d'une validation croisée en quatre blocs, ce qui amène à réaliser quatre apprentissages de classifieurs. 
{\tt Exp1} désigne en haut la première expérience avec le premier apprentissage. Les trois premiers sons de la base 
d'apprentissage $(x_1,y_1),(x_2,y_2),(x_3,y_3)$ servent de base pour tester le classifieur et sont affichés sur fond rouge. Le classifieur testé est entraîné 
en utilisant tous les autres sons $(x_4,y_4),\ldots,(x_{12},y_{12})$ qui sont eux affichés sur fond bleu. Le test du classifieur permet de calculer une matrice 
de confusion spécifique à {\tt Exp1} et celle-ci permet de calculer la sensibilité globale $\sm{OA}_1$.
Les trois autres expériences sont fait de la même façon, mais en utilisant successivement comme sons tests les 
sons $(x_4,y_4),(x_5,y_5),(x_6,y_6)$, puis $(x_4,y_4),(x_5,y_5),(x_6,y_6)$ et enfin $(x_4,y_4),(x_5,y_5),(x_{12},y_{12})$.





\chapter{Descripteurs de trames}
\label{ch:desc}

La partie précédente ayant montrée comment un descripteur par trame permet de définir une technique de classification, cette 
partie traite de la détermination d'un descripteur par trame. 
L'inspiration qui a guidé l'élaboration des descripteurs provient de l'étude des caractéristiques des ondes sonores émises par un individu,
c'est ce qui constitue la section~\ref{sec:model_parole} et qui montre l'intérêt de trouver la fréquence fondamentale et la plage de fréquences présentes
dans le son émis. 
La section~\ref{sec:estimation_spectrale} présente différentes heuristiques permettant de décrire ce contenu spectral en indiquant la fréquence fondamentale, la 
fréquence moyenne et la largeur de spectre. 
La section~\ref{sec:banc_filtres} présente une technique plus systématique pour décrire le contenu spectral, c'est en utilisant un banc de filtres, chaque 
filtre constitue une heuristique donnant une information partielle sur le contenu spectral du son. 


\section{Modélisation de la production de la parole}
\label{sec:model_parole}

La présentation de la modélisation de la façon dont un humain produit un son est 
faite en trois parties. La section~\ref{ssec:onde_stationnaire} décrit le phénomène physique 
permettant de transformer une source sonore en un son dont le caractère plus ou moins aigü du son 
peut être déterminé assez précisément au moyen d'une note. 
La section~\ref{ssec:appareil_phonatoire} décrit brièvement les organes humains intervenant pour 
la production d'un son. 
Enfin la section~\ref{ssec:spectrogramme} présente la notion d'analyse temps-fréquence illustré 
avec la présentation d'un spectrogramme.

\subsection{Onde stationnaire}
\label{ssec:onde_stationnaire}

On dit qu'une onde est stationnaire si en chaque point, on observe que  la surpression évolue dans le temps comme une sinusoïde. 
Par exemple l'équation suivante décrit une évolution sinusoïdale dont l'amplitude crête à crête dépend de l'indice $x$ et vaut 
$\cos(2\pi \frac{x}{\lambda_0})$. 
\beqns
P(x,t)=\Delta P_0\cos(2\pi f_0t)\cos(2\pi \frac{x}{\lambda_0})
\eeqns
où $\lambda$ et $f_0$ sont 
Cette onde peut approximativement correspondre à un cas particulier de l'équation~(\ref{eq:propag_onde}) lorsque le coefficient $\frac{1}{r}$ est 
supposé approximativement constant et~$r$ est remplacé par~$x$. 
La trigonométrie nous indique
que le produit de deux cosinus est une différence entre deux sinus,
 $\cos(a)\cos(b)=\frac{1}{2}\cos(a-b)+\frac{1}{2}\cos(a+b)$. 
Cela permet de voir qu'une onde stationnaire est la somme d'une onde se propageant dans le sens des $x$ croissants et 
une autre dans le sens des $x$ décroissants.
\beqn\label{eq:onde_stationnaire}
P(x,t)=\frac{\Delta P_0}{2}\cos\left (2\pi f_0(t-\frac{x}{c})\right )
+\frac{\Delta P_0}{2}\cos\left (2\pi f_0(t+\frac{x}{c})\right )
\eeqn
où $c=\lambda_0 f_0$ est la vitesse de propagation du son dans l'air. 
Cette modélisation correspond à $g_1=g_2$ dans l'équation~(\ref{eq:propag_onde}). 




\begin{figure}[htbp]
\begin{center}
\begin{tabular}{c}
\includegraphics[width=0.5\linewidth]{onde_stationnaire.png}
\end{tabular}
\end{center}
\caption{Pour une même taille donnée, un même obstacle peut être le siège de trois ondes stationnaires. 
La vitesse moyenne des particules d'air doit être nulle aux deux extrémités de la caisse de résonnance. }
\label{fig:onde_stationnaire}
\end{figure}

La figure~\ref{fig:onde_stationnaire} illustre de manière simplifiée la façon dont la forme géométrique d'une caisse de 
résonance détermine une fréquence de résonance. 
Le haut de la figure schématise al caisse de résonance qui est un pavé. La coupe est un rectangle. La zone colorée 
en bleu schématise une onde stationnaire qui consiste en une variation spatiale et temporelle avec une relation 
entre la longueur d'onde et la fréquence de la vibration indiquée dans l'équation~\ref{eq:long_onde} ($\lambda=c/f$ où 
$c$ est ici la vitesse de propagation du son dans l'air, approximativement 1km toutes les $3$~secondes). Les trois dessins 
illustrent qu'avec une même forme géométrique (un pavé de longueur $d$), $3$ longueurs d'onde sont montrés. 
\begin{center}
\begin{tabular}{|c|c|c|}
\hline 
$\lambda=2d$ & $f=\frac{c}{2d}$ & $d=\frac{\lambda}{2}$\\[0.1cm]
\hline
$\lambda=d$ & $f=2\frac{c}{2d}$ & $d={\lambda}$\\[0.1cm]
\hline
$\lambda=\frac{2}{3}d$ & $f=3\frac{c}{2d}$ & $d=\frac{3\lambda}{2}$\\[0.1cm]
\hline
\end{tabular} 
\end{center}

Cette schématisation illustre un phénomène plus général, à savoir que l'émission d'un son à une certaine fréquence de base
produit généralement des harmoniques qui sont des vibrations à des fréquences qui sont multiples de cette fréquence de base. 
La relation entre longueur du rectangle et longueur d'onde est ici déterminé par le fait que la vibration 
du son est nul sur la paroi (i.e. la paroi est fixe). Dans une onde stationnaire modélisée par l'équation~(\ref{eq:onde_stationnaire}),
c'est à cet endroit que la pression est soit maximale soit minimale.
L'annexe~\ref{app:onde_stationnaire_1D} formalise cette description de manière plus précise.  

Une onde stationnaire peut aussi exister avec un rectangle ouvert sur un côté. Dans ce cas c'est la pression qui est fixée et la vibration 
qui est maximale à l'endroit où le rectangle est ouvert. Les relations entre longueurs d'onde, fréquences et longueur du rectangle sont alors modifiées. 
\begin{center}
\begin{tabular}{|c|c|c|}
\hline 
$\lambda=4d$ & $f=\frac{c}{4d}$ & $d=\frac{\lambda}{4}$\\[0.1cm]
\hline
$\lambda=\frac{4}{3}d$ & $f=3\frac{c}{4d}$ & $d=\frac{3\lambda}{4}$\\[0.1cm]
\hline
$\lambda=\frac{4}{5}d$ & $f=5\frac{c}{4d}$ & $d=\frac{5\lambda}{4}$\\[0.1cm]
\hline
\end{tabular} 
\end{center}



\subsection{Modélisation de l'appareil phonatoire}
\label{ssec:appareil_phonatoire}


\begin{figure}[htbp]
\begin{center}
\begin{tabular}{c}
\includegraphics[width=0.5\linewidth]{parole_formation.jpg}
\end{tabular}
\end{center}
\caption{Diagramme représentant les organes de la parole }
\label{fig:parole_formation}
\end{figure}

On appelle appareil phonatoire l'ensemble des organes humains permettant de produire un son. 
L'objet de cette partie est une brève description de son fonctionnement. 

La figure~\ref{fig:parole_formation} représente une coupe de la tête d'une personne, (coupe dite sagittale), avec la gorge en bas à droite, la bouche au milieu à gauche, les dents le long d'une ligne horizontale placée légèrement au dessus de la bouche. 
Cette figure permet de modéliser la façon dont un son est formé. 
\begin{itemize}
\item Le son est produit par la vibration d'un organe musculaire appelé corde vocale ou plis vocaux. Cet organe musculaire 
permet un contrôle de la fréquence du son émis à ce niveau.  
\item L'intensité du son est modulé par l'intensité du flux d'air sortant du poumon situé plus bas. 
\item Une première caisse de résonance est localisée dans la bouche et sa forme géométrique est modulée notamment par 
la position de la langue et l'ouverture de la bouche. Cette forme géométrique entraîne la formation de vibrations. 
\item Une deuxième caisse de résonance est localisée dans un espace libre au dessus de la bouche au niveau du nez, espace 
appelé cavité nasale. Cette deuxième caisse de résonance entraîne la formation d'un son avec une certaine fréquence. 
\end{itemize}

Ainsi l'anatomie du corps humain permet de modifier l'intensité d'un son et la différence entre deux fréquences 
de résonance. 




%\begin{figure}[htbp]
%\begin{center}
%\begin{tabular}{c}
%\includegraphics[width=0.5\linewidth]{coupe_schematique_parole.png}
%\end{tabular}
%\end{center}
%\caption{Diagramme représentant les organes de la parole, extraite de~\cite{KhederW17} }
%\label{fig:coupe_schematique_parole}
%\end{figure}
%\section{Estimation spectrale}

\subsection{Spectrogramme et notion de description temps-fréquence}
\label{ssec:spectrogramme}

\begin{figure}[htbp]
\begin{center}
\begin{tabular}{c}
\includegraphics[width=0.5\linewidth]{spectrogramme.png}
\end{tabular}
\end{center}
\caption{spectrogramme d'un signal sonore.}
\label{fig:spectrogramme}
\end{figure}

La figure~\ref{fig:spectrogramme} est un exemple de spectrogramme, c'est une visualisation d'un son, ici 
constitué d'une partie parlée à gauche, un silence au milieu, et de nouveau une partie parlée à droite. 
L'axe horizontal est le temps en seconde. L'axe vertical est la fréquence en Hertz. 
Il s'agit d'une représentation temps-fréquence, ce qui peut paraître contradictoire dans le cadre de ce cours. 
En effet une description temporelle d'un signal ne dépend pas de la fréquence et une description fréquentielle d'un signal 
au moyen de son spectre ne dépend pas du temps. En fait la position latérale d'un point détermine une portion du signal sur un intervalle
de temps. Tous les points d'une même verticale concernent la même portion du signal. 
Cette portion de signal est transformée en un spectre qui permet d'indiquer comment l'énergie de cette portion du signal est décomposée en 
une somme  de signaux sinusoïdaux. Chaque point de cette verticale représente une de ces sinusoïdes, c'est la hauteur de ce point qui en déterminant 
une fréquence détermine aussi la sinusoïde. Et un point 
 est d'autant plus sombre ou rouge que l'amplitude du signal sinusoïdal est plus importante. Sur ce spectrogramme, on observe une alternance de 
bandes sombres/rouges horizontales qui sont à la fois régulièrement espacées et avec des intensités qui diminues lorsque la fréquence augmente. 
Ce phénomène est lié au caisses de résonance qui produisent des sons avec une fréquence de base et des harmoniques qui sont des multiples 
de la fréquence de base.

Historiquement la recherche en reconnaissance de la parole s'est d'abord donnée comme guide le fait 
de modéliser les organes qui produisent ou reconnaissent la parole. En pratique la complexité numérique 
et la difficulté à modéliser limitaient la précision des modèles obtenues et par suite la performance. 
Il semble aujourd'hui admis que les techniques de machine learning permettent plus facilement d'obtenir 
des techniques efficaces. Il reste cependant de toutes ces études l'importance apportée à l'utilisation 
d'un certain type de descripteurs et par exemple l'importance d'estimer la fréquence fondamentale. 
L'utilité de s'intéresser à la fréquence fondamentale pour reconnaître une voyelle est 
expliquée en détail dans~\cite{Meunier07}.











\section{Estimation spectrale}
\label{sec:estimation_spectrale}

L'objet de cette partie est de définir 
une application transformant les valeurs sur une trame~$k$ en une valeur donnée, appelée valeur du 
descripteur. 
La section~\ref{ssec:estimation_frequence_fondamentale} présente des techniques permettant 
d'estimer la fréquence fondamentale. 
La section~\ref{sec:descripteur_spectre} presente d'autres techniques permettant d'estimer 
d'autre caractéristiques du spectre, par exemple sa largeur. 

\subsection{Estimation de la fréquence fondamentale}
\label{ssec:estimation_frequence_fondamentale}

Dans cette partie, les deux indicateurs présentés ont pour objectif d'estimer la fréquence fondamentale.~\footnote{Pour un son musical assez simple, cette 
fréquence correspond au {\em pitch} défini section~C.3, p.~215-217 de~\cite{Rocchesso03}.} 

Une autre technique existe pour mesurer la fréquence fondamentale en s'appuyant sur l'autocorrélation.~\footnote{Cette 
technique est brièvement présentée p.~45-46 dans~\cite{Camastra07}.}


\subsubsection{Zero Crossing Rate}

\begin{figure}[htbp]
\begin{center}
\begin{tabular}{c}
\includegraphics[width=0.5\linewidth]{zero_crossing_rate.png}
\end{tabular}
\end{center}
\caption{Graphe illustrant le fonctionnement de l'indicateur $\mb{ZCR}$. }
\label{fig:zero_crossing_rate}
\end{figure}


La figure~\ref{fig:zero_crossing_rate} montre l'évolution de deux signaux en fonction du temps. 
Le premier en trait plus foncé/bleu est la superposition de 2 sinusoïdes. Le deuxième 
 en trait plus clair/vert est une sinusoïde.  Le descripteur~\footnote{Cette technique 
appelée {\em zero crossing rate} est évoquée dans la section~2.4 p.~12 de~\cite{Peeters04}, 
et définie dans~\cite{Camastra07} p.~43-44.} 
$\mb{ZCR}$ détermine le nombre de fois où la courbe traverse l'axe horizontal par une unité de temps. 
Ici il y a deux traversées toutes les secondes. 

Le nombre de passage par zéro n'est en fait pas une notion qui se prête à une formalisation 
utilisant le temps continu. 
Le nombre moyen de passages par zéro pour la trame $k$ est donnée par
\beqn
\label{eq:ZCR}
\boxed{
Z_k=\frac{1}{N_K}{\sum_{n=0}^{N_K-1} \1\left (\signe(x_k[n+1])\neq \signe(x_k[n])\right)}
}
\eeqn
Le fait de normaliser par la longueur de la trame ($N_K$) fait que $Z_k$ n'est pas augmenté lorsque 
les trames sont plus longues. 

Ce nombre moyen de passage par zéro est utilisé pour estimer la fréquence fondamentale, c'est la fréquence 
de la sinusoïde qui aurait ce nombre moyen de passages par zéros. 
\beqn
\label{eq:f_ZCR}
\boxed{
f^{(\sm{ZCR})}_k=\frac{Z_k f_e}{2}
}
\eeqn
En effet, pour une sinusoïde de fréquence $f^{(\sm{ZCR})}_k$, sa période est $T=\frac{1}{f^{(\sm{ZCR})}_k}$ 
et le nombre moyen de passages par zéros est $2$ divisé par le nombre de points sur une période $Tf_e$, 
aussi 
\beqns
f^{(\sm{ZCR})}_k=\frac{1}{T}=\left(\frac{2}{T f_e}\right ) \frac{f_e}{2}=\frac{Z_k f_e}{2}
\eeqns


\subsubsection{Fréquence moyenne du spectre}

\begin{figure}[htbp]
\begin{center}
\begin{tabular}{c}
\includegraphics[width=0.5\linewidth]{illustration_frequence_moyenne.png}
\end{tabular}
\end{center}
\caption{Illustration du calcul de la fréquence moyenne et 
de sa signification comme séparant en deux parties 
égales la surface sous la courbe.}
\label{fig:illustration_frequence_moyenne}
\end{figure}

La notion de temps-fréquence évoquée lors de la description du spectrogramme dans la section~\ref{ssec:spectrogramme}
permet de définir une densité spectrale d'énergie qui dépend du temps. Ici cela se fait en 
appliquant une fenêtre rectangulaire avec l'intervalle $\left [t-\frac{T}{2},t-\frac{T}{2}\right]$
sur le signal $x(t)$. 
\beqn
\label{eq:DSP_t}
\boxed{
\left|\ww{X}_t(f)\right|^2=\left |\mb{TF}\left [x(t)\1_{\left [t-\frac{T}{2},t-\frac{T}{2}\right]}(t)\right](f)
\right|^2
}
\eeqn
Ensuite cette densité spectrale dépendant du temps et de la fréquence est une utilisée 
comme pondération dans $\mu(t)$ qui est appelée la fréquence moyenne (son unité est bien le Hertz). 
\beqn\label{eq:mu_t}
\boxed{
\mu(t)=\frac{{\int\limits_0^{+\infty} f\left |\ww{X}(f)\right |^2\,df}}
{{\int\limits_0^{+\infty} \left |\ww{X}(f)\right |^2\,df}}
}
\eeqn
On peut voir ce calcul de moyenne comme assez similaire au calcul de l'espérance 
d'une variable aléatoire à partir de la densité de probabilité d'une variable aléatoire~: 
$E[T]={\int_\bb{R} tf_T(t)\,dt}$ où ici $f$ jouerait le rôle de $t$ et 
$\frac{\left |\ww{X}(f)\right |^2}{{\int\limits_0^{+\infty} \left |\ww{X}(f)\right |^2\,df}}$
jouerait le rôle de $f_T(t)$.

La figure~\ref{fig:illustration_frequence_moyenne} donne une justification 
de la définition de $\mu(t)$ dans l'équation~(\ref{eq:mu_t}).
La courbe en noir notée $P(f)$,
correspondant en réalité à $|\ww{X}_t(f)|^2$, 
est la densité spectrale d'énergie d'une portion du signal 
$x(t)\1_{[t-\frac{T}{2},t+\frac{T}{2}]}(t)$. 
Le trait semi-pointillé vertical est positionné 
%à la fréquence $\mu(t)$. On considère maintenant 
%la surface sous la courbe à gauche de $\mu(t)$, 
%elle est égale au terme de gauche de la deuxième 
%égalité
%\beqns
%{\int_{0}^{\mu(t)}(\mu(t)-f)P(f)\,df}
%\eeqns
%La surface sous la courbe à droite de $\mu(t)$ 
%est égale au terme de droite de la deuxième égalité
%\beqns
%{\int_{\mu(t)}^{+\infty}(f-\mu(t))P(f)\,df}
%\eeqns
%Ainsi qu'il est indiqué à gauche de la figure, 
%l'égalité de ces deux dernières équations conduit 
%à la définition de $\mu(t)$ donnée dans l'équation~(\ref{eq:mu_t}). 
%Ainsi on peut dire que cette moyenne temporelle est 
%la fréquence qui divise en deux parties égales la surface 
%sous la courbe de la densité spectrale d'énergie de la portion 
%de signal. 
%de signal. 

Cette notion est adaptée aux signaux à temps discret en 
considérant la portion du signal~\footnote{Cette application 
de la transformée de Fourier discrète sur 
le signal découpé peut être vu comme 
l'utilisation d'une transformée 
de Fourier à court terme, p.~99 de~\cite{Rocchesso03}.} 
 sur une trame $x_k[n]$ et en lui calculant la transformée de Fourier discrète considérant 
que la longueur de la trame est suffisante pour que cette transformée de Fourier discrète
soit une bonne approximation de la transformée de Fourier de cette portion de signal. 
On utilise ici un indice $l$ pour les fréquences et on ne considère que la première 
moitié des $N_K$ indices parce que la deuxième moitié des indices correspond aux fréquences 
négatives qui n'est pas prise en compte dans l'équation~(\ref{eq:mu_t}).
Cette première moitié des indices est notée 
\beqn\label{eq:N_K_2}
\boxed{
N_K^{\deux}=\left \lfloor \frac{N_K}{2} \right\rfloor
}
\eeqn
où $\lfloor\ldots \rfloor$ désigne l'arrondi par en dessous. 
Les $N_K^{\deux}$ premières fréquences sont 
$\left [0\ldots \frac{N_K^{\deux}f_e}{N_K}\right]$. 
Ces différentes valeurs sont écrites au moyen d'un nouvel indice $l$ dont dépend la fréquence. 
\beqn\label{eq:f_l}
\boxed{
f_l=\frac{lf_e}{N_K}\mbox{ pour }l\in \{0\ldots N_K^{\deux}
}
\eeqn
La pondération utilisée est la densité spectrale de puissance de la trame $k$.
\beqn
\boxed{
\left |\ww{X}_k[l]\right |^2= \left |
\sm{TFD}\left [x_k[n]\right][l]\right |^2
}
\eeqn
Un estimateur de la fréquence moyenne du spectre $\mu_k$~\footnote{Cet estimateur 
est défini dans la section~6.1.1 p.~13 de~\cite{Peeters04}.}
 est  
\beqn\label{eq:mu_sp}
\boxed{
\mu_k=\frac{{\sum_{l=0}^{N_K^{\deux}}\,\,f_l\,\,\left |\widehat{X}_k[l]\right |^2}}
{{\sum_{l'=0}^{N_K^{\deux}}\left |\widehat{X}_k[l']\right |^2}}
}
\eeqn 
% où $\widehat{X}_k[l]$ est la transformée de Fourier discrète à $k$ fixé de $x_k[n]$ définie par 
% $\widehat{X}_k[l]=\frac{1}{N_K}{\sum_{n=0}^{N_K-1}x_k[n]e^{-j2\pi\frac{ln}{N_K}}}$~;
% et ${\lfloor \frac{N_K}{2}\rfloor}$ signifie le plus grand entier inférieur à $N_K/2$. 
Un indice $l'$ est utilisé parce qu'il n'y a en fait aucun lien entre le compteur utilisé dans la sommation au niveau du numérateur et
le compteur utilisé dans la sommation au niveau du dénominateur. 

\subsection{Autre descripteurs du spectre}
\label{sec:descripteur_spectre}

\subsubsection{Largeur du spectre}

\begin{figure}[htbp]
\begin{center}
\begin{tabular}{c}
\includegraphics[width=0.5\linewidth]{illustration_largeur_spectre.png}
\end{tabular}
\end{center}
\caption{Illustration graphique sur un exemple du sens donné à la notion d'estimation de la largeur d'un spectre.}
\label{fig:illustration_largeur_spectre}
\end{figure}


La largeur du spectre est estimée connaissant $\mu(t)$ avec 
\beqn
\label{eq:largeur_spectre}
\boxed{
\sigma(t)=\frac{\sqrt{{\int\limits_{\bb{R}_+}\left(f-\mu(t)\right)^2\left |\ww{X}_t(f)\right|^2\,df}}}{\sqrt{{\int\limits_{\bb{R}_+}\left |\ww{X}_t(f)\right|^2\,df}}}
}
\eeqn

La figure~\ref{fig:illustration_largeur_spectre} représente l'exemple d'un spectre d'une porte. 
La fréquence est en abscisse. Ce spectre a pour équation un sinus cardinal avec un demi-lobe principal de $3000$Hz. 
Cette figure illustre deux descripteurs $\mu$ et $\sigma$. $\mu$ est la fréquence moyenne et $\sigma$ est l'écart-type. 
Les deux sont calculés comme si les spectres étaient nuls pour les fréquences négatives (s'ils étaient calculés sur les 
vrais spectres, comme leur module est symétrique, la moyenne serait nulle. 
$\mu$ est indiqué par un trait vertical en pointillé. $\sigma$ est représenté par deux traits verticaux autour de celui associé à $\mu$. 
Ces deux traits verticaux indiquent que si le spectre était une gaussienne (courbe en traits pointillés), $66\%$ de sa surface serait incluse dans ces deux traits
verticaux en pointillés. Ce graphe n'est en fait pas tout à fait exact, d'une part la proportion de $66\%$ et l'axe de symétrie au centre de la gaussienne n'est 
ici pas valable puisqu'on ne considère que les fréquences positives, d'autre part la moyenne et le calcul de la largeur se fait en considérant 
la densité spectrale et non le module de la transformée de Fourier et cette densité spectrale n'est donc pas exactement un sinus cardinal.

De même pour le calcul de la moyenne temporelle, l'équation~(\ref{eq:largeur_spectre}) décrivant l'estimation de la largeur du spectre peut 
se voir comme l'estimation de l'écart-type d'une variable aléatoire positive de densité de probabilité $f_T(t)$
\beqns
\sqrt{\mb{var}(T)}=\sqrt{E[(T-E[T])^2]}=\sqrt{{\int\limits_{\bb{R}_+}(t-E[T])^2f_T(t)\,dt}}
\eeqns
où ce qui remplace ici la variable $t$ est $f$ et la densité de probabilité $f_T(t)$ est 
\beqns
\frac{1}{{\int\limits_{\bb{R}_+}\left |\ww{X}_t(f)\right|^2\,df}}\, \left |\ww{X}_t(f)\right|^2
\eeqns



En utilisant les mêmes notations que pour (\ref{eq:mu_sp}), une estimation de la largeur du spectre~\footnote{Cet estimateur est défini dans la section~6.1.2 p.~13 de~\cite{Peeters04}.} est
\beqn
\label{eq:sigma_sp}
\boxed{
\sigma_k=\sqrt{\frac{{\sum_{l=0}^{N_K^\deux}\,\,\left (f_l-\mu_k\right )^2\,\,
\left |\ww{X}_k[l]\right |^2}}{{\sum_{l'=0}^{N_K^\deux}\left |\widehat{X}_k[l']\right |^2}}}
}
\eeqn

%En reprenant les notations utilisée pour (\ref{eq:mu_pl}), cet estimateur de la largeur du spectre peut s'écrire ainsi. 
%\beqn
%\sigma=\sqrt{
%{\sum_{l=0}^{l_{\max{}}}(f_l-\mu)^2 \frac{p_l}{{\sum_{l'=0}^{l_{\max{}}} p_{l'}}}}
%}
%\eeqn
%Ainsi $\sigma$ peut s'interpréter comme la racine carré de la variance d'une variable aléatoire discrète $F$ dont les probabilités sont 
%données par $\frac{p_l}{{\sum_{l'=0}^{l_{\max{}}} p_{l'}}}$. 


\subsubsection{Coefficient d'asymétrie du spectre}

Un estimateur du coefficient d'asymétrie ({\em skewness})~\footnote{Cet estimateur est défini dans la section~6.1.3 p.~13 de~\cite{Peeters04}.} est donné 
par 
\beqns
\gamma_1(t)=\frac{1}{\sigma^3(t)}\frac{{\int\limits_{\bb{R}_+}\left(f-\mu(t)\right)^3\left |\ww{X}_t(f)\right|^2\,df}}{{\int\limits_{\bb{R}_+}\left |\ww{X}_t(f)\right|^2\,df}}
\eeqns
qui devient avec les notations utilisées dans (\ref{eq:sigma_sp}).
\beqn
\gamma_1[k]=\frac{1}{\sigma_k^3}{\frac{{\sum_{l=0}^{N_K^\deux}\,\,\left (f_l-\mu_k\right )^3\,\,
\left |\ww{X}_k[l]\right |^2}}{{\sum_{l'=0}^{N_K^\deux}\left |\widehat{X}_k[l']\right |^2}}}
\eeqn
De même, un estimateur du coefficient d'aplatissement ({\em kurtosis})~\footnote{Cet estimateur est défini dans la section~6.1.4 p.~14 de~\cite{Peeters04}.} est donné par
\beqns
\gamma_1(t)=\frac{1}{\sigma^4(t)}\frac{{\int\limits_{\bb{R}_+}\left(f-\mu(t)\right)^4\left |\ww{X}_t(f)\right|^2\,df}}{{\int\limits_{\bb{R}_+}\left |\ww{X}_t(f)\right|^2\,df}}
\eeqns
qui devient avec les notations utilisées dans (\ref{eq:sigma_sp}).
\beqn
\gamma_2[k]=\frac{1}{\sigma_k^4}{\frac{{\sum_{l=0}^{N_K^\deux}\,\,\left (f_l-\mu_k\right )^4\,
\,\left |\widehat{X}_k[l]\right |^2}}{{\sum_{l'=0}^{N_K^\deux}\left |\widehat{X}_k[l']\right |^2}}}
\eeqn


\section{Utilisation de bancs de filtres}
\label{sec:banc_filtres}


\begin{figure}[htbp]
\begin{center}
\begin{tabular}{c}
\includegraphics[width=0.5\linewidth]{banc_de_filtre.png}
\end{tabular}
\end{center}
\caption{Schéma d'un banc de filtres }
\label{fig:banc_de_filtre}
\end{figure}

On introduit de nouvelles notations pour décrire un banc de filtres. 
\begin{itemize}
\item $l$ est un indice qui compte les raies du spectre des trames. 
\item $f_l$ est la valeur de la fréquence associée à la raie~$l$. 
\item $m$ est un indice qui numérote les filtres utilisés dans le banc de filtres. 
\item $\ww{H}_m(f)$ est la réponse fréquentielle du filtre numéro $m$. 
\end{itemize}


La figure~\ref{fig:banc_de_filtre} schématise un banc de filtres. Le bas de la figure montre les réponses fréquentielles de $4$~filtres notés~$\ww{H}_1(f)$, 
$\ww{H}_2(f)$, $\ww{H}_3(f)$ et $\ww{H}_4(f)$. Le filtre~$\ww{H}_1$ est un passe-bas. Les filtres $\ww{H}_2(f)$ et~$\ww{H}_3(f)$ sont des filtres passe-bande.
Le filtre $\ww{H}_4(f)$ est un filtre passe-haut. Une particularité de ces filtres est que la somme de leur réponses fréquentielles est un filtre passe-tout 
généralement un simple filtre à retard dont le module de la réponse fréquentielle vaut~$1$. 

Dans la partie supérieure de la figure~\ref{fig:banc_de_filtre}, on retrouve à gauche les~$4$ filtres $\ww{H}_1(f)$, 
$\ww{H}_2(f)$, $\ww{H}_3(f)$ et $\ww{H}_4(f)$. Ces filtres reçoivent tous en entrée le signal $x(t)$, celui-ci est visualisé en haut à droite en noir. 
Le signal en bleu représenté juste en dessous est $y_1(t)$, c'est la sortie du filtre de réponse fréquentielle $\ww{H}_1(f)$. On observe que ce signal 
présente des variations de moindre amplitudes, c'est la conséquence de ce que $\ww{H}_1(f)$ est un passe-bas. 
Les signaux représentés en dessous en vert, rouge et cyan, sont notés $y_2(t), y_3(t), y_4(t)$. Ce sont respectivement les sorties des filtres
$\ww{H}_2(f)$, $\ww{H}_3(f)$ et $\ww{H}_4(f)$. On y retrouve des variations parfois significativement plus importantes. 
La décomposition du signal $x(t)$ en $4$ signaux $y_1(t), y_2(t), y_3(t), y_4(t)$ est appelé {\em analyse}, terme indiqué en bas à gauche de la figure~\ref{fig:banc_de_filtre}. Ces signaux, $y_1(t), y_2(t), y_3(t), y_4(t)$ sont ensuite additionnés pour former le signal visualisé en bas à droite en violet et noté 
$y_1(t)+y_2(t)+y_3(t)+y_4(t)$. Tel qu'on peut l'observer, ce signal est identique à $x(t)$. En réalité, ce dernier signal est généralement retardé par rapport 
à $x(t)$. Il est en effet impossible de réaliser une décomposition en banc de filtres avec des filtres causaux sans introduire un retard. 
La formation d'une reconstruction retardée de $x(t)$ à partir des signaux $y_1(t), y_2(t), y_3(t), y_4(t)$ s'appelle {\em synthèse}, ce qui est indiqué en 
bas du deuxième bloc. 

En regardant plus attentivement le bas de la figure~\ref{fig:banc_de_filtre}, on peut observer que les supports~\footnote{Par support, on entend ici l'intervalle sur lequel une fonction ici la réponse fréquentielle est non nulle.} des réponses 
fréquentielles des différents filtres ne sont pas disjoints, on dit que ces filtres se chevauchent. En fait l'allure même du signal $y_1(t)$ avec ces variations atténuées mais existantes laisse penser qu'il y a probablement un chevauchement assez important. Et en effet la notion de banc de filtre 
n'est pas du tout contradictoire avec un chevauchement même assez important. 
Pour la suite de ce document et pour plus de simplicité, on va considérer des bancs de filtres sans chevauchement où les réponses
fréquentielles sont en fait des portes définies par $\1_{[f_1,f_2]}(f)$. 

On dit qu'un banc de filtres suit une échelle linéaire lorsque les intervalles associés aux différentes portes caractérisant les réponses fréquentielles 
des filtres $\ww{H}_m(f)$ sont de longueur identiques. 
\beqn\boxed{
[f_{\min},f_{\max}]=\bigcup_{m}[f_m,f_{m+1}]\quad\mbox{où}\quad 
\left \{ \begin{array}{l}
f_{\min}=f_1,\,\,f_{\max}=f_{M+1}\\[0.3cm]
f_m=f_{\min}+(m-1)\frac{f_{\max}-f_{\min}}{M}\\[0.3cm]
\ww{H}_m(f)=\1_{[f_m,f_{m+1}]}(f)
\end{array}
\right. 
}
\eeqn

\begin{figure}
\begin{center}
\begin{tabular}{cc}
\includegraphics[width=0.5\linewidth]{fig9a.png}&
 \includegraphics[width=0.5\linewidth]{fig9b.png}
\end{tabular}
\end{center}
\caption{\`A gauche~: les courbes $\widehat{H}_m(f)$ en fonction de $f$ pour $m\in\{1,\ldots,8\}$ sont superposées
sur un même graphe.
 \`A droite~: ces courbes ont chacune leur abscisse.}
\label{fig9}
\end{figure}

La sensibilité de l'oreille humaine vis-à-vis de la décomposition fréquentielle d'un son et la façon dont les sons sont produits 
par les organes humains amènent à choisir pour les intervalles caractérisant les filtres $\ww{H}_m(f)$ une échelle logarithmique. 
Ce terme d'échelle logarithmique signifie que les intervalles sont de longueurs {\em croissantes} et que les bornes des ces intervalles 
suivent une loi {\em géométriques}. 
\beqn\boxed{
[f_{\min},f_{\max}]=\bigcup_{m}[f_m,f_{m+1}]\quad\mbox{où}\quad 
\left \{ \begin{array}{l}
f_{\min}=f_1,\,\,f_{\max}=f_{M+1}\\[0.3cm]
f_m=f_{\min}\left (\frac{f_{\max}}{f_{\min}}\right)^{\frac{m-1}{M}}\\[0.3cm]
%r=e^{\frac{\ln(f_{\max})-\ln(f_{\min})}{M}}=\left (\frac{f_{\max}}{f_{\min}}\right)^{\frac{1}{M}}\\[0.3cm]
\ww{H}_m(f)=\1_{[f_m,f_{m+1}]}(f)
\end{array}
\right. 
}
\eeqn

En pratique pour un banc de filtre suivant une échelle linéaire, on peut choisir $f_{\min}=0$ et $f_{\max}=\frac{f_e}{2}$, 
et pour une échelle logarithmique, il faut que $f_{\min}>0$, on peut choisir $f_{\min}=\frac{1}{T_K}$ et $f_{\max}=\frac{f_e}{2}$,
$T$ étant la durée de la trame.  

La figure~\ref{fig9} montre les réponses fréquentielles de huit filtres $\ww{H}_m$ qui suivent une échelle logarithmique, à gauche 
en les superposant sur un même graphe 2D et à droite en mettant chaque courbe le long d'un axe différent. 

\begin{figure}
\begin{center}
\begin{tabular}{cc}
\includegraphics[width=0.5\linewidth]{fig10a.png} &\includegraphics[width=0.5\linewidth]{fig10b.png}
\end{tabular}
\end{center}
\caption{\`A gauche~: superposition de l'évolution des descripteurs en fonction du temps. Chaque courbe
est associée à un filtre en particulier dont la légende indique la fréquence centrale associée à ce filtre.
\`A droite~: représentation séparée de l'évolution de chaque descripteur en fonction du temps.Dans les 
deux graphes, l'échelle en temps indique les instants associés aux milieux de chaque trame.}
\label{fig10}
\end{figure}

La figure~\ref{fig10} représente un exemple de représentation de ce descripteur temps-fréquence, 
il s'agit à gauche et à droite des courbes qui dans la figure~\ref{fig9} sont appelées $y_1(t), y_2(t), y_3(t), 
y_4(t)$. La différence est qu'ici il y en a $5$ et que les filtres utilisés ici ne se chevauchent pas. 
On observe des variations d'amplitudes plus faibles pour les quatre  premières 
par rapport à la dernière associées au fréquences plus élevées. 
Cependant il est significatif que la courbe bleue foncée, associée au filtre passe-bas et située au milieu sur le graphe de gauche et en 
haut à gauche sur le graphe de droite, a des variations qui sont d'une amplitude assez significatives, là 
on aurait pu s'attendre à des variations moins importantes. Cela traduit le fait que le signal 
sonore étudié présente des variations temporelles importantes d'une trame à une autre. 

Ces bancs de filtres servent à définir des descripteurs, un par filtre du banc de filtre.
De multiples descripteurs sont proposés dans la littérature scientifique. 
On aurait pu s'attendre à définir un descripteur comme la puissance sur une portion du signal en 
sortie du filtre $\ww{H}_m(f)$
autour de l'instant $t$.
\beqn\label{eq:desc_bf}
\boxed{
D_m(t)=\frac{1}{T}{\int_{-\frac{T}{2}}^{\frac{T}{2}} |h_m(\tau)\ast x_t(\tau)|^2\,d\tau}
\quad \mbox{ où }\quad \left \{ \begin{array}{l}
h_m(\tau)\mbox{ est la réponse impulsionnelle du filtre }\ww{H}_m(f)\\[0.3cm]
x_t(\tau)=x(\tau+t)\1_{\left [-\frac{T}{2},\frac{T}{2}\right]}(\tau)
\end{array}
\right . 
}
\eeqn

Mais comme la perception de l'intensité sonore est mieux corrélée à une intensité mesurée en décibel et donc 
suivant une échelle logarithmique vis-à-vis de la puissance, il convient d'ajouter un logarithme dans l'équation~(\ref{eq:desc_bf}).
La littérature scientifique a fait le choix d'utiliser un autre descripteur dont une version en temps continu serait 
\beqn
\sm{D\_LOG}_m(t)=\frac{1}{f_{m+1}-f_m}\,{\int_{f_m}^{f_{m+1}} 10\log_{10} \left |\ww{H}_m(f) \ww{X}_t(f)\right|^2\,df}
\eeqn
Et en pratique, le descripteur utilisé, dépend de deux paramètres, $m$ pour le filtre et par 
suite la fréquence associée à ce filtre, et $k$ pour la trame considérée. 

Le descripteur utilisé dans les travaux pratiques 
a pour nom {\tt LOG\_MAG\_FB\_LOG}~\footnote{La signification du nom se retrouve en lisant 
l'expression de droite à gauche. {\tt LOG} en dernier signifie qu'on considère une échelle logarithme, puis 
que cette échelle permet de définir un banc de filtre ({\em filter bank}), qu'on calcule ensuite le module ({\em magnitude}) 
et qu'avant de considérer la moyenne on considère le logarithme des modules.}

En pratique, le descripteur est ainsi défini.
\beqn
\boxed{
\sm{LOG\_MAG\_FB\_LOG}(m,k)=
\frac{1}{\left |\bb{L}_m\right |}
{\sum_{l\in \bb{L}_m} 10\log_{10}\left |\widehat{H}_{m,l}\widehat{X}_{k,l}\right|^2}
}
\eeqn
où $\bb{L}_m$ désigne les indices $l$ pour lesquels $\widehat{H}_{m}\left(\frac{lf_e}{N_K}\right)$ est non-nul, 
ce sont a priori les indices $l$ pour lesquels la fréquence $\frac{lf_e}{N_K}$ sont contenus dans 
$\left [f_m,f_{m+1}\right]$. 
$|\bb{L}_m|$ désigne le nombre d'indices $l$ contenus dans $\bb{L}_m$. 

Remarquons que le fait de modifier un descripteur en le multipliant par une certaine constante ou 
en lui ajoutant une constante n'a aucune incidence sur la classification qui en résulte. 


%\section{Conclusion}

D'autres suggestions de descripteurs pour la reconnaissance de la parole se trouvent dans~\cite{Rabiner93}.


\include{annexe_son}


==> sedT10YmQ <==

\newcommand{\msm}{$\mbox{m}.\mbox{s}^{-1}$}
\newcommand{\de}{{({\mbox{\small de}})}}
\newcommand{\moy}{{({ \mbox{\small moy})}}}
\newcommand{\der}{{({ \mbox{\small fin}})}}
\newcommand{\ce}{{({ \mbox{\small ce}})}}
\newcommand{\PMCT}{{\mbox{PMCT}}}
\newcommand{\arr}[1]{\rotatebox[origin=c]{#1}{$\xrightarrow{\hspace{1cm}}$}}
\newcommand{\fr}[1]{\framebox{#1}}
\newcommand{\bz}{{\mathbf z}}
\newcommand{\deux}{{\text{\tiny{|2}}}}     


\DeclareMathOperator{\OA}{OA}

\title{
Introduction à la reconnaissance de la parole  \\
}
\author{{\small Gabriel Dauphin}}


\begin{document}




%\pagenumbering{Alph}

%\pagenumbering{arabic}

\maketitle
\tableofcontents


\chapter*{Introduction}

Ce cours présente un ensemble de techniques qui sont utilisées en travaux pratiques 
pour distinguer les sons correspondant aux mots {\tt un}, {\tt deux} et {\tt trois}. 
Ces techniques utilisent la notion de description temps-fréquence qui est implicite dans la 
décomposition d'un son en trames, explicite dans la notion de {\tt spectrogramme} et qui est 
utilisée dans les différents descripteurs présentés dans le chapitre~\ref{ch:desc}.
Le chapitre~\ref{ch:traitement_son} a pour objectif de décrire la façon des sons sont représentées, cela amène 
à décrire brièvement les organes humains de la perception et le prétraitement qui est appliqué 
aux données associées aux sons. 
Le chapitre~\ref{ch:classification_par_descripteurs} a pour objectif de présenter la classification, à savoir son objectif, la façon dont on l'évalue et 
la manière dont elle utilise des valeurs calculées pour chaque son  que l'on appelle ici {\em descripteur}. 
Le chapitre~\ref{ch:desc} présente différentes techniques permettant de calculer les valeurs de descripteurs à partir des données 
associés aux sons. Cela amène à décrire brièvement les organes humains de la génération d'un son car cela explique 
l'intérêt porté à l'utilisation d'une description fréquentielle de portions de signaux temporels. 

En tant que document de cours, il a pour objectif de préciser les notions à connaître. Les notions 
à connaître le plus précisément sont la compréhension et la connaissance des {\em formules encadrées}, la compréhension 
des {\em graphiques et schémas} présentés et la connaissance et la signification des {\em termes techniques}. 





\chapter{Représentation d'un son}
\label{ch:traitement_son}

Pour décrire et discuter de la façon dont les sons sont représentées, la 
section~\ref{sec:questce_quun_son} discute de ce qu'est physiquement un son et donne 
une brève description des organes humains utilisées pour la perception d'un son. 
La section~\ref{sec:son_temps} rappelle comment le traitement numérique du signal permet 
de représenter un son.
La section~\ref{sec:N:son_trames} montre une façon un peu différente de représenter le son au moyens 
de {\em trames}, c'est-à-dire de petites portions du signal sonore. 
La section~\ref{sec:detection_silence} montre une façon simplifiée de détecter les phases de silence et de paroles, 
il se trouve que ceci était un des objectifs de ce cours. Cette détection est utilisée pour réaliser un 
prétraitement permettant d'améliorer la performance de la classification. 
La section~\ref{sec:implementation} donne quelques indications sur la façon dont les techniques proposées sont implémentées
dans les travaux pratiques qui illustre ce cours. 



\section{Qu'est-ce qu'un son~?}
\label{sec:questce_quun_son}


La section~\ref{ssec:model_physique} présente une description du son en tant qu'onde sonore se propageant 
dans l'air. 
La section~\ref{ssec:oreille} présente une très brève description du fonctionnement de l'oreille 
en tant qu'organe de perception des sons. 
La section~\ref{ssec:audibilite} présente des courbes d'audibilité, c'est-à-dire les seuils hauts et bas 
de perception du son. 


\subsection{Modélisation physique}
\label{ssec:model_physique}
Un son est généralement décrit comme plus ou moins aigu ou plus ou moins fort. Nous allons voir
que la première notion correspond à une fréquence et la deuxième à un niveau sonore. 

Le son est une variation de la pression de l'air.~\footnote{Un son peut aussi se propager à travers d'autres matériaux et dans ce cas 
c'est le matériau traversé qui se met à vibrer, en revanche le son ne peut pas se propager à travers le vide.}
Cette variation se propage sous la forme d'une onde. Une modélisation sphérique de cette onde est décrite par 
\beqn\label{eq:propag_onde}
P(r,t)=P_0+\frac{1}{r}\left [g_1(t-\frac{r}{c})+g_2(t+\frac{r}{c})\right ]
\eeqn
\begin{itemize}
\item $P_0$ est la pression atmosphérique moyenne. L'unité dans laquelle elle s'exprime est le Pa (Pascal). La pression de l'air est environ $10^5$Pa.
\item $r$ est la distance en mètres (m) entre le point où on mesure la pression et la  source de ce signal sonore. 
\item $t$ est l'instant en secondes~(s) pour lequel on mesure la pression $P(r,t)$. 
\item $c$ est la vitesse ($\mbox{m}.\mbox{s}^{-1}$) de propagation du son à travers l'air. C'est environ de $340$\msm. 
\item $g_1$ et $g_2$ peuvent a priori être des fonctions quelconques. Pour modéliser la propagation d'un signal sonore, on 
considère $g_2=0$ et pour un son stationnaire par exemple dans une caisse de résonnance, $g_1$ et $g_2$ sont similaires. 
\end{itemize}

Pour modéliser une note de musique qui dure un temps infini, on utilise 
\beqn
\boxed{
g_1(\tau)=\cos(2\pi f_0\tau)
}
\eeqn
Cette note est caractérisée par sa fréquence $f_0$ en Hz. 
En effet, avec cette modélisation on observe que $P(r,t+\frac{1}{f_0})=P(r,t)$, 
c'est-à-dire qu'en chaque point la pression évolue dans le temps avec une périodicité de $\frac{1}{f_0}$. 
{\small 
\beqns
P(r,t+\frac{1}{f_0})=P_0+\frac{1}{r}\cos(2\pi f_0(t+\frac{1}{f_0}-\frac{r}{c}))
=P_0+\frac{1}{r}\cos(2\pi f_0(t-\frac{r}{c}))=P(r,t)
\eeqns
}
Et $f_0$ est reliée à une longueur d'onde notée $\lambda_0$ mesurée en mètres.
\beqn\label{eq:long_onde}
\boxed{
\lambda =\frac{c}{f_0}
}
\eeqn
Ceci traduit une évolution quasi-périodique du signal dans l'espace $P(r+\lambda,t)\approx P(r,t)$. 
{\small 
\beqns
P(r+\lambda,t)=P_0+\frac{1}{r+\lambda}\cos(2\pi f_0(t-\frac{r}{c}-\frac{\lambda}{c}))
=P_0+\frac{1}{r+\lambda}\cos(2\pi f_0(t-\frac{r}{c}))\approx P(r,t)
\eeqns
}
\`A l'oreille, ce son apparaît comme une note de musique. Il s'agit d'un La lorsque $f_0=440$Hz. 
Cette fréquence est donc liée au caractère plus ou moins aigu du son. 

L'intensité sonore d'un son correspond au produit de la surpression par la vitesse. Dans le cadre de ce cours, 
on considère qu'il s'agit du carré de la partie variable de la pression. 
\beqns
I=\left (P(r,t)-P_0\right )^2
\eeqns
Cette intensité sonore est en Watt par mètres carrés ($\mbox{W}.\mbox{m}^{-2}$).
Dans le cadre de ce cours, on attache de l'importance au fait que cette intensité sonore est proportionnelle à $\frac{1}{r^2}$. 
\beqn
\boxed{
I=\frac{I_e}{r^2}
}
\eeqn
$I_e$ étant une quantité inconnue à estimer. 
Aussi lorsqu'on s'éloigne de la source en doublant la distance, l'intensité sonore est divisée par $4$. 

On appelle niveau sonore, le fait d'utiliser une échelle en décibel pour mesurer l'intensité sonore. 
\beqn\label{eq:N:niveau_sonore}
\boxed{
L=10\log_{10}\left (\frac{I}{I_0}\right )
}
\eeqn
où $I_0$ est une intensité sonore de référence. On peut remarquer que dans l'équation~(\ref{eq:N:niveau_sonore}), 
l'échelle en décibel n'est pas calculé avec un facteur multiplicatif de $20$ mais de $10$, parce que l'intensité sonore est 
déjà un terme carré. Et en effet lorsqu'on s'éloigne d'une source sonore en multipliant par deux la distance, 
le niveau sonore est diminué de $10\log_{10}(4)=6$dB.~\footnote{C'est en effet la même diminution que pour 
le rapport signal sur bruit, si on divisait par deux le bruit sans modifier le signal source.}

\subsection{Fonctionnement schématique de l'oreille}
\label{ssec:oreille}

\begin{figure}
\begin{center}
\begin{tabular}{c}
\includegraphics[width=0.5\linewidth]{oreille.png}
\end{tabular}
\end{center}
\caption{Schéma détaillé de l'oreille.}
\label{fig:N:oreille}
\end{figure}
	

La figure~\ref{fig:N:oreille} (extraite d'une publication) 
représente un schéma détaillé de l'oreille. Schématiquement, le son s'introduit dans le conduit auditif, 
fait vibrer le tympan qui actionne le marteau, l'enclume et l'étrier qui à son tour fait vibrer le liquide présent dans la cochlée. 
Cette cochlée est tapissée de cellules ciliées qui transmettent les vibrations vers des nerfs auditifs. Les cellules au début 
de la cochlée sont sensibles aux sons aigus tandis que celles en fin de cochlée sont sensibles aux sons graves. 

\subsection{Courbes d'audibilité humaine}
\label{ssec:audibilite}

\begin{figure}
\begin{center}
\begin{tabular}{c}
\includegraphics[width=0.5\linewidth]{courbe_audibilite.png}
\end{tabular}
\end{center}
\caption{Courbe d'audibilité humaine.}
\label{fig:N:courbe_audibilite}
\end{figure}
	
Dans la figure~\ref{fig:N:courbe_audibilite} (extraite d'une publication), l'échelle des ordonnées est le niveau sonore d'un son écouté. L'échelle 
des abscisses est une échelle de fréquences (Hz) mais avec une distribution logarithmique. \`A gauche ce sont les infrasons qui
correspondent aux sons qu'on ne peut entendre parce que leur fréquence est trop basse. \`A droite ce sont les ultrasons 
qu'on ne peut pas non plus entendre parce que leur fréquence est trop haute. Entre ces deux fréquences, il y a deux courbes, 
si le niveau sonore d'un son est supérieur à la limite donnée par la courbe inférieure alors on peut l'entendre et s'il 
est supérieur à la limite donnée par la courbe supérieure alors ce son peut abîmer l'oreille. 
Ces courbes sont obtenues en expérimentant sur un grand nombre de patients, elles indiquent un sensibilité moyenne, mais 
il y a en réalité des différences importantes d'un individu à un autre. 
Ces courbes nous amènent à affirmer qu'une assez grande partie de l'information sonore est obtenue en ne considérant 
que les fréquences inférieures à $4$kHz et qu'a priori la totalité de l'information sonore est obtenue en 
ne considérant que les fréquences inférieures à $20$kHz. 


\section{Représentation temporelle d'un son}
\label{sec:son_temps}


\begin{figure}
\begin{center}
\begin{tabular}{c}
\includegraphics[width=0.5\linewidth]{son_temps.png}
\end{tabular}
\end{center}
\caption{Représentation temporelle du signal sonore.}
\label{fig:N:son_temps}
\end{figure}
	
	
En tant qu'onde sonore, un son est un signal temps continu à valeurs continus. Mais lorsqu'il est 
converti en signal électrique avec un capteur acoustique appelé microphone puis converti en signal numérique avec 
échantillonnage et quantification, le signal devient temps discret. 
Du fait du critère de Shannon-Nyquist, la fréquence d'échantillonnage $f_e$ est entre $40$kHz et $50$kHz (en général 
$44.1$kHz mais, 
elle peut parfois être de $8$kHz. Le signal est souvent quantifié sur $8$ bits, mais cela peut être $10$ ou $12$ bits. 
Le signal échantillonné est noté $x_n$, chaque indique $n$ correspondant à un instant $t_n=nT_e$ où $T_e=\frac{1}{f_e}$.
La figure~\ref{fig:N:son_temps} (extraite d'une publication), indique l'évolution au cours du temps de l'intensité sonore. 
En ordonnée, il n'y a pas d'unité, c'est a priori une fraction de la valeur maximale. Mais le carré du signal est proportionnel à l'intensité sonore. 
Le signal représenté est celui obtenu en enregistrant la phrase {\em Le metteur en scène termine le scénario.} 



On appelle {\em durée} du signal, le temps qui s'écoule entre le début 
du signal sonore et la fin. Cette durée est égale à $NT_e$ où ici $N$ est 
le nombre d'échantillons~\footnote{\'Etant donné 
la valeur de $f_e$, il est tout à fait satisfaisant d'approcher cette durée 
à un multiple de $T_e$.} représenté sur la figure~\ref{fig:N:son_temps}. 
\'Etant donné la valeur élevée de $f_e$, on a en fait un très grand nombre d'échantillons, 
bien plus qu'il n'est possible de distinguer à l'oeil en observant la figure. L'allure générale permet aussi de distinguer les
 moments où il y a du silence, des moments où 
il y a un signal sonore important~: le silence correspond à des valeurs très faibles en valeur absolues et le signal sonore important correspond à des 
valeurs importantes du signal. 
Comme chaque intervalle de temps dans le graphe correspond aussi à un intervalle de 
temps durant lequel un son est prononcé, il est possible de faire correspondre chaque syllabe à un morceau du signal. On peut ainsi visualiser pour certaines sons des particularités, le premier {\em t} et les deux {\em s} correspondent à des parties très foncées du graphe. 

Bref, cette représentation temporelle du signal suggère l'étude séparée de chaque morceau de signal correspondant à un son ou à une syllabe. Mais comme on ne connaît 
pas a priori quand commence et quand finit le son ou la syllabe, la 
section~\ref{sec:N:son_trames} montre que l'on découpe le signal en une succession
de trames. 

Les notations utilisées pour décrire l'ensemble du signal sont les suivantes. 
\begin{itemize}
\item $T$ durée du signal en secondes.
\item $N$ nombre total d'échantillons.
\item $t_n=nT_e$ échelle de temps du signal pour $n\in\{0\ldots N-1\}$. 
\end{itemize}
On a la relation entre durée du signal et période d'échantillonnage. 
\beqn
\boxed{
T=NT_e
}
\eeqn
On a aussi l'échantillonnage du signal.
\beqn
\boxed{
x_n=x(t_n)
}
\eeqn


Pour illustrer des notions traitement du signal, on s'interroge ici sur la façon 
de rendre un son plus grave au moyen d'un traitement numérique du vecteur $x_n$. 
\begin{itemize}
\item En diminuant $f_e$, le son est plus grave. 
Mais sa durée est aussi diminuée d'autant puisqu'elle est égale à $\frac{N}{f_e}$. 
\item Si on effectue un sur-échantillonnage tout en conservant la fréquence 
d'échantillonnage alors le son devient plus grave mais sa durée est 
augmentée d'autant. 
\item Si on effectue une modulation, c'est-à-dire qu'on multiplie le graphe
par une sinusoïde d'une certaine fréquence alors on déplace effectivement 
le son à la fois en le rendant plus aigu et plus grave. Si ce son a un spectre
très étroit alors il est possible de supprimer la composante aigüe ou la composante grave. Et la durée est alors inchangée.  
\end{itemize}


\section{Représentation du signal sonore en une succession de trames}
\label{sec:N:son_trames}

\subsection{Découpage en trames sans chevauchement}

\begin{figure}
\begin{center}
\begin{tabular}{c}
\includegraphics[width=0.8\linewidth]{son_trames_simples.png}
\end{tabular}
\end{center}
\caption{Découpage d'une sinusoïde en trames qui ne se chevauchent pas.}
\label{fig:N:son_trames_simples}
\end{figure}
	
La figure~\ref{fig:N:son_trames_simples} donne quatre représentation 
d'un même signal défini par 
\beqns
x_n=\sin(20\pi nT_e)
\eeqns
C'est le signal représenté en haut à gauche de cette figure où sur une seconde, il
y $10$ périodes de la sinusoïde qui sont répétées et où donc, la fréquence de la 
sinusoïde est de $10$Hz et la période $T=0.1$s. L'échelle des ordonnées est 
une fraction de l'amplitude maximale. L'échelle des abscisses est la seconde. 

Dans cet exemple, on découpe le signal d'une seconde en $10$ trames chacune 
dure ici $0.1$s. La figure en haut à droite représente chaque trame avec une couleur 
différente~: bleu pour la première trame, vert pour la deuxième, rouge pour la troisième, cyan pour la quatrième, violet pour la cinquième, etc...

Le graphe en bas à gauche est une autre représentation de ces trames. L'axe pointant vers la droite est le temps écoulé depuis le début de chaque trame. 
L'axe pointant vers la gauche et commençant à zéro au milieu indique le numéro 
de la trame considérée. L'axe vers le haut indique la valeur du signal pour la trame considérée à l'instant de la trame considérée. La valeur zéro est ici à mi-hauteur. Ici la couleur ne distingue plus les trames entre elles, elle dépend de la valeur prise par le signal. Dans cet exemple le signal est identique sur chaque trame, c'est pour cela qu'on retrouve exactement le même signal sur chaque courbe. 

La courbe en noir du graphe en bas à droite est la même que le graphe en haut à gauche, il s'agit du signal $x_n$ représenté en fonction du temps. Sur ce graphe, il y a en plus des traits horizontaux de couleurs et de hauteurs différentes
qui permettent d'identifier chaque trame. Ce sont ces traits qui permettent de lire 
les instants associés au début et à la fin de chaque trame en trouvant l'abscisse 
du début et de la fin du trait horizontal. 

\subsection{Notations pour définir les trames}

On utilise ici les notations suivantes. Ces notations ne sont pas 
universelles, il est donc nécessaire de les redéfinir quand on les utilise. 
\begin{itemize}
\item $K$ désigne le nombre de trames. 
\item $T_K$ est la durée d'une trame. 
\item $N_K$ est le nombre d'échantillons dans une trame, il est identique pour toutes les trames d'un même son.
\item $k\in \{0\ldots K-1\}$ est un indice qui identifie la trame. 
\item $t_k^\de$ instant associé au premier échantillon de la trame $k$.
\item $t_k^\der$ instant associé au dernier échantillon de la trame $k$. 
\item $t_k^\ce$ instant associé au centre de la trame $k$. 
\item $t_{k,n}$ échelle de temps associée à la trame $k$ donnant 
les instants associées aux échantillons $n=0$ jusqu'à $n=N_K-1$. 
\end{itemize}

Du fait qu'il n'y a pas de chevauchement, on a
\beqn\label{eq:N:T_K}
\boxed{
T_K=\frac{T}{K}\mbox{ et }N_K=\frac{N}{K}
}
\eeqn

D'une façon générale, le début, le centre et la fin d'une trame 
$k$
sont définies par
\beqn\label{eq:N:t_k_de}
\boxed{
\mbox{Pour }k\in\{0\ldots K-1\},\quad\left \{
\begin{array}{l}
t_k^\de=k\frac{T}{K}\\[0.2cm]
 t_k^\der=t_k^\de+T_K-T_e\\[0.2cm]
t_k^\ce=\frac{1}{2}\left (t_k^\de+t_k^\der\right )
\end{array}
\right. 
}\eeqn

Avec ces définitions et pour une trame $k$, on peut définir une échelle de temps et déterminer les valeurs du signal
\beqn\label{eq:N:ech_temps_trame}
\boxed{
\begin{array}{c}
\mbox{Pour }k\in\{0\ldots\}\mbox{ et }n\in \{0\ldots N_K-1\}\\[0.5cm]
t_{k,n}=t_k^\de+nT_e \mbox{ et }x_{k,n}=x(t_{k,n})=x\left[\frac{t_{k,n}}{T_e}\right ]
\end{array}
}
\eeqn
Dans la dernière expression en bas à droite de l'équation~(\ref{eq:N:ech_temps_trame}), l'expression entre crochet est un indice 
\beqns
n'=\frac{t_{k,n}}{T_e}=k\frac{N}{K}+n
\eeqns
et cet indice est utilisé pour retrouver dans le signal $x_n$ la valeur recherchée 
$x_{k,n}=x_{n'}$. 


\subsection{Découpage en trames avec chevauchement}

\begin{figure}
\begin{center}
\begin{tabular}{c}
\includegraphics[width=0.8\linewidth]{son_trames_chevauchement.png}
\end{tabular}
\end{center}
\caption{Découpage d'une sinusoïde en trames qui se chevauchent.}
\label{fig:N:son_trames_chevauchement}
\end{figure}


\`Etant donné un nombre total d'échantillons $N$, un nombre de trames $K$ et 
du choix de chevauchement utilisé, on a les deux propriétés suivantes. 
\begin{itemize}
\item Les instants de débuts des trames ne sont pas modifiées.
\beqn
\boxed{
t_k^\de=k\frac{T}{K}
}
\eeqn
\item La longueur des trames est augmenté d'un facteur $\frac{1}{1-\alpha}$. 
\beqn\label{eq:N:T_K_alpha}
\boxed{
T_K=\frac{T}{K}\frac{1}{1-\alpha}\mbox{ et }N_K=\frac{N}{K}\frac{1}{1-\alpha}
}
\eeqn
\item Hormis la première trame, toutes les trames partagent avec la précédente
$\alpha N_K$ échantillons. Et hormis la dernière trame, toutes les trames partagent avec la suivante $\alpha N_K$ échantillons. 
\end{itemize}


La dernière affirmation se calcule ainsi pour $k\in\{0\ldots K-1\}$
\beqns
t_k^\der-t_{k+1}^\de+T_e=\left (k\frac{T}{K}+\frac{T}{K}\frac{1}{1-\alpha}-T_e\right ) -(k+1)\frac{T}{K}+T_e=\frac{T}{K}\left (\frac{1}{1-\alpha}-1\right )
=\alpha T_K
\eeqns


Ainsi les équations (\ref{eq:N:t_k_de}) et (\ref{eq:N:ech_temps_trame})
ne sont pas modifiées quand on met un chevauchement. En revanche l'équation~(\ref{eq:N:T_K})
est remplacée par l'équation~(\ref{eq:N:T_K_alpha}).

Lors de l'implémentation, ces formules ont été un peu modifiées pour tenir 
compte de ce que le découpage en trames ne tombe pas exactement sur un échantillon 
et qu'il faut donc commencer à partir de l'échantillon le plus proche. 

\section{Signaux sonores et silences}
\label{sec:detection_silence}
\subsection{Puissance moyenne à court terme}
\label{ssec:PMCT}


\begin{figure}
\begin{center}
\begin{tabular}{c}
\includegraphics[width=0.8\linewidth]{son_puissance.png}
\end{tabular}
\end{center}
\caption{Signal temps discret représentant un signal sonore commençant et terminant par un silence.}
\label{fig:N:son_puissance}
\end{figure}

En traitement du signal, on définit une puissance moyenne qui évolue dans le temps
qui est appelée puissance moyenne à court terme. 
Cela se fait en introduisant une fenêtre notée $w_T$ qui est un signal temps 
continu de durée $T$ centré en zéro. 
La notion de fenêtre a déjà été présentée lors du cours sur la 
synthèse des filtres numérique à réponse impulsionnelle finie avec notamment la fenêtre rectangulaire et triangulaire. 
\`A temps continu, la fenêtre rectangulaire de largeur $T$ est ainsi définie.
\beqns
w_T(\tau)=\1_{\left [-\frac{T}{2},\frac{T}{2}\right]}(\tau)
\eeqns
La fenêtre triangulaire de largeur $T$ est ainsi définie.
\beqns
w'_T(\tau)=\left (1-\frac{2t}{T}\right)\1_{\left [-\frac{T}{2},\frac{T}{2}\right]}(\tau)
\eeqns
Ici la fenêtre est utilisée, non pour modifier une réponse impulsionnelle mais un signal, ici $x^2(t)$. L'action de la fenêtre 
porte sur l'intervalle de temps centré en $t$. Aussi elle est d'abord centrée en $t$ puis normalisée.
\beqns
w_T(\tau)\mapsto w_T(t-\tau)\mapsto \frac{1}{\int_\Rr w_T(t-\tau)\,d\tau}\,w_T(t-\tau)
\eeqns
Ainsi modifiée la fenêtre est ensuite multipliée par $x^2(\tau)$
\beqns
x^2(\tau)\mapsto x^2(\tau)\frac{1}{\int_\Rr w_T(t-\tau)\,d\tau}\,w_T(t-\tau)
\eeqns

Cette puissance moyenne à court terme, notée $\sm{PMCT}$~\footnote{{\tt PMCT}
est défini dans \cite{Camastra07} p.~41-42.}~\footnote{Une interprétation en terme d'énergie
existe dans page~3, section~2.1 dans~\cite{Peeters04}.}
 est 
\beqn\label{eq:PMCT_TC}
P(t)=\frac{{\int_\Rr {x^2(\tau)w_T(t-\tau)\,d\tau }}}{{\int_\Rr w_T(\tau)\,d\tau}}
\eeqn
Avec une fenêtre rectangulaire, $P(t)$ devient 
\beqn\label{eq:PMCT_TC_rect}
\boxed{
P(t)=\frac{1}{T}{\int_{t-\frac{T}{2}}^{t-\frac{T}{2}} x^2(\tau)\,d\tau}
}
\eeqn


Ici le découpage en trame du signal se prête justement à un calcul très similaire.
\begin{itemize}
\item $T$ est remplacée par la longueur de la trame $T_K$ qui compte $N_K$ échantillons. 
\item $t$ est remplacée par $t_k^\ce$, le milieu de la trame $k$ qui se trouve à peu près à l'échantillon $\frac{N_K}{2}$ de 
la trame $k$. 
\end{itemize} 
 Cela permet ainsi d'approcher la  discrétisation de l'équation~(\ref{eq:PMCT_TC}).
\beqn
\PMCT_k=\frac{{\sum_{n=0}^{N_K-1} x_k^2[n]w_{N_K}[n-\frac{N_K}{2}]}}{{\sum_{n=0}^{N_K-1} w_{N_K}[n-\frac{N_K}{2}]}}
\eeqn
où $w_{N_K}[n]$ est une fenêtre de support $\{-\frac{N_K}{2}\ldots \frac{N_K}{2}\}$ {\bf mais} avec des indices allant de $0$ à $N_K-1$.  

Avec une fenêtre rectangulaire, 
\beqn
\boxed{
\PMCT_k=\frac{1}{N_K}
{\sum_{n=0}^{N_K-1} x_k^2[n]}
}
\eeqn


\subsection{Détection du début et de la fin d'un signal sonore.}
\label{ssec:det_deb_fin_son}

La figure~\ref{fig:N:son_puissance} montre un exemple de signal sonore commençant et terminant par un silence. 
On souhaite dans cet exemple retrouver l'instant à partir duquel le signal sonore commence et l'instant auquel ce
 signal sonore s'arrête. 


On se donne un seuil, il est ici fixé à $10\%$ de la valeur maximale.
\beqn\label{eq:seuil}
\boxed{
s_e=\frac{1}{10}\max_k({\PMCT_k})
}
\eeqn
Ce seuil est utilisé pour déterminer deux numéros de trames~: $k^\de$ la première trame pour laquelle la puissance $\PMCT_k$ est supérieure 
$s_e$ et $k^\der$ la dernière  pour laquelle ceci est vrai. 
\beqn
\boxed{
k^{\de}=\underset{k}{\min}\,\{k|\,\PMCT_k>s_e\}
\mbox{ et }
k^{\der}=\underset{k}{\max}\,\{k|\,\PMCT_k>s_e\}
}
\eeqn
Les instants $t^\de$ et $t^\der$ associés au début et à la fin du signal sonore sont les centres des trames $k^\de$ et $k^\der$. 
\beqn
\boxed{
\left\{\begin{array}{l}
t^{\de}=t_{k}^{\ce}\mbox{ avec }k=k^{\de}\\[0.3cm]
t^{\der}=t_k^{\ce}\mbox{ avec }k=k^{\der}
\end{array}
\right . 
}
\eeqn
où $t_k^{\ce}$ désigne l'instant associé au centre de la trame $k$. 

\subsection{Normalisation d'un signal sonore}

La normalisation du signal a pour but de rendre comparable 
un son qui serait prononcé de façon forte et un son prononcé à voix plus basse. 
Cette normalisation consiste à imposer que la puissance moyenne soit fixe et en l'occurrence égale à $1$, mais 
cette étape se fait après avoir retiré les silences du signal.~\footnote{Si on effectuait cette normalisation du 
signal avant de retirer les silences, un son avec beaucoup de silences 
que l'on aurait normalisé  avec ses silences, aurait une 
puissance moyenne plus forte, une fois retirés les silences.}


Pour comparer les signaux, il est souhaitable que les signaux soient comparable en terme de puissance moyenne. Cette moyenne étant calculée sans considérer les silences. 
Pour obtenir que les signaux soient comparés, on effectue une {\em normalisation}, c'est-à-dire qu'on chacun des signaux par une valeur appropriée. 
Cette valeur est déterminée avec les étapes suivantes. 
\begin{itemize}
\item On utilise la technique de détection du début et de fin du signal sonore présentée en section~\ref{ssec:det_deb_fin_son}. 
\item On calcule la puissance moyenne en ne considérant que les trames qui se situent entre la première et la dernière des trames associées au signal sonore. 
On note $\bb{K}$ l'ensemble des trames où le son est plus fort que le seuil fixé par l'équation~(\ref{eq:seuil})
et $|\bb{K}|$ le nombre de ces trames. 
\beqns
\boxed{
P_\moy=\frac{1}{|\bb{K}|}{\sum\limits_{k\in \bb{K}} \sm{PMCT}_k}
}
\eeqns
\item La normalisation consiste à multiplier le signal par $\frac{1}{\sqrt{P_\moy}}$. 
\beqn
\boxed{
x_n\mapsto \frac{1}{\sqrt{P_\moy}} x_n
}
\eeqn
\end{itemize}


\section{Indications sur l'implémentation proposée}
\label{sec:implementation}

\begin{figure}
\begin{center}
\begin{tabular}{c}
\includegraphics[width=0.6\linewidth]{projet_son1.png}
\end{tabular}
\end{center}
\caption{Organisation des données dans l'implémentation}
\label{fig:N:projet_son1}
\end{figure}

Dans la simulation proposée, le répertoire principal est subdivisé en {\tt prg} contenant les programmes Matlab (fichiers {\tt .m} ou {\tt .p}) et {\tt donnee} qui contient 
les fichiers audio répartis en trois répertoires  {\tt un},  {\tt deux } et {\tt trois}. 
Cette organisation est schématisée sur la figure~\ref{fig:N:projet_son1}.


\chapter{Obtenir une classification grâce à des descripteurs}
\label{ch:classification_par_descripteurs}

L'objectif au cours de la séance de TP correspondante est de classer les sons à partir de descripteurs. Un descripteur peut 
soit être une valeur pour l'ensemble du signal, soit un ensemble de valeurs, une pour chaque trame.
On suppose dans cette partie qu'on dispose d'un certain nombre de descripteurs qui nous donnent des valeurs, une valeur par trame. 
La classification des sons est alors exposée en trois parties. 
La section~\ref{sec:distance_entre_sons} permet à partir de descripteurs d'évaluer numériquement 
une similarité entre deux sons. En fait on parle plutôt de distance entre sons, la distance correspondant ici à un défaut de similarité. 
une distance entre deux sons. 
La section~\ref{sec:knn} permet à partir de distances entre sons de prédire l'identité d'un son quelconque, 
c'est-à-dire s'il ressemble plus à un son de type {\tt un}, {\tt deux} ou {\tt trois}. 
Enfin la section~\ref{sec:evaluation_classification} montre comment on évalue généralement un classifieur. 


%\fbox{\begin{minipage}{0.8\linewidth}
%\imp
%Des descripteurs sont disponibles en utilisant la fonction {\tt traitement}. 
%\end{minipage}}

\section{Calcul d'une distance entre deux sons}
\label{sec:distance_entre_sons}



\begin{figure}
\begin{center}
\begin{tabular}{c}
\begin{tikzpicture}
[node distance = 10mm,thick, main/.style = {draw, circle},
  rect/.style={draw,rectangle,fill=green!50},rect_y/.style={draw,rectangle},
  minimum size=0mm]
	\node (H1) {};
	\node (L1)[below of=H1] {};
	\node (L11) [below of=L1] {};
		\node (L12) [below of=L11] {};
		\node (L13) [below of=L12] {};
		\node (L14) [below of=L13] {};
	  \node (sons) [right of=L1] {sons}; 
		\node[rect_y] (xn) [below of=sons] {$x_a[n]$};   
		\node (xmn) [below of=xn] {};  
		\node[rect_y] (xpn) [below of=xmn] {$x_b[n]$};  
		\node (L2) [right of=sons] {};
	  \node (trames) [right of=L2] {trames}; 
		\node[rect_y] (xkn) [below of=trames] {$x_a[k,n]$};   
		\node (xmkn) [below of=xkn] {};  
		\node[rect_y] (xpkn) [below of=xmkn] {$x_b[k,n]$};  
		\node (L3) [right of=trames] {};
		\node (sans_silence) [right of=L3] {$\begin{array}{c}\mbox{sans le}\\ \mbox{silence}\end{array}$}; 
		\node[rect_y] (xkn1) [below of=sans_silence] {$x_a[k,n]$};   
		\node (xmkn1) [below of=xkn1] {};  
		\node[rect_y] (xpkn1) [below of=xmkn1] {$x_b[k,n]$};  
		\node (L4) [right of=sans_silence] {};
		\node (normalisation) [right of=L4] {$\begin{array}{c}\mbox{normali-}\\ \mbox{sation}\end{array}$}; 
		\node[rect_y] (xkn2) [below of=normalisation] {$x_a[k,n]$};   
		\node (xmkn2) [below of=xkn2] {};  
		\node[rect_y] (xpkn2) [below of=xmkn2] {$x_b[k,n]$};  
		\node (L5) [right of=normalisation] {};
		\node (H5) [above of=L5] {};
		\node (L51) [below of=L5] {};
		\node (L52) [below of=L51] {};
		\node (L53) [below of=L52] {};
		\node (L54) [below of=L53] {};
		\node (descripteur) [right of=L5] {$\begin{array}{c}\mbox{calcul des}\\ \mbox{descripteurs}\end{array}$}; 
		\node[rect_y] (zkj) [below of=descripteur] {$z_{a}^{(j)}[k]$};   
		\node (zmkj) [below of=zkj] {};  
		\node[rect_y] (zpkj) [below of=zmkj] {${z}_{b}^{(j)}[k]$};  		
		\node (L6) [right of=descripteur] {};
		\node (distance) [right of=L6] {$\begin{array}{c}\mbox{calcul de la}\\ \mbox{distance}\end{array}$}; 
		\node (L67l) [below of=distance] {}; 
		\node[rect_y] (d) [below of=L67l] {$d(x_a,x_b)$};   
		
		\begin{scope}[-latex]
\draw[thick,->,blue] (xn) to   (xkn);
\draw[thick,->,blue] (xkn) to   (xkn1);
\draw[thick,->,blue] (xkn1) to   (xkn2);
\draw[thick,->,green] (xkn2) to   (zkj);
\draw[thick,->,blue] (xpn) to   (xpkn);
\draw[thick,->,blue] (xpkn) to   (xpkn1);
\draw[thick,->,blue] (xpkn1) to   (xpkn2);
\draw[thick,->,green] (xpkn2) to   (zpkj);
\draw[thick,->,red] (zpkj) to   (d);
\draw[thick,->,red] (zkj) to   (d);
\draw[gray,dashed,-] (H1) to   (H5);
\draw[gray,dashed,-] (H5) to   (L54);
\draw[gray,dashed,-] (L14) to   (L54);
\draw[gray,dashed,-] (H1) to   (L14);
\end{scope}
\end{tikzpicture}
\end{tabular}
\end{center}
\caption{Schéma décrivant la mise en oeuvre du calcul de la distance entre deux sons noté $x$ et $x'$. 
La partie encadrée en pointillé est la préparation des signaux
transformant $x_a[n]$ et $x_b[n]$ en $x_a[k,n]$ et $x_b[k,n]$, $n$ étant dans $x_a[n]$ et $x_b[n]$ l'indice de l'échantillon pour  l'ensemble du son 
et pour $x_a[k,n]$ et $x_b[k,n]$, l'indice dans la trame $k$. La lettre $j$ désigne un type de descripteur et celui-ci est calculé pour les deux sons et pour chaque 
%trame $k$, les valeurs obtenues sont rangées dans $z_{k}^{(j)}$ et ${z'}_{k}^{(j)}$. 
$d(x_a,x_b)$ désigne la valeur de la distance entre les deux sons.  }
\label{fig:dist_sons}
\end{figure}
 %\beqns
%\begin{array}{c@{}c@{}c@{}c@{}c@{}c@{}c}
%\mbox{sons} &  & \mbox{trames} && \hspace{-1cm}\mbox{descripteurs}\hspace{-1cm} && \mbox{distance}\\[0.3cm]
%\fr{$x_n$} &\arr{0}& \fr{$x_{k,n}$}& \arr{0}& \fr{$z_{k,j}$}\\[-0.4cm]
%&& && &\arr{-30} \\[-0.3cm]
%&& && &  &\fr{d(x,x')}\\[-0.3cm]
%&& && &\arr{+30} \\[-0.4cm]
%\fr{$x'_n$} &\arr{0}& \fr{$x'_{k,n}$}& \arr{0}& \fr{$z'_{k,j}$}\\[0.3cm]
%\end{array}
%\eeqns


La figure~\ref{fig:dist_sons} schématise la façon de calculer une distance (i.e. une non-similarité) entre deux sons. 
La partie encadrée en pointillé figure la préparation des signaux avec les tâches suivantes. 

\begin{minipage}{0.95\linewidth}
\begin{itemize}
\item Chaque signal sonore est décrit avec $x_a[n]$ et $x_b[n]$ par un signal temps discret échantillonné à la même fréquence d'échantillonnage, mais 
pas forcément de même durée. 
\item Chaque signal est découpé en trames, de longueur et de chevauchement identique, le nombre de trames est a priori différent d'un signal à l'autre. 
\item Les trames silencieuses en début et fin de son sont retirées. 
\item Les valeurs des signaux au sein de chaque trames sont normalisées globalement au niveau du son, c'est-à-dire que si une trame est 
en moyenne deux fois plus forte qu'une autre trame du même son, elle reste deux fois plus forte après la normalisation. 
Par contre quand on compare deux sons, le fait de multiplier par deux toutes les valeurs d'un des deux sons, ne modifie pas la distance entre les 
deux sons. 
\end{itemize}
\end{minipage}

On rajoute les notations suivantes~: 

\begin{minipage}{0.95\linewidth}
\begin{itemize}
\item $x_a$ et~$x_b$ désignent les sons~$a$ et~$b$. 
\item $x_a[n]$ et~$x_b[n]$ désignent les~$N_a$ et~$N_b$ valeurs des signaux associés aux sons~$a$ et~$b$. 
\item $x_a[kn]$ et~$x_b[kn]$ désignent les~$N_k$ valeurs des sons $a$ et $b$ pour la trame~$k$, c'est l'équivalent pour le son~$a$ de ce qui était noté précédemment~$x_k[n]$. 
\item $J$ désigne le nombre total de descripteur. 
\item $j\in\{1\ldots J\}$ désigne un descripteur spécifique. $\PMCT$ est un exemple de descripteur, les autres seront décrits dans le 
chapitre~\ref{ch:desc}. 
\item ${z}_a^{(j)}[k]$ et~${z}_b^{(j)}[k]$  désigne la valeur du descripteur~$j$ pour la trame~$k$ et les sons~$a$ et~$b$. 
\end{itemize}
\end{minipage}

Les calculs figurés par les flèches vertes joignant $x_a[kn]$ et $x_b[kn]$ à  ${z}_a^{(j)}[k]$ et ${z}^{(j)}_b[k]$ correspondent aux 
calculs des valeurs des descripteurs, 
Les flèches rouges joignant  ${z}_{a}^{(j)}[k]$ et ${z}_{b}^{(j)}[k]$ à $d(x_a,x_b)$ figurent les calculs permettant d'évaluer la distance à partir 
des valeurs des descripteurs, trois techniques sont proposées dans cette section. 

\subsection{Les descripteurs par trames sont transformés en descripteurs par son}
\label{ssec:mu_sigma}
On rajoute ici un autre sens au mot descripteur. Précédemment, il s'agissait d'un descripteur par trame, ici il s'agit d'un descripteur 
pour l'ensemble d'un son. Ce descripteur est identifié par $j$ correspondant aux valeurs du descripteur par trame qui sont 
résumés dans une seule valeur. Ce descripteur est aussi identifié par la façon de faire ce résumé~: $\mu$ pour la moyenne, $\sigma$ 
pour l'écart-type, $\gamma_1$ et $\gamma_2$ pour les coefficients d'asymétrie et d'aplatissement.

Ces quatre descripteurs de sons sont calculés à partir des valeurs d'un descripteur obtenu pour chaque trame d'un son. 

\begin{minipage}{0.95\linewidth}
\begin{itemize}
\item La moyenne d'un descripteur $j$ est la moyenne des valeurs de $z_k^{(j)}$ pour chaque trame $k$. 
\beqn\label{eq:mu}
\boxed{
\mu^{(j)}=\frac{1}{K}{\sum_{k=0}^{K-1} z_k^{(j)}}
}
\eeqn
\item 
L'écart-type d'un descripteur $j$ est la racine carré de la moyenne des variances.
\beqn\label{eq:sigma}
\boxed{
\sigma^{(j)}=\sqrt{\frac{1}{K}{\sum_{k=1}^K \left (z_k^{(j)} -\mu^{(j)}\right)^2}}
}
\eeqn
\item Le coefficient d'asymétrie d'un descripteur $j$ est 
\beqn
\gamma_1^{(j)}=\frac{1}{(\sigma^{(j)})^3}{\frac{1}{K}{\sum_{k=1}^K \left (z_k^{(j)} -\mu^{(j)}\right)^3}}
\eeqn
\item Le coefficient d'aplatissement d'un descripteur $j$ est 
\beqn
\gamma_2^{(j)}=\frac{1}{(\sigma^{(j)})^4}{\frac{1}{K}{\sum_{k=1}^K \left (z_k^{(j)} -\mu^{(j)}\right)^4}}
\eeqn
\end{itemize}
 \end{minipage}

Ces quatre descripteur de sons permettent de définir différentes distances entre sons suivant ce qui est pris en compte. 
Par exemple en prenant en compte la moyenne et l'écart-type des descripteur $j\in\{1\ldots J\}$, on a la distance suivante~: 
\beqn
\boxed{
d(x_a,x_b)=\sqrt{{\sum_{j=1}^J \left( \mu_a^{(j)}-\mu_b^{(j)}\right )^2+\left( \sigma_a^{(j)}-\sigma_b^{(j)}\right )^2}}
}
\eeqn

\subsection{La distance entre deux sons est obtenue en comparant trame par trame, les valeurs des descripteurs.}
\label{ssec:dist_trames}

Les sons $a$ et $b$ n'ont pas a priori la même durée et donc pas le même nombre de trames. On note $\min(K_a,K_b)$ le nombre de trames du son 
le plus court. On définit la distance comme la moyenne des distances entre les descripteurs trame par trame. Cette distance est 
en fait la racine carré de la somme des carrés des différences. Chaque son est décrit par $J{\times}K_a$ et $J{\times}K_b$ valeurs, 
on arrive à la définition suivante. 
\beqn
\boxed{
d(x_a,x_b)=\sqrt{\frac{1}{\min(K_a,K_b)}
{\sum_{k=0}^{\min(K_a,K_b)-1}{\sum_{j=1}^J\left (z_a^{(j)}[k]-z_b^{(j)}[k]\right )^2}}}
}
\eeqn

Un important défaut de cette technique est qu'elle amène à considérer un son comme différent, lorsqu'il est prononcé avec une vitesse différente ou simplement une vitesse qui varie différemment. 

\subsection{La distance entre deux sons est obtenue en cherchant la déformation temporelle minimisant la différence entre les deux sons.}
\label{ssec:dist_def_temp}

\subsubsection{Notion de déformation temporelle dynamique }


\begin{figure}
\begin{center}
\begin{tabular}{cc}
\includegraphics[width=0.5\linewidth]{fig_def_temp1.png}
\includegraphics[width=0.5\linewidth]{fig_def_temp2.png}\\
\includegraphics[width=0.5\linewidth]{fig_def_temp4.png}
\includegraphics[width=0.5\linewidth]{fig_def_temp3.png}
\end{tabular}
\end{center}
\caption{Quatre déformations possibles d'un même signal sinusoïdal représenté sur les quatre figures en vert. 
Le temps est représenté sur l'axe horizontal et les valeurs des signaux sont représentées sur l'axe vertical. En haut à gauche, le signal bleu 
est perturbé par un bruit additif, en haut à droite, il est perturbé par une bruit additif de moindre ampleur ajouté à la fois sur les valeurs du signal 
et celles du temps~; en bas à gauche, il est perturbé par un bruit additif ajouté seulement sur les valeurs de temps~; en bas à droite, le bruit 
additif ajouté seulement sur les valeurs de temps est corrigé par le fait qu'un évènement postérieur à un autre évènement doit rester postérieur après 
la perturbation.}
\label{fig:def_temp_1}
\end{figure}

La figure~\ref{fig:def_temp_1} représente un même signal sinusoïdal colorié en vert $x_v(t)$ et 
différentes déformations de ce signal sinusoïdal, $x_b(t)$, colorées en 
bleu. 

Il est d'usage lorsqu'on évalue la distance entre deux courbes définies sur un même intervalle de temps $[0,T]$, de calculer la 
moyenne quadratique de la différence entre $x_v(t)$ et $x_b(t)$. 
\beqn
\boxed{
d_1(x_v,x_b)=\sqrt{\frac{1}{T}{\int_0^T \left(x_v(t)-x_b(t)\right )^2\,dt}}
}
\eeqn
Cette évaluation est souvent choisie pour sa simplicité, elle a une interprétation pertinente lorsque le signal déformé $x_b(t)$ resulte 
d'un bruit blanc gaussien centré additif, car dans ce cas $d_1(x_v,x_b)$ est une estimation de l'écart-type de cette gaussienne. Le graphe en haut à gauche 
de la figure~\ref{fig:def_temp_1} montre en bleu un signal déformé par un bruit blanc additif, on y observe que parfois la courbe bleue est au dessus 
de la courbe verte et parfois elle est en dessous. 

Il existe dans la littérature scientifique une technique permettant d'évaluer la distance avec les différences en hauteur entre les signaux mais
avec les distances euclidienne entre les courbes, c'est-à-dire pour chaque point de la courbe $x_b(t)$, on utilise la distance entre ce point et 
le point le plus proche de $x_v(t)$. Cette évaluation est pertinente lorsqu'on considère que la déformation de $x_b(t)$ résulte d'une part 
d'un variation de  la valeur du signal $x_b(t^b_n)-x_v(t^v_n)$ mais aussi une variation de la base de temps $t^b_n-t^v_n$. Le graphe en haut à droite est obtenu en ajoutant deux bruits blancs 
gaussiens centrés additifs indépendants sur les valeurs du signal et sur les instants associés à ces valeurs. 

Le graphe en bas à gauche est obtenu en ne modifiant que les bases de temps $t^b_n$ par rapport à $t^v_n$, il s'agit d'un bruit blanc gaussien centré 
additif. C'est-à-dire qu'on a l'égalité entre les valeurs des signaux $x_b$ et $x_v$ mais les valeurs ont lieu à des instants différents. 
\beqns
x_b(t^b_n)=x_v(t^v_n)
\eeqns
Sur ce graphe, la courbe bleue présente des boucles suggérant que le temps s'inverse parfois. Ceci n'est pas une modélisation réaliste. 

Le graphe en bas à droite est obtenu aussi en ne modifiant que les bases de temps $t^b_n$ par rapport à $t^v_n$, mais pour plus de réalisme, l'ordre des 
évènements est respecté, il n'y a donc plus de boucles.
\beqns
t^v_n\leq t^v_{n'}\quad\Rightarrow\quad t^b_n\leq t^b_{n'}
\eeqns
Concrètement, les variations de $t^b_n$ sont limitées par la contrainte que $t^b_{n}\leq t^b_{n+1}$ doit toujours être vrai. 
C'est ce type de  déformation du signal que l'on cherche à prendre en compte. Quand on prononce un son plus lentement pour plus rapidement ou 
avec une vitesse qui varie au cours de la prononciation du son, il s'agit du même son. La distance devrait théoriquement ne pas 
être sensible à ce type de déformation. 
On appelle cette déformation, une déformation temporelle dynamique.~\footnote{Cette notion est présentée en détail dans~\cite{Cassisi12}.} 


\subsubsection{Table d'indexation}

\begin{figure}
\begin{center}
\begin{tabular}{c}
\includegraphics[width=0.5\linewidth]{fig_7.png}
\end{tabular}
\end{center}
\caption{En vert et bleu, deux signaux sont définis sur des intervalles de temps différents $(t_n,x_n)$, $(t'_n,y_n)$.
En rouge, le signal $(t_n,x_n)$ est transformé par une table d'indexation en 
$(t'_{\Phi_{y}[n]},x_{\Phi_x[n]})$ de façon à approcher le signal $(t'_n,y_n)$.}
\label{fig7}
\end{figure}

La figure~\ref{fig7} illustre ce que l'on cherche à faire avec deux tables d'indexation. 
Le trait bleu associé à $x_n$ est défini sur l'intervalle de temps $[0,20]$, tandis que la courbe verte associée à $y_n$ 
est définie sur l'intervalle de 
temps $[0,15]$. Le signal $x_{\Phi_x[n]}$ est défini pour les entiers $\{0\ldots 21\}$ et est à valeurs parmi les 
valeurs de $\{x_0\ldots x_{20}\}$, ce sont des points qui sont sur la courbe rouge. La courbe rouge est en fait 
obtenue avec reliant les points $(t_{\Phi_y[n]},x_{\Phi_x[n]})$.
\beqns
\begin{array}{llcl}
\Phi_x[0]=0 & \Phi_y[0]=0 & (t_{\Phi_y[0]},x_{\Phi_x[0]})=(t_0,x_0)=(0,0) & \mbox{position initiale en bas à gauche}\\
& & \vdots& \\
\Phi_x[3]=3 & \Phi_y[1]=0 & (t_{\Phi_y[3]},x_{\Phi_x[3]})=(t_0,x_3)=(0,3) & \mbox{déplacement vertical {\bf V}}\\
\Phi_x[4]=3 & \Phi_y[4]=1 & (t_{\Phi_y[4]},x_{\Phi_x[4]})=(t_1,x_3)=(1,3) & \mbox{déplacement horizontal {\bf H}}\\
\Phi_x[5]=4 & \Phi_y[5]=2 & (t_{\Phi_y[5]},x_{\Phi_x[5]})=(t_2,x_4)=(2,4) & \mbox{déplacement diagonal {\bf D}}\\
&&\vdots &
\end{array}
\eeqns 
Cet exemple illustre le fait que deux tables d'indexation permettent de modéliser un déplacement horizontal et vertical. 

En pratique, on n'utilise pas la base de temps, on modifie juste les indices avec les deux tables 
d'indexation de façon à minimiser le carré des différences entre $x_{\Phi_x[n]}$ et $y_{\Phi_y[n]}$. 
\beqn
y_{\Phi_y[n]}\approx x_{\Phi_x[n]}
\eeqn

On introduit de nouvelles notations. 
\begin{itemize}
\item $N_\Phi$: Les tables d'indexation sont définies sur une plage d'indices communs 
\beqns
n\in\{0\ldots N_\Phi-1\}
\eeqns
\item $N_x$ et $N_y$ sont le nombre d'indices pour $x_n$ et $y_n$. 
Chaque table d'indexation est à valeurs dans les indices sur lesquels $x_n$ et $y_n$ sont définis
\beqns
\Phi_x[n]\in \{0\ldots N_x-1\} \mbox{ et }\Phi_y[n]\in \{0\ldots N_y-1\}
\eeqns
\end{itemize}


En pratique, on impose que le premier indice de $\Phi_x$ corresponde au point de départ de $x_n$, le dernier de $\Phi_x$
avec le point d'arrivée de $x_n$ et de même pour $\Phi_y$ avec $y_n$. 
\beqn\label{eq:phi_contr1}
\left \{
\begin{array}{ll}
\Phi_x[0]=0,\,&\Phi_x[N_{\Phi}-1]=N_x-1\\[0.2cm]
\Phi_{y}[0]=0,\,&\Phi_{y}[N_{\Phi}-1]=N_y-1\\[0.2cm]
\end{array}
\right . 
\eeqn

On introduit la contrainte modélisant le non-retournement du temps 
\beqn\label{eq:phi_contr2}
\Phi_x[n]\leq \Phi_x[n+1] \mbox{ et }\Phi_{y}[n]\leq \Phi_{y}[n+1]
\eeqn


On rajoute une autre contrainte qui indique que la différence de temporalité entre les deux signaux ne doit pas 
être trop grande. 
Cette contrainte a aussi l'avantage de diminuer la complexité numérique de l'algorithme utilisé pour calculer cette nouvelle distance. 
\beqn\label{eq:phi_contr3}
\left |\Phi_x[n]-\Phi_{y}[n]\right |\leq \delta
\eeqn
$\delta$ étant un paramètre à définir pour calculer cette distance. 

\subsubsection{Distance définie au moyen d'un problème d'optimisation}


Pour chaque choix de $\Phi_x$ et $\Phi_y$, on a une valeur de distance qui est obtenue classiquement avec la moyenne quadratique. 
\beqn
\label{eq:tw_d1}
\boxed{
d_{\Phi_x,\Phi_{y}}(x,y)=\sqrt{\frac{1}{N_x+N_y}{\sum_{n=0}^{N_{\Phi}-1} \left(x_{\Phi_x[n]}-y_{\Phi_{y}[n]} \right )^2}}
}
\eeqn
La distance prenant  en compte de la déformation temporelle dynamique est alors défini en choisissant 
$\Phi_x$ et $\Phi_y$ de façon à respecter les contraintes définies par les équations~(\ref{eq:phi_contr1}),~(\ref{eq:phi_contr2}) et~(\ref{eq:phi_contr3}). 
et à minimiser $d_{\Phi_x,\Phi_{y}}(x,y)$.
\beqn\label{eq:prob_min}
\boxed{
d_\delta(x,y)=\underset{\Phi_x,\Phi_y}{\min}\,d_{\Phi_x,\Phi_{y}}(x,y)
}
\eeqn

\subsubsection{Algorithme résolvant ce problème d'optimisation}

\begin{figure}
\begin{center}
\begin{tabular}{c}
\includegraphics[width=0.5\linewidth]{fig_8c.png}
\includegraphics[width=0.5\linewidth]{fig_8d.png}
\end{tabular}
\end{center}
\caption{\`A gauche~: représentation temporelle des signaux $x_n$, $y_n$ et $x_n$ transformés par déformation temporelle. 
\`A droite~: représentation des tables d'indexation permettant de générer la déformation temporelle du signal $x_n$. 
}
\label{fig8}
\end{figure}

La gauche de la figure~\ref{fig8} est similaire à la figure~\ref{fig7} avec en bleu et vert deux signaux $(t_n,x_n)$ et $(t_n,y_n)$ et 
en rouge, la déformation du premier signal pour se rapprocher du second~: $(t_{\Phi_y[n]},x_{\Phi_x[n]})$. 
La droite de cette figure montre les valeurs prises par~$\Phi_x[n]$ et~$\Phi_y[n]$ en représentant ces deux tables 
comme une succession de points formant un chemin reliant au départ~$(0,0)$ au point d'arrivée~$(N_x,N_y)=(5,3)$.
Ces contraintes correspondent à  l'équation~(\ref{eq:phi_contr1}). 
On satisfait la contrainte de l'équation~(\ref{eq:phi_contr2}) en imposant que le chemin soit composé seulement de 
déplacement verticaux, horizontaux ou diagonaux et en l'occurrence seulement d'un pas à la fois. 
La contrainte indiquée par l'équation~(\ref{eq:phi_contr3}) est indiquée par les traits noirs hachurés à l'extérieur de la zone autorisée sur la 
droite de la figure~\ref{fig8}. 
 


Les valeurs utilisées pour les signaux représentés sur la figure~\ref{fig8} sont 
\beqns
\begin{array}{llllll}
x_0=0 & x_1=1 & x_2=2 & x_3=3 & x_4=4 & x_5=5\\[0.2cm]
y_0=0 & y_1=2 & y_2=4 & y_3=5\\[0.2cm]
\end{array}
\eeqns
Les tables d'indexations créées sont~: 
\beqns
\begin{array}{llllll}
\Phi_x[0]=0 & \Phi_x[1]=1 & \Phi_x[2]=2 & \Phi_x[3]=3 & \Phi_x[4]=4 & \Phi_x[5]=5 \\[0.2cm]
\Phi_y[0]=0 & \Phi_y[1]=0 & \Phi_y[2]=0 & \Phi_y[3]=1 & \Phi_y[4]=2 & \Phi_y[5]=3 \\[0.2cm]
\end{array}
\eeqns

On appelle arête ({\em edge}) les traits associés au déplacement sur le graphe de droite. On appelle noeud ({\em node}, {\em vertice}) les 
points indiqués par des ronds bleus sur le graphe de droite. 
La localisation du point $n$ est déterminé par $\Phi_x[n]$ et $\Phi_y[n]$, il se trouve que ces valeurs déterminent aussi 
\beqns
(x_{\Phi_x[n]}-y_{\Phi_y[n]})^2
\eeqns
Les nombres en bleus situés à côté de chaque noeud donnent la valeur de cette quantité. 
Ce sont les valeurs de $x_n$ et $y_n$ qui donnent à chaque point du graphe de droite une valeur pour $(x_{\Phi_x[n]}-y_{\Phi_y[n]})^2$
dépendant uniquement de la position du point. 
La distance entre les deux signaux telle que définie dans l'équation est à la somme des quantités inscrites à côté de chaque noeud. 
L'équation~(\ref{eq:prob_min}) indiquant que la distance est obtenue à partir du chemin minimisant $d_{\Phi_x,\Phi_y}(x,y)$
 définie par l'équation~(\ref{eq:tw_d1}). Il se trouve que le graphe à droite de la figure~\ref{fig8} donne une interprétation de cette minimisation. 
$d_{\Phi_x,\Phi_y}(x,y)$ est la somme des valeurs associées à chaque point et qui ne dépend que de la position des points. 
La minimisation consiste donc à trouver le chemin minisant la somme des valeurs de chaque noeud en utilisant que des déplacements verticaux, horizontaux ou diagonaux et menant d'un point de départ à un point d'arrivée tout en restant dans le domaine délimité par les zones hachurées. 

L'algorithme permettant cette minimisation s'appelle l'algorithme de Dijkstra. 
Il consiste dans un premier temps à découvrir tous les noeuds possibles.
\begin{itemize}
\item Le premier noeud regardé est le point de départ et on lui affecte la valeur associée $(x_0-y_0)^2$. 
\item On répète la tâche suivante
\begin{enumerate}
\item\label{it:vois} Aller au voisin et lui donner la valeur de la distance entre le point de départ et ce voisin. 
\item On indique aussi à ce voisin le noeud précédent où l'on était. 
\item Si sur ce voisin il y a déjà une valeur, alors cette valeur doit être diminuée si la distance trouvée est moindre et 
on lui change l'origine que si l'on change sa valeur. 
\item Revenir au noeud précédent. 
\item Aller à l'étape~\ref{it:vois} s'il y a un voisin disponible et non-exploré dans cette tâche. 
\item Revenir au premier voisin et s'autoriser à aller à une profondeur supplémentaire. 
\end{enumerate}
\end{itemize}
Lorsque ces tâches ne peuvent plus être répétés parce qu'on a été au maximum de la profondeur possible, alors 
on part du point d'arrivée et on remonte au point de départ en suivant les indications laissées à chaque noeud. 




\begin{figure}
\begin{center}
\begin{tabular}{c}
\includegraphics[width=\linewidth]{fig_dist_temp_bis.png}
\end{tabular}
\end{center}
\caption{\`A gauche~: représentation temporelle des signaux $x_n$, $y_n$ et $x_n$ transformés par déformation temporelle. 
\`A droite~: représentation des tables d'indexation permettant de générer la déformation temporelle du signal $x_n$. 
}
\label{fig8bis}
\end{figure}

La figure~\ref{fig8bis} est assez similaire à la figure~\ref{fig8} mais avec d'autres valeurs pour les signaux $x_n$, $y_n$, $\Phi_x[n]$ et $\Phi_y[n]$. 



\section{Prédiction par le plus proche voisin}
\label{sec:knn}
\subsection{Principe}

\begin{figure}
\begin{center}
\begin{tabular}{c}
\includegraphics[width=\linewidth]{knn_ex1.png}
\end{tabular}
\end{center}
\caption{Visualisation de sons à travers les valeurs des indicateurs $\mu_\sm{PMCT}$ et $\sigma_\sm{PMCT}$}
\label{fig_knn}
\end{figure}

On appelle {\bf classifieur} le programme ou le procédé par lequel il est estimé que le son appartient à telle classe. 

On appelle {\bf prédiction} le fait pour un classifieur d'estimer qu'un son appartient à une classe en utilisant uniquement les données 
numériques disponible pour ce son. 

La prédiction par le plus proche voisin est un cas particulier d'un classifieur appelé $k$-NN pour {\em Nearest Neighbor} ce qui signifie 
justement les $k$ plus proche voisins. Ce classifieur est performant mais très coûteux en terme de complexité numérique dès lors que la 
base de donnée est assez importante. Il est aussi particulièrement simple à implémenter, ce qui est la raison principal de son choix ici. 
Il est utilisé ici dans le cas où $k=1$. 

Ce classifieur consiste pour chaque son inconnu appelé requête, de parcourir tous les sons de la base de données et pour chaque son de 
calculer sa distance avec la requête. Le classifieur détermine la classe comme étant celle du son ayant la plus petite distance avec la requête. 
Cette classe est appelée la prédiction faite par le classifieur pour cette requête. 
Il est intéressant de remarquer que ce choix de faire une classification en fonction d'un seul élément (ou de $k$ éléments dans la version plus 
générale de cet algorithme) permet de s'adapter à une situation ou une classe regrouperait des éléments très hétérogènes. 


La figure~\ref{fig_knn} montre comment une vingtaine de sons peuvent être visualisés sur un graphe. Chaque point correspond à un son, sa couleur 
(bleu pour {\tt un}, vert pour {\tt deux}, rouge pour {\tt trois}) indique le mot que ce son vocalise. Cette information est ce que l'on cherche à prédire avec 
la prédiction par le plus proche voisin. La localisation de chaque point dépend des valeurs de deux indicateurs, $\mu_{\sm{PMCT}}$ et $\sigma_{\sm{PMCT}}$. 
Ces indicateurs ont été présentés dans les sections~\ref{ssec:PMCT} et~\ref{ssec:mu_sigma}, c'est un programme informatique qui à partir des
données enregistrées permet de calculer ces deux valeurs et ainsi de positionner ces points sur ce graphique.
Pour illustrer le fonctionnement de cette technique de prédiction, voici son fonctionnement. 
\begin{enumerate}
\item  Sélectionnez dix points que vous numérotez de $1$ à $10$. 
\item Considérer un autre 
point qui ne figure pas parmi ces points. Ce point est appelé requête. 
\item Mesurez avec une règle la distance entre ce point requête et chacun de ces 10 points numérotés. 
\item Regardez la couleur du point qui a la distance avec le point requête la plus faible (et qui est donc sur le graphique 
le plus proche du point requête parmi les 10 points numérotés).
\item La prédiction consiste à attribuer au point requête la couleur du point le plus proche et par suite la classe, {\tt un}, {\tt deux} ou 
{\tt trois} suivant la 
couleur observée. 
\end{enumerate}

\subsection{Formalisation de la technique du plus proche voisin}

 Pour formaliser cette technique du plus proche voisin, on adopte les notations suivantes. 
\begin{itemize}
\item $x$ désigne en général un son défini pour plus de généralité par ses valeurs  $x_n$. 
\item $\chi$ désigne un ensemble de sons. 
\item $y$ désigne la classe à laquelle le son $x$ appartient, ({\tt un}, {\tt deux} ou {\tt trois}), est indiqué par son appartenance respective à $\chi_1, \chi_2,\chi_3$. 
\item $\br{d}(x_a,x_b)$ est une valeur positive correspondant à 
la distance entre les sons $x_a$ et $x_b$. En fait pour plus de généralité, ce calcul repose sur la réalisation des 
étapes suvantes. 
\begin{itemize}
\item Découpage de $x_a$ et $x_b$ en trames décrit à la section~\ref{sec:N:son_trames}.
\item Calcul d'un indicateur par trame pour $x_a$ et $x_b$, illustré par $\sm{PMCT}$ décrite à la section~\ref{ssec:PMCT}.
\item Mise en  oeuvre d'une des trois distance présentées dans les sections~\ref{ssec:mu_sigma},~\ref{ssec:dist_trames},~\ref{ssec:dist_def_temp}. 
\end{itemize}
\item $\br{d}(x,\chi)$ désigne la distance entre le son $x$ et un ensemble de sons regroupés dans $\chi$. 
Du fait du choix de la technique du plus proche voisin, cette distance est ici définie par 
\beqn
\boxed{
\br{d}(x,\chi)=\min\limits_{x'\in \chi} \br{d}(x,x')
}
\eeqn
où $\min\limits_{x'\in \chi} \br{d}(x,x')$ désigne la valeur la plus faible parmi les distances mesurées entre un son donné $x$ et 
tous les sons $x'$ contenus dans $\chi$. 
\item $\ww{x}$ désigne la classe prédite. Cette classe est prédite de cette façon. 
\beqn
\boxed{
\ww{x}=\argmin_{c\in\{1,2,3\}}\br{d}(x,\chi_c)
}
\eeqn
où $\chi_1,\chi_2,\chi_3$ regroupent des sons dont on sait qu'ils sont respectivement associés à {\tt un}, {\tt deux} et {\tt trois}. 
et $\argmin\limits_{c\in\{1,2,3\}}\br{d}(x,\chi_c)$ est ainsi défini. 
\beqns
\argmin\limits_{c\in\{1,2,3\}}\br{d}(x,\chi_c)=\left \{
\begin{array}{lclcl}
1 & \mbox{si} & \br{d}(x,\chi_1)\leq \br{d}(x,\chi_2) &\mbox{et}& \br{d}(x,\chi_1)\leq \br{d}(x,\chi_3)\\
2 & \mbox{si} & \br{d}(x,\chi_2)\leq \br{d}(x,\chi_1) &\mbox{et}& \br{d}(x,\chi_2)\leq \br{d}(x,\chi_3)\\
3 & \mbox{si} & \br{d}(x,\chi_3)\leq \br{d}(x,\chi_1) &\mbox{et}& \br{d}(x,\chi_3)\leq \br{d}(x,\chi_2)\\
\end{array}
\right . 
\eeqns

\end{itemize}


\subsection{Illustration avec l'implémentation proposée en TP}

\begin{figure}
\begin{center}
\begin{tabular}{c}
\includegraphics[width=\linewidth]{fig_rep_req.png}
\end{tabular}
\end{center}
\caption{Schéma correspondant aux différents dossiers existant et créés pour réaliser la prédiction en utilisant la technique du plus proche voisin. 
}
\label{fig9bis}
\end{figure}

La figure~\ref{fig9bis} illustre la façon  dont l'algorithme est ici implémenté. Chaque bloc représente un répertoire 
contenant des fichiers. 
Les sons que l'on utilise pour tester et évaluer la performance d'un classifieur sont en réalité issus de la base de données. 
Il faudrait donc s'assurer qu'ils ne sont pas utilisés aussi pour l'apprentissage. 
La partie qui n'est pas encadré en pointillé n'est pas modifiée lors de la mise en oeuvre de la classification. Cette
mise en oeuvre consiste à tirer aléatoirement une partie des sons des répertoires {\tt un}, {\tt deux} et {\tt trois}, 
de les placer dans le
répertoire {\tt requête}, les autres sons sont placés dans trois nouveaux répertoires contenus dans le répertoire 
{\tt simulation} et appelé {\tt un}, {\tt deux} et {\tt trois}. 
L'information selon laquelle les sons placés dans {\tt requête} n'est pas disponible sur les fichiers sons, mais elle 
est stockée pour être utilisée ultérieurement lors de l'évaluation de l'algorithme. 

\section{\'Evaluation de la performance d'un classifieur}
\label{sec:evaluation_classification}

En pratique quand on utilise un procédé de reconnaissance vocal, on a besoin de savoir dans quelle mesure on peut lui faire confiance. 
Cette mesure est ce qu'on appelle l'{\bf évaluation de la performance}. Pour se faire, on utilise des sons dont on connaît la classe à laquelle 
ils appartiennent et on compare cette classe avec ce que le classifieur prédit. Il existe un très grand nombre de mesures de performance, on en présente 
trois types~: la sensibilité globale, la précision et le rappel. 

\subsection{Matrice de confusion}

Le rôle de la matrice de confusion est de résumer sous la forme d'une matrice les données utiles au calcul de l'évaluation de la performance. 
Ces données utiles consistent en le fait de connaître le nombre d'expérience où le son requête appartenait à telle classe et où la classe prédite est 
celle-là. Dans le cadre de cette étude, il s'agit d'une matrice $3{\times}3$ puisqu'il y a trois sons possibles. 

\begin{itemize}
\item Chaque {\bf ligne} est associée aux expérimentations sur les sons qui en réalité appartiennent à telle classe. 
\item Chaque {\bf colonne} est associée aux expérimentations sur les sons qui ont été prédit comme étant de telle classe. 
\item La somme de toutes les cases est égale au nombre total d'expérimentations. 
\item \`A la case $i,j$, il y a le nombre d'expérimentations pour lesquelles le son appartient en réalité à la classe~$i$ et 
le classifieur l'a prédit comme étant de la classe~$j$. 
\item $m$ est un indice faisant référence à un son $x$. 
\item $M$ est le nombre total de sons utilisés pour les différentes requêtes. 
\item $\1(\ldots)$ est la fonction caractéristique, elle prend la valeur $1$ si les trois points de suspension sont remplacés par 
une affirmation exacte et par $0$ si l'affirmation est fausse. 
\item $\1(y_m=c)$ vaut $1$ si  le son numéro $m$ est de la classe $c$ et $\1(y_m=c)$ vaut $0$ si ce n'est pas le cas. 
\item $\1(\ww{x}_m=c)$ vaut $1$ si le son numéro $m$ est prédit par le classifieur comme étant de classe $c$ et $\1(\ww{x}_m=c)$ vaut $0$ 
si ce n'est pas le cas. 
\item $\1(y_m=i)\1(\ww{x}_m=j)$ vaut $1$ is le son numéro $m$ est d'une part de la classe $i$ et d'autre part a été prédit par le classifieur 
comme étant de la classe $j$. 
\end{itemize}

Les composantes de la matrices de confusion sont~: 
\beqn\label{eq:matrice_confusion}
\boxed{
C_{ij}={\sum_{m=1}^M\1(y_m=i)\1(\ww{x}_m=j)}
}
\eeqn


\subsection{Sensibilité globale}

La sensibilité globale, notée $\OA$ pour {\em Overall Assessment}, est 
le rapport entre le nombre de classifications correctes sur le nombre totales de requêtes, noté $M$. 
Les classifications correctes sont celles pour lesquelles $y_m=\ww{x}_m$. 

\beqn
\label{eq:OA}
\boxed{
\OA=\frac{C_{11}+C_{22}+C_{33}}{3}
}
\eeqn

\subsection{Précision et rappel}

La précision et le rappel sont des notions très utilisées pour les classifieurs binaires, c'est-à-dire pour lesquels, il n'y a que deux classes. 
Mais ces notions sont parfois étendues au cas plus général où on considère un nombre plus important de classes, c'est ce que nous utilisons ici. 

Pour chaque classe~$c$, on calcule deux indicateurs. La {\bf précision} $\p{P}_c$ est le rapport entre le nombre de requête correctement attribuées à la classe~$c$
et le nombre de requêtes que le classifieur évalué a prédit comme étant de la classe~$c$. 
Le {\bf rappel} $\p{R}_c$  est le rapport entre le nombre de requête correctement attribué à la classe~$c$ 
et le nombre de requêtes qui dans la réalité correspondent à la classe~$c$. 
\beqn
\boxed{
\left\{
\begin{array}{l}
\p{P}_1=\frac{C_{11}}{C_{11}+C_{21}+C_{31}}\\[0.3cm]
\p{P}_2=\frac{C_{22}}{C_{12}+C_{22}+C_{32}}\\[0.3cm]
\p{P}_3=\frac{C_{33}}{C_{13}+C_{23}+C_{33}}\\[0.3cm]
\end{array}
\right.
\quad
\mbox{et} \quad 
\left\{
\begin{array}{l}
\p{R}_1=\frac{C_{11}}{C_{11}+C_{12}+C_{13}}\\[0.3cm]
\p{R}_2=\frac{C_{22}}{C_{21}+C_{22}+C_{23}}\\[0.3cm]
\p{R}_3=\frac{C_{33}}{C_{31}+C_{32}+C_{33}}\\[0.3cm]
\end{array}
\right.
}
\eeqn
Ainsi la précision indique la probabilité  qu'un échantillon, dont le classeur évalué indique qu'il s'agit de la classe~$i$, 
soit effectivement de la classe~$i$. 
Par contre,  le rappel indique la probabilité pour qu'un échantillon dont on sait qu'il est de la classe~$i$, soit détecté 
comme tel par le classifieur évalué. 


\subsection{Validation croisée}

\begin{figure}
\begin{center}
\begin{tabular}{c}
\includegraphics[width=0.8\linewidth]{illustration_validation_croisee.png}
\end{tabular}
\end{center}
\caption{Schéma décrivant ce qu'est une validation croisée.}
\label{fig:O:valid_croisee}
\end{figure}


La {\bf validation croisée} est une technique souvent utilisée pour la mise en oeuvre d'un algorithme de classification, 
elle n'est pas destinée à améliorer l'efficacité d'un classifieur, elle est destinée à évaluer plus précisément sa 
performance vis-à-vis d'une base de données en particulier  lorsqu'il est compliqué d'augmenter le nombre de sons dont on connaît la
classe à laquelle chacun appartient. 
La figure~\ref{fig:O:valid_croisee} illustre le fonctionnement de la validation croisée avec un schéma. 
En haut de cette figure se trouve 12 sons figurés par $x_1\ldots x_{12}$ et $12$ valeurs notées $y_1\ldots y_{12}$ indiquant les véritables classes à laquelle chaque son appartient.
Ici il s'agit d'une validation croisée en quatre blocs, ce qui amène à réaliser quatre apprentissages de classifieurs. 
{\tt Exp1} désigne en haut la première expérience avec le premier apprentissage. Les trois premiers sons de la base 
d'apprentissage $(x_1,y_1),(x_2,y_2),(x_3,y_3)$ servent de base pour tester le classifieur et sont affichés sur fond rouge. Le classifieur testé est entraîné 
en utilisant tous les autres sons $(x_4,y_4),\ldots,(x_{12},y_{12})$ qui sont eux affichés sur fond bleu. Le test du classifieur permet de calculer une matrice 
de confusion spécifique à {\tt Exp1} et celle-ci permet de calculer la sensibilité globale $\sm{OA}_1$.
Les trois autres expériences sont fait de la même façon, mais en utilisant successivement comme sons tests les 
sons $(x_4,y_4),(x_5,y_5),(x_6,y_6)$, puis $(x_4,y_4),(x_5,y_5),(x_6,y_6)$ et enfin $(x_4,y_4),(x_5,y_5),(x_{12},y_{12})$.





\chapter{Descripteurs de trames}
\label{ch:desc}

La partie précédente ayant montrée comment un descripteur par trame permet de définir une technique de classification, cette 
partie traite de la détermination d'un descripteur par trame. 
L'inspiration qui a guidé l'élaboration des descripteurs provient de l'étude des caractéristiques des ondes sonores émises par un individu,
c'est ce qui constitue la section~\ref{sec:model_parole} et qui montre l'intérêt de trouver la fréquence fondamentale et la plage de fréquences présentes
dans le son émis. 
La section~\ref{sec:estimation_spectrale} présente différentes heuristiques permettant de décrire ce contenu spectral en indiquant la fréquence fondamentale, la 
fréquence moyenne et la largeur de spectre. 
La section~\ref{sec:banc_filtres} présente une technique plus systématique pour décrire le contenu spectral, c'est en utilisant un banc de filtres, chaque 
filtre constitue une heuristique donnant une information partielle sur le contenu spectral du son. 


\section{Modélisation de la production de la parole}
\label{sec:model_parole}

La présentation de la modélisation de la façon dont un humain produit un son est 
faite en trois parties. La section~\ref{ssec:onde_stationnaire} décrit le phénomène physique 
permettant de transformer une source sonore en un son dont le caractère plus ou moins aigü du son 
peut être déterminé assez précisément au moyen d'une note. 
La section~\ref{ssec:appareil_phonatoire} décrit brièvement les organes humains intervenant pour 
la production d'un son. 
Enfin la section~\ref{ssec:spectrogramme} présente la notion d'analyse temps-fréquence illustré 
avec la présentation d'un spectrogramme.

\subsection{Onde stationnaire}
\label{ssec:onde_stationnaire}

On dit qu'une onde est stationnaire si en chaque point, on observe que  la surpression évolue dans le temps comme une sinusoïde. 
Par exemple l'équation suivante décrit une évolution sinusoïdale dont l'amplitude crête à crête dépend de l'indice $x$ et vaut 
$\cos(2\pi \frac{x}{\lambda_0})$. 
\beqns
P(x,t)=\Delta P_0\cos(2\pi f_0t)\cos(2\pi \frac{x}{\lambda_0})
\eeqns
où $\lambda$ et $f_0$ sont 
Cette onde peut approximativement correspondre à un cas particulier de l'équation~(\ref{eq:propag_onde}) lorsque le coefficient $\frac{1}{r}$ est 
supposé approximativement constant et~$r$ est remplacé par~$x$. 
La trigonométrie nous indique
que le produit de deux cosinus est une différence entre deux sinus,
 $\cos(a)\cos(b)=\frac{1}{2}\cos(a-b)+\frac{1}{2}\cos(a+b)$. 
Cela permet de voir qu'une onde stationnaire est la somme d'une onde se propageant dans le sens des $x$ croissants et 
une autre dans le sens des $x$ décroissants.
\beqn\label{eq:onde_stationnaire}
P(x,t)=\frac{\Delta P_0}{2}\cos\left (2\pi f_0(t-\frac{x}{c})\right )
+\frac{\Delta P_0}{2}\cos\left (2\pi f_0(t+\frac{x}{c})\right )
\eeqn
où $c=\lambda_0 f_0$ est la vitesse de propagation du son dans l'air. 
Cette modélisation correspond à $g_1=g_2$ dans l'équation~(\ref{eq:propag_onde}). 




\begin{figure}[htbp]
\begin{center}
\begin{tabular}{c}
\includegraphics[width=0.5\linewidth]{onde_stationnaire.png}
\end{tabular}
\end{center}
\caption{Pour une même taille donnée, un même obstacle peut être le siège de trois ondes stationnaires. 
La vitesse moyenne des particules d'air doit être nulle aux deux extrémités de la caisse de résonnance. }
\label{fig:onde_stationnaire}
\end{figure}

La figure~\ref{fig:onde_stationnaire} illustre de manière simplifiée la façon dont la forme géométrique d'une caisse de 
résonance détermine une fréquence de résonance. 
Le haut de la figure schématise al caisse de résonance qui est un pavé. La coupe est un rectangle. La zone colorée 
en bleu schématise une onde stationnaire qui consiste en une variation spatiale et temporelle avec une relation 
entre la longueur d'onde et la fréquence de la vibration indiquée dans l'équation~\ref{eq:long_onde} ($\lambda=c/f$ où 
$c$ est ici la vitesse de propagation du son dans l'air, approximativement 1km toutes les $3$~secondes). Les trois dessins 
illustrent qu'avec une même forme géométrique (un pavé de longueur $d$), $3$ longueurs d'onde sont montrés. 
\begin{center}
\begin{tabular}{|c|c|c|}
\hline 
$\lambda=2d$ & $f=\frac{c}{2d}$ & $d=\frac{\lambda}{2}$\\[0.1cm]
\hline
$\lambda=d$ & $f=2\frac{c}{2d}$ & $d={\lambda}$\\[0.1cm]
\hline
$\lambda=\frac{2}{3}d$ & $f=3\frac{c}{2d}$ & $d=\frac{3\lambda}{2}$\\[0.1cm]
\hline
\end{tabular} 
\end{center}

Cette schématisation illustre un phénomène plus général, à savoir que l'émission d'un son à une certaine fréquence de base
produit généralement des harmoniques qui sont des vibrations à des fréquences qui sont multiples de cette fréquence de base. 
La relation entre longueur du rectangle et longueur d'onde est ici déterminé par le fait que la vibration 
du son est nul sur la paroi (i.e. la paroi est fixe). Dans une onde stationnaire modélisée par l'équation~(\ref{eq:onde_stationnaire}),
c'est à cet endroit que la pression est soit maximale soit minimale.
L'annexe~\ref{app:onde_stationnaire_1D} formalise cette description de manière plus précise.  

Une onde stationnaire peut aussi exister avec un rectangle ouvert sur un côté. Dans ce cas c'est la pression qui est fixée et la vibration 
qui est maximale à l'endroit où le rectangle est ouvert. Les relations entre longueurs d'onde, fréquences et longueur du rectangle sont alors modifiées. 
\begin{center}
\begin{tabular}{|c|c|c|}
\hline 
$\lambda=4d$ & $f=\frac{c}{4d}$ & $d=\frac{\lambda}{4}$\\[0.1cm]
\hline
$\lambda=\frac{4}{3}d$ & $f=3\frac{c}{4d}$ & $d=\frac{3\lambda}{4}$\\[0.1cm]
\hline
$\lambda=\frac{4}{5}d$ & $f=5\frac{c}{4d}$ & $d=\frac{5\lambda}{4}$\\[0.1cm]
\hline
\end{tabular} 
\end{center}



\subsection{Modélisation de l'appareil phonatoire}
\label{ssec:appareil_phonatoire}


\begin{figure}[htbp]
\begin{center}
\begin{tabular}{c}
\includegraphics[width=0.5\linewidth]{parole_formation.jpg}
\end{tabular}
\end{center}
\caption{Diagramme représentant les organes de la parole }
\label{fig:parole_formation}
\end{figure}

On appelle appareil phonatoire l'ensemble des organes humains permettant de produire un son. 
L'objet de cette partie est une brève description de son fonctionnement. 

La figure~\ref{fig:parole_formation} représente une coupe de la tête d'une personne, (coupe dite sagittale), avec la gorge en bas à droite, la bouche au milieu à gauche, les dents le long d'une ligne horizontale placée légèrement au dessus de la bouche. 
Cette figure permet de modéliser la façon dont un son est formé. 
\begin{itemize}
\item Le son est produit par la vibration d'un organe musculaire appelé corde vocale ou plis vocaux. Cet organe musculaire 
permet un contrôle de la fréquence du son émis à ce niveau.  
\item L'intensité du son est modulé par l'intensité du flux d'air sortant du poumon situé plus bas. 
\item Une première caisse de résonance est localisée dans la bouche et sa forme géométrique est modulée notamment par 
la position de la langue et l'ouverture de la bouche. Cette forme géométrique entraîne la formation de vibrations. 
\item Une deuxième caisse de résonance est localisée dans un espace libre au dessus de la bouche au niveau du nez, espace 
appelé cavité nasale. Cette deuxième caisse de résonance entraîne la formation d'un son avec une certaine fréquence. 
\end{itemize}

Ainsi l'anatomie du corps humain permet de modifier l'intensité d'un son et la différence entre deux fréquences 
de résonance. 




%\begin{figure}[htbp]
%\begin{center}
%\begin{tabular}{c}
%\includegraphics[width=0.5\linewidth]{coupe_schematique_parole.png}
%\end{tabular}
%\end{center}
%\caption{Diagramme représentant les organes de la parole, extraite de~\cite{KhederW17} }
%\label{fig:coupe_schematique_parole}
%\end{figure}
%\section{Estimation spectrale}

\subsection{Spectrogramme et notion de description temps-fréquence}
\label{ssec:spectrogramme}

\begin{figure}[htbp]
\begin{center}
\begin{tabular}{c}
\includegraphics[width=0.5\linewidth]{spectrogramme.png}
\end{tabular}
\end{center}
\caption{spectrogramme d'un signal sonore.}
\label{fig:spectrogramme}
\end{figure}

La figure~\ref{fig:spectrogramme} est un exemple de spectrogramme, c'est une visualisation d'un son, ici 
constitué d'une partie parlée à gauche, un silence au milieu, et de nouveau une partie parlée à droite. 
L'axe horizontal est le temps en seconde. L'axe vertical est la fréquence en Hertz. 
Il s'agit d'une représentation temps-fréquence, ce qui peut paraître contradictoire dans le cadre de ce cours. 
En effet une description temporelle d'un signal ne dépend pas de la fréquence et une description fréquentielle d'un signal 
au moyen de son spectre ne dépend pas du temps. En fait la position latérale d'un point détermine une portion du signal sur un intervalle
de temps. Tous les points d'une même verticale concernent la même portion du signal. 
Cette portion de signal est transformée en un spectre qui permet d'indiquer comment l'énergie de cette portion du signal est décomposée en 
une somme  de signaux sinusoïdaux. Chaque point de cette verticale représente une de ces sinusoïdes, c'est la hauteur de ce point qui en déterminant 
une fréquence détermine aussi la sinusoïde. Et un point 
 est d'autant plus sombre ou rouge que l'amplitude du signal sinusoïdal est plus importante. Sur ce spectrogramme, on observe une alternance de 
bandes sombres/rouges horizontales qui sont à la fois régulièrement espacées et avec des intensités qui diminues lorsque la fréquence augmente. 
Ce phénomène est lié au caisses de résonance qui produisent des sons avec une fréquence de base et des harmoniques qui sont des multiples 
de la fréquence de base.

Historiquement la recherche en reconnaissance de la parole s'est d'abord donnée comme guide le fait 
de modéliser les organes qui produisent ou reconnaissent la parole. En pratique la complexité numérique 
et la difficulté à modéliser limitaient la précision des modèles obtenues et par suite la performance. 
Il semble aujourd'hui admis que les techniques de machine learning permettent plus facilement d'obtenir 
des techniques efficaces. Il reste cependant de toutes ces études l'importance apportée à l'utilisation 
d'un certain type de descripteurs et par exemple l'importance d'estimer la fréquence fondamentale. 
L'utilité de s'intéresser à la fréquence fondamentale pour reconnaître une voyelle est 
expliquée en détail dans~\cite{Meunier07}.











\section{Estimation spectrale}
\label{sec:estimation_spectrale}

L'objet de cette partie est de définir 
une application transformant les valeurs sur une trame~$k$ en une valeur donnée, appelée valeur du 
descripteur. 
La section~\ref{ssec:estimation_frequence_fondamentale} présente des techniques permettant 
d'estimer la fréquence fondamentale. 
La section~\ref{sec:descripteur_spectre} presente d'autres techniques permettant d'estimer 
d'autre caractéristiques du spectre, par exemple sa largeur. 

\subsection{Estimation de la fréquence fondamentale}
\label{ssec:estimation_frequence_fondamentale}

Dans cette partie, les deux indicateurs présentés ont pour objectif d'estimer la fréquence fondamentale.~\footnote{Pour un son musical assez simple, cette 
fréquence correspond au {\em pitch} défini section~C.3, p.~215-217 de~\cite{Rocchesso03}.} 

Une autre technique existe pour mesurer la fréquence fondamentale en s'appuyant sur l'autocorrélation.~\footnote{Cette 
technique est brièvement présentée p.~45-46 dans~\cite{Camastra07}.}


\subsubsection{Zero Crossing Rate}

\begin{figure}[htbp]
\begin{center}
\begin{tabular}{c}
\includegraphics[width=0.5\linewidth]{zero_crossing_rate.png}
\end{tabular}
\end{center}
\caption{Graphe illustrant le fonctionnement de l'indicateur $\mb{ZCR}$. }
\label{fig:zero_crossing_rate}
\end{figure}


La figure~\ref{fig:zero_crossing_rate} montre l'évolution de deux signaux en fonction du temps. 
Le premier en trait plus foncé/bleu est la superposition de 2 sinusoïdes. Le deuxième 
 en trait plus clair/vert est une sinusoïde.  Le descripteur~\footnote{Cette technique 
appelée {\em zero crossing rate} est évoquée dans la section~2.4 p.~12 de~\cite{Peeters04}, 
et définie dans~\cite{Camastra07} p.~43-44.} 
$\mb{ZCR}$ détermine le nombre de fois où la courbe traverse l'axe horizontal par une unité de temps. 
Ici il y a deux traversées toutes les secondes. 

Le nombre de passage par zéro n'est en fait pas une notion qui se prête à une formalisation 
utilisant le temps continu. 
Le nombre moyen de passages par zéro pour la trame $k$ est donnée par
\beqn
\label{eq:ZCR}
\boxed{
Z_k=\frac{1}{N_K}{\sum_{n=0}^{N_K-1} \1\left (\signe(x_k[n+1])\neq \signe(x_k[n])\right)}
}
\eeqn
Le fait de normaliser par la longueur de la trame ($N_K$) fait que $Z_k$ n'est pas augmenté lorsque 
les trames sont plus longues. 

Ce nombre moyen de passage par zéro est utilisé pour estimer la fréquence fondamentale, c'est la fréquence 
de la sinusoïde qui aurait ce nombre moyen de passages par zéros. 
\beqn
\label{eq:f_ZCR}
\boxed{
f^{(\sm{ZCR})}_k=\frac{Z_k f_e}{2}
}
\eeqn
En effet, pour une sinusoïde de fréquence $f^{(\sm{ZCR})}_k$, sa période est $T=\frac{1}{f^{(\sm{ZCR})}_k}$ 
et le nombre moyen de passages par zéros est $2$ divisé par le nombre de points sur une période $Tf_e$, 
aussi 
\beqns
f^{(\sm{ZCR})}_k=\frac{1}{T}=\left(\frac{2}{T f_e}\right ) \frac{f_e}{2}=\frac{Z_k f_e}{2}
\eeqns


\subsubsection{Fréquence moyenne du spectre}

\begin{figure}[htbp]
\begin{center}
\begin{tabular}{c}
\includegraphics[width=0.5\linewidth]{illustration_frequence_moyenne.png}
\end{tabular}
\end{center}
\caption{Illustration du calcul de la fréquence moyenne et 
de sa signification comme séparant en deux parties 
égales la surface sous la courbe.}
\label{fig:illustration_frequence_moyenne}
\end{figure}

La notion de temps-fréquence évoquée lors de la description du spectrogramme dans la section~\ref{ssec:spectrogramme}
permet de définir une densité spectrale d'énergie qui dépend du temps. Ici cela se fait en 
appliquant une fenêtre rectangulaire avec l'intervalle $\left [t-\frac{T}{2},t-\frac{T}{2}\right]$
sur le signal $x(t)$. 
\beqn
\label{eq:DSP_t}
\boxed{
\left|\ww{X}_t(f)\right|^2=\left |\mb{TF}\left [x(t)\1_{\left [t-\frac{T}{2},t-\frac{T}{2}\right]}(t)\right](f)
\right|^2
}
\eeqn
Ensuite cette densité spectrale dépendant du temps et de la fréquence est une utilisée 
comme pondération dans $\mu(t)$ qui est appelée la fréquence moyenne (son unité est bien le Hertz). 
\beqn\label{eq:mu_t}
\boxed{
\mu(t)=\frac{{\int\limits_0^{+\infty} f\left |\ww{X}(f)\right |^2\,df}}
{{\int\limits_0^{+\infty} \left |\ww{X}(f)\right |^2\,df}}
}
\eeqn
On peut voir ce calcul de moyenne comme assez similaire au calcul de l'espérance 
d'une variable aléatoire à partir de la densité de probabilité d'une variable aléatoire~: 
$E[T]={\int_\bb{R} tf_T(t)\,dt}$ où ici $f$ jouerait le rôle de $t$ et 
$\frac{\left |\ww{X}(f)\right |^2}{{\int\limits_0^{+\infty} \left |\ww{X}(f)\right |^2\,df}}$
jouerait le rôle de $f_T(t)$.

La figure~\ref{fig:illustration_frequence_moyenne} donne une justification 
de la définition de $\mu(t)$ dans l'équation~(\ref{eq:mu_t}).
La courbe en noir notée $P(f)$,
correspondant en réalité à $|\ww{X}_t(f)|^2$, 
est la densité spectrale d'énergie d'une portion du signal 
$x(t)\1_{[t-\frac{T}{2},t+\frac{T}{2}]}(t)$. 
Le trait semi-pointillé vertical est positionné 
%à la fréquence $\mu(t)$. On considère maintenant 
%la surface sous la courbe à gauche de $\mu(t)$, 
%elle est égale au terme de gauche de la deuxième 
%égalité
%\beqns
%{\int_{0}^{\mu(t)}(\mu(t)-f)P(f)\,df}
%\eeqns
%La surface sous la courbe à droite de $\mu(t)$ 
%est égale au terme de droite de la deuxième égalité
%\beqns
%{\int_{\mu(t)}^{+\infty}(f-\mu(t))P(f)\,df}
%\eeqns
%Ainsi qu'il est indiqué à gauche de la figure, 
%l'égalité de ces deux dernières équations conduit 
%à la définition de $\mu(t)$ donnée dans l'équation~(\ref{eq:mu_t}). 
%Ainsi on peut dire que cette moyenne temporelle est 
%la fréquence qui divise en deux parties égales la surface 
%sous la courbe de la densité spectrale d'énergie de la portion 
%de signal. 
%de signal. 

Cette notion est adaptée aux signaux à temps discret en 
considérant la portion du signal~\footnote{Cette application 
de la transformée de Fourier discrète sur 
le signal découpé peut être vu comme 
l'utilisation d'une transformée 
de Fourier à court terme, p.~99 de~\cite{Rocchesso03}.} 
 sur une trame $x_k[n]$ et en lui calculant la transformée de Fourier discrète considérant 
que la longueur de la trame est suffisante pour que cette transformée de Fourier discrète
soit une bonne approximation de la transformée de Fourier de cette portion de signal. 
On utilise ici un indice $l$ pour les fréquences et on ne considère que la première 
moitié des $N_K$ indices parce que la deuxième moitié des indices correspond aux fréquences 
négatives qui n'est pas prise en compte dans l'équation~(\ref{eq:mu_t}).
Cette première moitié des indices est notée 
\beqn\label{eq:N_K_2}
\boxed{
N_K^{\deux}=\left \lfloor \frac{N_K}{2} \right\rfloor
}
\eeqn
où $\lfloor\ldots \rfloor$ désigne l'arrondi par en dessous. 
Les $N_K^{\deux}$ premières fréquences sont 
$\left [0\ldots \frac{N_K^{\deux}f_e}{N_K}\right]$. 
Ces différentes valeurs sont écrites au moyen d'un nouvel indice $l$ dont dépend la fréquence. 
\beqn\label{eq:f_l}
\boxed{
f_l=\frac{lf_e}{N_K}\mbox{ pour }l\in \{0\ldots N_K^{\deux}
}
\eeqn
La pondération utilisée est la densité spectrale de puissance de la trame $k$.
\beqn
\boxed{
\left |\ww{X}_k[l]\right |^2= \left |
\sm{TFD}\left [x_k[n]\right][l]\right |^2
}
\eeqn
Un estimateur de la fréquence moyenne du spectre $\mu_k$~\footnote{Cet estimateur 
est défini dans la section~6.1.1 p.~13 de~\cite{Peeters04}.}
 est  
\beqn\label{eq:mu_sp}
\boxed{
\mu_k=\frac{{\sum_{l=0}^{N_K^{\deux}}\,\,f_l\,\,\left |\widehat{X}_k[l]\right |^2}}
{{\sum_{l'=0}^{N_K^{\deux}}\left |\widehat{X}_k[l']\right |^2}}
}
\eeqn 
% où $\widehat{X}_k[l]$ est la transformée de Fourier discrète à $k$ fixé de $x_k[n]$ définie par 
% $\widehat{X}_k[l]=\frac{1}{N_K}{\sum_{n=0}^{N_K-1}x_k[n]e^{-j2\pi\frac{ln}{N_K}}}$~;
% et ${\lfloor \frac{N_K}{2}\rfloor}$ signifie le plus grand entier inférieur à $N_K/2$. 
Un indice $l'$ est utilisé parce qu'il n'y a en fait aucun lien entre le compteur utilisé dans la sommation au niveau du numérateur et
le compteur utilisé dans la sommation au niveau du dénominateur. 

\subsection{Autre descripteurs du spectre}
\label{sec:descripteur_spectre}

\subsubsection{Largeur du spectre}

\begin{figure}[htbp]
\begin{center}
\begin{tabular}{c}
\includegraphics[width=0.5\linewidth]{illustration_largeur_spectre.png}
\end{tabular}
\end{center}
\caption{Illustration graphique sur un exemple du sens donné à la notion d'estimation de la largeur d'un spectre.}
\label{fig:illustration_largeur_spectre}
\end{figure}


La largeur du spectre est estimée connaissant $\mu(t)$ avec 
\beqn
\label{eq:largeur_spectre}
\boxed{
\sigma(t)=\frac{\sqrt{{\int\limits_{\bb{R}_+}\left(f-\mu(t)\right)^2\left |\ww{X}_t(f)\right|^2\,df}}}{\sqrt{{\int\limits_{\bb{R}_+}\left |\ww{X}_t(f)\right|^2\,df}}}
}
\eeqn

La figure~\ref{fig:illustration_largeur_spectre} représente l'exemple d'un spectre d'une porte. 
La fréquence est en abscisse. Ce spectre a pour équation un sinus cardinal avec un demi-lobe principal de $3000$Hz. 
Cette figure illustre deux descripteurs $\mu$ et $\sigma$. $\mu$ est la fréquence moyenne et $\sigma$ est l'écart-type. 
Les deux sont calculés comme si les spectres étaient nuls pour les fréquences négatives (s'ils étaient calculés sur les 
vrais spectres, comme leur module est symétrique, la moyenne serait nulle. 
$\mu$ est indiqué par un trait vertical en pointillé. $\sigma$ est représenté par deux traits verticaux autour de celui associé à $\mu$. 
Ces deux traits verticaux indiquent que si le spectre était une gaussienne (courbe en traits pointillés), $66\%$ de sa surface serait incluse dans ces deux traits
verticaux en pointillés. Ce graphe n'est en fait pas tout à fait exact, d'une part la proportion de $66\%$ et l'axe de symétrie au centre de la gaussienne n'est 
ici pas valable puisqu'on ne considère que les fréquences positives, d'autre part la moyenne et le calcul de la largeur se fait en considérant 
la densité spectrale et non le module de la transformée de Fourier et cette densité spectrale n'est donc pas exactement un sinus cardinal.

De même pour le calcul de la moyenne temporelle, l'équation~(\ref{eq:largeur_spectre}) décrivant l'estimation de la largeur du spectre peut 
se voir comme l'estimation de l'écart-type d'une variable aléatoire positive de densité de probabilité $f_T(t)$
\beqns
\sqrt{\mb{var}(T)}=\sqrt{E[(T-E[T])^2]}=\sqrt{{\int\limits_{\bb{R}_+}(t-E[T])^2f_T(t)\,dt}}
\eeqns
où ce qui remplace ici la variable $t$ est $f$ et la densité de probabilité $f_T(t)$ est 
\beqns
\frac{1}{{\int\limits_{\bb{R}_+}\left |\ww{X}_t(f)\right|^2\,df}}\, \left |\ww{X}_t(f)\right|^2
\eeqns



En utilisant les mêmes notations que pour (\ref{eq:mu_sp}), une estimation de la largeur du spectre~\footnote{Cet estimateur est défini dans la section~6.1.2 p.~13 de~\cite{Peeters04}.} est
\beqn
\label{eq:sigma_sp}
\boxed{
\sigma_k=\sqrt{\frac{{\sum_{l=0}^{N_K^\deux}\,\,\left (f_l-\mu_k\right )^2\,\,
\left |\ww{X}_k[l]\right |^2}}{{\sum_{l'=0}^{N_K^\deux}\left |\widehat{X}_k[l']\right |^2}}}
}
\eeqn

%En reprenant les notations utilisée pour (\ref{eq:mu_pl}), cet estimateur de la largeur du spectre peut s'écrire ainsi. 
%\beqn
%\sigma=\sqrt{
%{\sum_{l=0}^{l_{\max{}}}(f_l-\mu)^2 \frac{p_l}{{\sum_{l'=0}^{l_{\max{}}} p_{l'}}}}
%}
%\eeqn
%Ainsi $\sigma$ peut s'interpréter comme la racine carré de la variance d'une variable aléatoire discrète $F$ dont les probabilités sont 
%données par $\frac{p_l}{{\sum_{l'=0}^{l_{\max{}}} p_{l'}}}$. 


\subsubsection{Coefficient d'asymétrie du spectre}

Un estimateur du coefficient d'asymétrie ({\em skewness})~\footnote{Cet estimateur est défini dans la section~6.1.3 p.~13 de~\cite{Peeters04}.} est donné 
par 
\beqns
\gamma_1(t)=\frac{1}{\sigma^3(t)}\frac{{\int\limits_{\bb{R}_+}\left(f-\mu(t)\right)^3\left |\ww{X}_t(f)\right|^2\,df}}{{\int\limits_{\bb{R}_+}\left |\ww{X}_t(f)\right|^2\,df}}
\eeqns
qui devient avec les notations utilisées dans (\ref{eq:sigma_sp}).
\beqn
\gamma_1[k]=\frac{1}{\sigma_k^3}{\frac{{\sum_{l=0}^{N_K^\deux}\,\,\left (f_l-\mu_k\right )^3\,\,
\left |\ww{X}_k[l]\right |^2}}{{\sum_{l'=0}^{N_K^\deux}\left |\widehat{X}_k[l']\right |^2}}}
\eeqn
De même, un estimateur du coefficient d'aplatissement ({\em kurtosis})~\footnote{Cet estimateur est défini dans la section~6.1.4 p.~14 de~\cite{Peeters04}.} est donné par
\beqns
\gamma_1(t)=\frac{1}{\sigma^4(t)}\frac{{\int\limits_{\bb{R}_+}\left(f-\mu(t)\right)^4\left |\ww{X}_t(f)\right|^2\,df}}{{\int\limits_{\bb{R}_+}\left |\ww{X}_t(f)\right|^2\,df}}
\eeqns
qui devient avec les notations utilisées dans (\ref{eq:sigma_sp}).
\beqn
\gamma_2[k]=\frac{1}{\sigma_k^4}{\frac{{\sum_{l=0}^{N_K^\deux}\,\,\left (f_l-\mu_k\right )^4\,
\,\left |\widehat{X}_k[l]\right |^2}}{{\sum_{l'=0}^{N_K^\deux}\left |\widehat{X}_k[l']\right |^2}}}
\eeqn


\section{Utilisation de bancs de filtres}
\label{sec:banc_filtres}


\begin{figure}[htbp]
\begin{center}
\begin{tabular}{c}
\includegraphics[width=0.5\linewidth]{banc_de_filtre.png}
\end{tabular}
\end{center}
\caption{Schéma d'un banc de filtres }
\label{fig:banc_de_filtre}
\end{figure}

On introduit de nouvelles notations pour décrire un banc de filtres. 
\begin{itemize}
\item $l$ est un indice qui compte les raies du spectre des trames. 
\item $f_l$ est la valeur de la fréquence associée à la raie~$l$. 
\item $m$ est un indice qui numérote les filtres utilisés dans le banc de filtres. 
\item $\ww{H}_m(f)$ est la réponse fréquentielle du filtre numéro $m$. 
\end{itemize}


La figure~\ref{fig:banc_de_filtre} schématise un banc de filtres. Le bas de la figure montre les réponses fréquentielles de $4$~filtres notés~$\ww{H}_1(f)$, 
$\ww{H}_2(f)$, $\ww{H}_3(f)$ et $\ww{H}_4(f)$. Le filtre~$\ww{H}_1$ est un passe-bas. Les filtres $\ww{H}_2(f)$ et~$\ww{H}_3(f)$ sont des filtres passe-bande.
Le filtre $\ww{H}_4(f)$ est un filtre passe-haut. Une particularité de ces filtres est que la somme de leur réponses fréquentielles est un filtre passe-tout 
généralement un simple filtre à retard dont le module de la réponse fréquentielle vaut~$1$. 

Dans la partie supérieure de la figure~\ref{fig:banc_de_filtre}, on retrouve à gauche les~$4$ filtres $\ww{H}_1(f)$, 
$\ww{H}_2(f)$, $\ww{H}_3(f)$ et $\ww{H}_4(f)$. Ces filtres reçoivent tous en entrée le signal $x(t)$, celui-ci est visualisé en haut à droite en noir. 
Le signal en bleu représenté juste en dessous est $y_1(t)$, c'est la sortie du filtre de réponse fréquentielle $\ww{H}_1(f)$. On observe que ce signal 
présente des variations de moindre amplitudes, c'est la conséquence de ce que $\ww{H}_1(f)$ est un passe-bas. 
Les signaux représentés en dessous en vert, rouge et cyan, sont notés $y_2(t), y_3(t), y_4(t)$. Ce sont respectivement les sorties des filtres
$\ww{H}_2(f)$, $\ww{H}_3(f)$ et $\ww{H}_4(f)$. On y retrouve des variations parfois significativement plus importantes. 
La décomposition du signal $x(t)$ en $4$ signaux $y_1(t), y_2(t), y_3(t), y_4(t)$ est appelé {\em analyse}, terme indiqué en bas à gauche de la figure~\ref{fig:banc_de_filtre}. Ces signaux, $y_1(t), y_2(t), y_3(t), y_4(t)$ sont ensuite additionnés pour former le signal visualisé en bas à droite en violet et noté 
$y_1(t)+y_2(t)+y_3(t)+y_4(t)$. Tel qu'on peut l'observer, ce signal est identique à $x(t)$. En réalité, ce dernier signal est généralement retardé par rapport 
à $x(t)$. Il est en effet impossible de réaliser une décomposition en banc de filtres avec des filtres causaux sans introduire un retard. 
La formation d'une reconstruction retardée de $x(t)$ à partir des signaux $y_1(t), y_2(t), y_3(t), y_4(t)$ s'appelle {\em synthèse}, ce qui est indiqué en 
bas du deuxième bloc. 

En regardant plus attentivement le bas de la figure~\ref{fig:banc_de_filtre}, on peut observer que les supports~\footnote{Par support, on entend ici l'intervalle sur lequel une fonction ici la réponse fréquentielle est non nulle.} des réponses 
fréquentielles des différents filtres ne sont pas disjoints, on dit que ces filtres se chevauchent. En fait l'allure même du signal $y_1(t)$ avec ces variations atténuées mais existantes laisse penser qu'il y a probablement un chevauchement assez important. Et en effet la notion de banc de filtre 
n'est pas du tout contradictoire avec un chevauchement même assez important. 
Pour la suite de ce document et pour plus de simplicité, on va considérer des bancs de filtres sans chevauchement où les réponses
fréquentielles sont en fait des portes définies par $\1_{[f_1,f_2]}(f)$. 

On dit qu'un banc de filtres suit une échelle linéaire lorsque les intervalles associés aux différentes portes caractérisant les réponses fréquentielles 
des filtres $\ww{H}_m(f)$ sont de longueur identiques. 
\beqn\boxed{
[f_{\min},f_{\max}]=\bigcup_{m}[f_m,f_{m+1}]\quad\mbox{où}\quad 
\left \{ \begin{array}{l}
f_{\min}=f_1,\,\,f_{\max}=f_{M+1}\\[0.3cm]
f_m=f_{\min}+(m-1)\frac{f_{\max}-f_{\min}}{M}\\[0.3cm]
\ww{H}_m(f)=\1_{[f_m,f_{m+1}]}(f)
\end{array}
\right. 
}
\eeqn

\begin{figure}
\begin{center}
\begin{tabular}{cc}
\includegraphics[width=0.5\linewidth]{fig9a.png}&
 \includegraphics[width=0.5\linewidth]{fig9b.png}
\end{tabular}
\end{center}
\caption{\`A gauche~: les courbes $\widehat{H}_m(f)$ en fonction de $f$ pour $m\in\{1,\ldots,8\}$ sont superposées
sur un même graphe.
 \`A droite~: ces courbes ont chacune leur abscisse.}
\label{fig9}
\end{figure}

La sensibilité de l'oreille humaine vis-à-vis de la décomposition fréquentielle d'un son et la façon dont les sons sont produits 
par les organes humains amènent à choisir pour les intervalles caractérisant les filtres $\ww{H}_m(f)$ une échelle logarithmique. 
Ce terme d'échelle logarithmique signifie que les intervalles sont de longueurs {\em croissantes} et que les bornes des ces intervalles 
suivent une loi {\em géométriques}. 
\beqn\boxed{
[f_{\min},f_{\max}]=\bigcup_{m}[f_m,f_{m+1}]\quad\mbox{où}\quad 
\left \{ \begin{array}{l}
f_{\min}=f_1,\,\,f_{\max}=f_{M+1}\\[0.3cm]
f_m=f_{\min}\left (\frac{f_{\max}}{f_{\min}}\right)^{\frac{m-1}{M}}\\[0.3cm]
%r=e^{\frac{\ln(f_{\max})-\ln(f_{\min})}{M}}=\left (\frac{f_{\max}}{f_{\min}}\right)^{\frac{1}{M}}\\[0.3cm]
\ww{H}_m(f)=\1_{[f_m,f_{m+1}]}(f)
\end{array}
\right. 
}
\eeqn

En pratique pour un banc de filtre suivant une échelle linéaire, on peut choisir $f_{\min}=0$ et $f_{\max}=\frac{f_e}{2}$, 
et pour une échelle logarithmique, il faut que $f_{\min}>0$, on peut choisir $f_{\min}=\frac{1}{T_K}$ et $f_{\max}=\frac{f_e}{2}$,
$T$ étant la durée de la trame.  

La figure~\ref{fig9} montre les réponses fréquentielles de huit filtres $\ww{H}_m$ qui suivent une échelle logarithmique, à gauche 
en les superposant sur un même graphe 2D et à droite en mettant chaque courbe le long d'un axe différent. 

\begin{figure}
\begin{center}
\begin{tabular}{cc}
\includegraphics[width=0.5\linewidth]{fig10a.png} &\includegraphics[width=0.5\linewidth]{fig10b.png}
\end{tabular}
\end{center}
\caption{\`A gauche~: superposition de l'évolution des descripteurs en fonction du temps. Chaque courbe
est associée à un filtre en particulier dont la légende indique la fréquence centrale associée à ce filtre.
\`A droite~: représentation séparée de l'évolution de chaque descripteur en fonction du temps.Dans les 
deux graphes, l'échelle en temps indique les instants associés aux milieux de chaque trame.}
\label{fig10}
\end{figure}

La figure~\ref{fig10} représente un exemple de représentation de ce descripteur temps-fréquence, 
il s'agit à gauche et à droite des courbes qui dans la figure~\ref{fig9} sont appelées $y_1(t), y_2(t), y_3(t), 
y_4(t)$. La différence est qu'ici il y en a $5$ et que les filtres utilisés ici ne se chevauchent pas. 
On observe des variations d'amplitudes plus faibles pour les quatre  premières 
par rapport à la dernière associées au fréquences plus élevées. 
Cependant il est significatif que la courbe bleue foncée, associée au filtre passe-bas et située au milieu sur le graphe de gauche et en 
haut à gauche sur le graphe de droite, a des variations qui sont d'une amplitude assez significatives, là 
on aurait pu s'attendre à des variations moins importantes. Cela traduit le fait que le signal 
sonore étudié présente des variations temporelles importantes d'une trame à une autre. 

Ces bancs de filtres servent à définir des descripteurs, un par filtre du banc de filtre.
De multiples descripteurs sont proposés dans la littérature scientifique. 
On aurait pu s'attendre à définir un descripteur comme la puissance sur une portion du signal en 
sortie du filtre $\ww{H}_m(f)$
autour de l'instant $t$.
\beqn\label{eq:desc_bf}
\boxed{
D_m(t)=\frac{1}{T}{\int_{-\frac{T}{2}}^{\frac{T}{2}} |h_m(\tau)\ast x_t(\tau)|^2\,d\tau}
\quad \mbox{ où }\quad \left \{ \begin{array}{l}
h_m(\tau)\mbox{ est la réponse impulsionnelle du filtre }\ww{H}_m(f)\\[0.3cm]
x_t(\tau)=x(\tau+t)\1_{\left [-\frac{T}{2},\frac{T}{2}\right]}(\tau)
\end{array}
\right . 
}
\eeqn

Mais comme la perception de l'intensité sonore est mieux corrélée à une intensité mesurée en décibel et donc 
suivant une échelle logarithmique vis-à-vis de la puissance, il convient d'ajouter un logarithme dans l'équation~(\ref{eq:desc_bf}).
La littérature scientifique a fait le choix d'utiliser un autre descripteur dont une version en temps continu serait 
\beqn
\sm{D\_LOG}_m(t)=\frac{1}{f_{m+1}-f_m}\,{\int_{f_m}^{f_{m+1}} 10\log_{10} \left |\ww{H}_m(f) \ww{X}_t(f)\right|^2\,df}
\eeqn
Et en pratique, le descripteur utilisé, dépend de deux paramètres, $m$ pour le filtre et par 
suite la fréquence associée à ce filtre, et $k$ pour la trame considérée. 

Le descripteur utilisé dans les travaux pratiques 
a pour nom {\tt LOG\_MAG\_FB\_LOG}~\footnote{La signification du nom se retrouve en lisant 
l'expression de droite à gauche. {\tt LOG} en dernier signifie qu'on considère une échelle logarithme, puis 
que cette échelle permet de définir un banc de filtre ({\em filter bank}), qu'on calcule ensuite le module ({\em magnitude}) 
et qu'avant de considérer la moyenne on considère le logarithme des modules.}

En pratique, le descripteur est ainsi défini.
\beqn
\boxed{
\sm{LOG\_MAG\_FB\_LOG}(m,k)=
\frac{1}{\left |\bb{L}_m\right |}
{\sum_{l\in \bb{L}_m} 10\log_{10}\left |\widehat{H}_{m,l}\widehat{X}_{k,l}\right|^2}
}
\eeqn
où $\bb{L}_m$ désigne les indices $l$ pour lesquels $\widehat{H}_{m}\left(\frac{lf_e}{N_K}\right)$ est non-nul, 
ce sont a priori les indices $l$ pour lesquels la fréquence $\frac{lf_e}{N_K}$ sont contenus dans 
$\left [f_m,f_{m+1}\right]$. 
$|\bb{L}_m|$ désigne le nombre d'indices $l$ contenus dans $\bb{L}_m$. 

Remarquons que le fait de modifier un descripteur en le multipliant par une certaine constante ou 
en lui ajoutant une constante n'a aucune incidence sur la classification qui en résulte. 


%\section{Conclusion}

D'autres suggestions de descripteurs pour la reconnaissance de la parole se trouvent dans~\cite{Rabiner93}.


\include{annexe_son}
\end{document}


==> sedpyFLL0 <==

\newcommand{\msm}{$\mbox{m}.\mbox{s}^{-1}$}
\newcommand{\de}{{({\mbox{\small de}})}}
\newcommand{\moy}{{({ \mbox{\small moy})}}}
\newcommand{\der}{{({ \mbox{\small fin}})}}
\newcommand{\ce}{{({ \mbox{\small ce}})}}
\newcommand{\PMCT}{{\mbox{PMCT}}}
\newcommand{\arr}[1]{\rotatebox[origin=c]{#1}{$\xrightarrow{\hspace{1cm}}$}}
\newcommand{\fr}[1]{\framebox{#1}}
\newcommand{\bz}{{\mathbf z}}
\newcommand{\deux}{{\text{\tiny{|2}}}}     


\DeclareMathOperator{\OA}{OA}

\title{
Introduction à la reconnaissance de la parole  \\
}
\author{{\small Gabriel Dauphin}}


\begin{document}




%\pagenumbering{Alph}

%\pagenumbering{arabic}

\maketitle
\tableofcontents


\chapter*{Introduction}

Ce cours présente un ensemble de techniques qui sont utilisées en travaux pratiques 
pour distinguer les sons correspondant aux mots {\tt un}, {\tt deux} et {\tt trois}. 
Ces techniques utilisent la notion de description temps-fréquence qui est implicite dans la 
décomposition d'un son en trames, explicite dans la notion de {\tt spectrogramme} et qui est 
utilisée dans les différents descripteurs présentés dans le chapitre~\ref{ch:desc}.
Le chapitre~\ref{ch:traitement_son} a pour objectif de décrire la façon des sons sont représentées, cela amène 
à décrire brièvement les organes humains de la perception et le prétraitement qui est appliqué 
aux données associées aux sons. 
Le chapitre~\ref{ch:classification_par_descripteurs} a pour objectif de présenter la classification, à savoir son objectif, la façon dont on l'évalue et 
la manière dont elle utilise des valeurs calculées pour chaque son  que l'on appelle ici {\em descripteur}. 
Le chapitre~\ref{ch:desc} présente différentes techniques permettant de calculer les valeurs de descripteurs à partir des données 
associés aux sons. Cela amène à décrire brièvement les organes humains de la génération d'un son car cela explique 
l'intérêt porté à l'utilisation d'une description fréquentielle de portions de signaux temporels. 

En tant que document de cours, il a pour objectif de préciser les notions à connaître. Les notions 
à connaître le plus précisément sont la compréhension et la connaissance des {\em formules encadrées}, la compréhension 
des {\em graphiques et schémas} présentés et la connaissance et la signification des {\em termes techniques}. 





\chapter{Représentation d'un son}
\label{ch:traitement_son}

Pour décrire et discuter de la façon dont les sons sont représentées, la 
section~\ref{sec:questce_quun_son} discute de ce qu'est physiquement un son et donne 
une brève description des organes humains utilisées pour la perception d'un son. 
La section~\ref{sec:son_temps} rappelle comment le traitement numérique du signal permet 
de représenter un son.
La section~\ref{sec:N:son_trames} montre une façon un peu différente de représenter le son au moyens 
de {\em trames}, c'est-à-dire de petites portions du signal sonore. 
La section~\ref{sec:detection_silence} montre une façon simplifiée de détecter les phases de silence et de paroles, 
il se trouve que ceci était un des objectifs de ce cours. Cette détection est utilisée pour réaliser un 
prétraitement permettant d'améliorer la performance de la classification. 
La section~\ref{sec:implementation} donne quelques indications sur la façon dont les techniques proposées sont implémentées
dans les travaux pratiques qui illustre ce cours. 



\section{Qu'est-ce qu'un son~?}
\label{sec:questce_quun_son}


La section~\ref{ssec:model_physique} présente une description du son en tant qu'onde sonore se propageant 
dans l'air. 
La section~\ref{ssec:oreille} présente une très brève description du fonctionnement de l'oreille 
en tant qu'organe de perception des sons. 
La section~\ref{ssec:audibilite} présente des courbes d'audibilité, c'est-à-dire les seuils hauts et bas 
de perception du son. 


\subsection{Modélisation physique}
\label{ssec:model_physique}
Un son est généralement décrit comme plus ou moins aigu ou plus ou moins fort. Nous allons voir
que la première notion correspond à une fréquence et la deuxième à un niveau sonore. 

Le son est une variation de la pression de l'air.~\footnote{Un son peut aussi se propager à travers d'autres matériaux et dans ce cas 
c'est le matériau traversé qui se met à vibrer, en revanche le son ne peut pas se propager à travers le vide.}
Cette variation se propage sous la forme d'une onde. Une modélisation sphérique de cette onde est décrite par 
\beqn\label{eq:propag_onde}
P(r,t)=P_0+\frac{1}{r}\left [g_1(t-\frac{r}{c})+g_2(t+\frac{r}{c})\right ]
\eeqn
\begin{itemize}
\item $P_0$ est la pression atmosphérique moyenne. L'unité dans laquelle elle s'exprime est le Pa (Pascal). La pression de l'air est environ $10^5$Pa.
\item $r$ est la distance en mètres (m) entre le point où on mesure la pression et la  source de ce signal sonore. 
\item $t$ est l'instant en secondes~(s) pour lequel on mesure la pression $P(r,t)$. 
\item $c$ est la vitesse ($\mbox{m}.\mbox{s}^{-1}$) de propagation du son à travers l'air. C'est environ de $340$\msm. 
\item $g_1$ et $g_2$ peuvent a priori être des fonctions quelconques. Pour modéliser la propagation d'un signal sonore, on 
considère $g_2=0$ et pour un son stationnaire par exemple dans une caisse de résonnance, $g_1$ et $g_2$ sont similaires. 
\end{itemize}

Pour modéliser une note de musique qui dure un temps infini, on utilise 
\beqn
\boxed{
g_1(\tau)=\cos(2\pi f_0\tau)
}
\eeqn
Cette note est caractérisée par sa fréquence $f_0$ en Hz. 
En effet, avec cette modélisation on observe que $P(r,t+\frac{1}{f_0})=P(r,t)$, 
c'est-à-dire qu'en chaque point la pression évolue dans le temps avec une périodicité de $\frac{1}{f_0}$. 
{\small 
\beqns
P(r,t+\frac{1}{f_0})=P_0+\frac{1}{r}\cos(2\pi f_0(t+\frac{1}{f_0}-\frac{r}{c}))
=P_0+\frac{1}{r}\cos(2\pi f_0(t-\frac{r}{c}))=P(r,t)
\eeqns
}
Et $f_0$ est reliée à une longueur d'onde notée $\lambda_0$ mesurée en mètres.
\beqn\label{eq:long_onde}
\boxed{
\lambda =\frac{c}{f_0}
}
\eeqn
Ceci traduit une évolution quasi-périodique du signal dans l'espace $P(r+\lambda,t)\approx P(r,t)$. 
{\small 
\beqns
P(r+\lambda,t)=P_0+\frac{1}{r+\lambda}\cos(2\pi f_0(t-\frac{r}{c}-\frac{\lambda}{c}))
=P_0+\frac{1}{r+\lambda}\cos(2\pi f_0(t-\frac{r}{c}))\approx P(r,t)
\eeqns
}
\`A l'oreille, ce son apparaît comme une note de musique. Il s'agit d'un La lorsque $f_0=440$Hz. 
Cette fréquence est donc liée au caractère plus ou moins aigu du son. 

L'intensité sonore d'un son correspond au produit de la surpression par la vitesse. Dans le cadre de ce cours, 
on considère qu'il s'agit du carré de la partie variable de la pression. 
\beqns
I=\left (P(r,t)-P_0\right )^2
\eeqns
Cette intensité sonore est en Watt par mètres carrés ($\mbox{W}.\mbox{m}^{-2}$).
Dans le cadre de ce cours, on attache de l'importance au fait que cette intensité sonore est proportionnelle à $\frac{1}{r^2}$. 
\beqn
\boxed{
I=\frac{I_e}{r^2}
}
\eeqn
$I_e$ étant une quantité inconnue à estimer. 
Aussi lorsqu'on s'éloigne de la source en doublant la distance, l'intensité sonore est divisée par $4$. 

On appelle niveau sonore, le fait d'utiliser une échelle en décibel pour mesurer l'intensité sonore. 
\beqn\label{eq:N:niveau_sonore}
\boxed{
L=10\log_{10}\left (\frac{I}{I_0}\right )
}
\eeqn
où $I_0$ est une intensité sonore de référence. On peut remarquer que dans l'équation~(\ref{eq:N:niveau_sonore}), 
l'échelle en décibel n'est pas calculé avec un facteur multiplicatif de $20$ mais de $10$, parce que l'intensité sonore est 
déjà un terme carré. Et en effet lorsqu'on s'éloigne d'une source sonore en multipliant par deux la distance, 
le niveau sonore est diminué de $10\log_{10}(4)=6$dB.~\footnote{C'est en effet la même diminution que pour 
le rapport signal sur bruit, si on divisait par deux le bruit sans modifier le signal source.}

\subsection{Fonctionnement schématique de l'oreille}
\label{ssec:oreille}

\begin{figure}
\begin{center}
\begin{tabular}{c}
\includegraphics[width=0.5\linewidth]{oreille.png}
\end{tabular}
\end{center}
\caption{Schéma détaillé de l'oreille.}
\label{fig:N:oreille}
\end{figure}
	

La figure~\ref{fig:N:oreille} (extraite d'une publication) 
représente un schéma détaillé de l'oreille. Schématiquement, le son s'introduit dans le conduit auditif, 
fait vibrer le tympan qui actionne le marteau, l'enclume et l'étrier qui à son tour fait vibrer le liquide présent dans la cochlée. 
Cette cochlée est tapissée de cellules ciliées qui transmettent les vibrations vers des nerfs auditifs. Les cellules au début 
de la cochlée sont sensibles aux sons aigus tandis que celles en fin de cochlée sont sensibles aux sons graves. 

\subsection{Courbes d'audibilité humaine}
\label{ssec:audibilite}

\begin{figure}
\begin{center}
\begin{tabular}{c}
\includegraphics[width=0.5\linewidth]{courbe_audibilite.png}
\end{tabular}
\end{center}
\caption{Courbe d'audibilité humaine.}
\label{fig:N:courbe_audibilite}
\end{figure}
	
Dans la figure~\ref{fig:N:courbe_audibilite} (extraite d'une publication), l'échelle des ordonnées est le niveau sonore d'un son écouté. L'échelle 
des abscisses est une échelle de fréquences (Hz) mais avec une distribution logarithmique. \`A gauche ce sont les infrasons qui
correspondent aux sons qu'on ne peut entendre parce que leur fréquence est trop basse. \`A droite ce sont les ultrasons 
qu'on ne peut pas non plus entendre parce que leur fréquence est trop haute. Entre ces deux fréquences, il y a deux courbes, 
si le niveau sonore d'un son est supérieur à la limite donnée par la courbe inférieure alors on peut l'entendre et s'il 
est supérieur à la limite donnée par la courbe supérieure alors ce son peut abîmer l'oreille. 
Ces courbes sont obtenues en expérimentant sur un grand nombre de patients, elles indiquent un sensibilité moyenne, mais 
il y a en réalité des différences importantes d'un individu à un autre. 
Ces courbes nous amènent à affirmer qu'une assez grande partie de l'information sonore est obtenue en ne considérant 
que les fréquences inférieures à $4$kHz et qu'a priori la totalité de l'information sonore est obtenue en 
ne considérant que les fréquences inférieures à $20$kHz. 


\section{Représentation temporelle d'un son}
\label{sec:son_temps}


\begin{figure}
\begin{center}
\begin{tabular}{c}
\includegraphics[width=0.5\linewidth]{son_temps.png}
\end{tabular}
\end{center}
\caption{Représentation temporelle du signal sonore.}
\label{fig:N:son_temps}
\end{figure}
	
	
En tant qu'onde sonore, un son est un signal temps continu à valeurs continus. Mais lorsqu'il est 
converti en signal électrique avec un capteur acoustique appelé microphone puis converti en signal numérique avec 
échantillonnage et quantification, le signal devient temps discret. 
Du fait du critère de Shannon-Nyquist, la fréquence d'échantillonnage $f_e$ est entre $40$kHz et $50$kHz (en général 
$44.1$kHz mais, 
elle peut parfois être de $8$kHz. Le signal est souvent quantifié sur $8$ bits, mais cela peut être $10$ ou $12$ bits. 
Le signal échantillonné est noté $x_n$, chaque indique $n$ correspondant à un instant $t_n=nT_e$ où $T_e=\frac{1}{f_e}$.
La figure~\ref{fig:N:son_temps} (extraite d'une publication), indique l'évolution au cours du temps de l'intensité sonore. 
En ordonnée, il n'y a pas d'unité, c'est a priori une fraction de la valeur maximale. Mais le carré du signal est proportionnel à l'intensité sonore. 
Le signal représenté est celui obtenu en enregistrant la phrase {\em Le metteur en scène termine le scénario.} 



On appelle {\em durée} du signal, le temps qui s'écoule entre le début 
du signal sonore et la fin. Cette durée est égale à $NT_e$ où ici $N$ est 
le nombre d'échantillons~\footnote{\'Etant donné 
la valeur de $f_e$, il est tout à fait satisfaisant d'approcher cette durée 
à un multiple de $T_e$.} représenté sur la figure~\ref{fig:N:son_temps}. 
\'Etant donné la valeur élevée de $f_e$, on a en fait un très grand nombre d'échantillons, 
bien plus qu'il n'est possible de distinguer à l'oeil en observant la figure. L'allure générale permet aussi de distinguer les
 moments où il y a du silence, des moments où 
il y a un signal sonore important~: le silence correspond à des valeurs très faibles en valeur absolues et le signal sonore important correspond à des 
valeurs importantes du signal. 
Comme chaque intervalle de temps dans le graphe correspond aussi à un intervalle de 
temps durant lequel un son est prononcé, il est possible de faire correspondre chaque syllabe à un morceau du signal. On peut ainsi visualiser pour certaines sons des particularités, le premier {\em t} et les deux {\em s} correspondent à des parties très foncées du graphe. 

Bref, cette représentation temporelle du signal suggère l'étude séparée de chaque morceau de signal correspondant à un son ou à une syllabe. Mais comme on ne connaît 
pas a priori quand commence et quand finit le son ou la syllabe, la 
section~\ref{sec:N:son_trames} montre que l'on découpe le signal en une succession
de trames. 

Les notations utilisées pour décrire l'ensemble du signal sont les suivantes. 
\begin{itemize}
\item $T$ durée du signal en secondes.
\item $N$ nombre total d'échantillons.
\item $t_n=nT_e$ échelle de temps du signal pour $n\in\{0\ldots N-1\}$. 
\end{itemize}
On a la relation entre durée du signal et période d'échantillonnage. 
\beqn
\boxed{
T=NT_e
}
\eeqn
On a aussi l'échantillonnage du signal.
\beqn
\boxed{
x_n=x(t_n)
}
\eeqn


Pour illustrer des notions traitement du signal, on s'interroge ici sur la façon 
de rendre un son plus grave au moyen d'un traitement numérique du vecteur $x_n$. 
\begin{itemize}
\item En diminuant $f_e$, le son est plus grave. 
Mais sa durée est aussi diminuée d'autant puisqu'elle est égale à $\frac{N}{f_e}$. 
\item Si on effectue un sur-échantillonnage tout en conservant la fréquence 
d'échantillonnage alors le son devient plus grave mais sa durée est 
augmentée d'autant. 
\item Si on effectue une modulation, c'est-à-dire qu'on multiplie le graphe
par une sinusoïde d'une certaine fréquence alors on déplace effectivement 
le son à la fois en le rendant plus aigu et plus grave. Si ce son a un spectre
très étroit alors il est possible de supprimer la composante aigüe ou la composante grave. Et la durée est alors inchangée.  
\end{itemize}


\section{Représentation du signal sonore en une succession de trames}
\label{sec:N:son_trames}

\subsection{Découpage en trames sans chevauchement}

\begin{figure}
\begin{center}
\begin{tabular}{c}
\includegraphics[width=0.8\linewidth]{son_trames_simples.png}
\end{tabular}
\end{center}
\caption{Découpage d'une sinusoïde en trames qui ne se chevauchent pas.}
\label{fig:N:son_trames_simples}
\end{figure}
	
La figure~\ref{fig:N:son_trames_simples} donne quatre représentation 
d'un même signal défini par 
\beqns
x_n=\sin(20\pi nT_e)
\eeqns
C'est le signal représenté en haut à gauche de cette figure où sur une seconde, il
y $10$ périodes de la sinusoïde qui sont répétées et où donc, la fréquence de la 
sinusoïde est de $10$Hz et la période $T=0.1$s. L'échelle des ordonnées est 
une fraction de l'amplitude maximale. L'échelle des abscisses est la seconde. 

Dans cet exemple, on découpe le signal d'une seconde en $10$ trames chacune 
dure ici $0.1$s. La figure en haut à droite représente chaque trame avec une couleur 
différente~: bleu pour la première trame, vert pour la deuxième, rouge pour la troisième, cyan pour la quatrième, violet pour la cinquième, etc...

Le graphe en bas à gauche est une autre représentation de ces trames. L'axe pointant vers la droite est le temps écoulé depuis le début de chaque trame. 
L'axe pointant vers la gauche et commençant à zéro au milieu indique le numéro 
de la trame considérée. L'axe vers le haut indique la valeur du signal pour la trame considérée à l'instant de la trame considérée. La valeur zéro est ici à mi-hauteur. Ici la couleur ne distingue plus les trames entre elles, elle dépend de la valeur prise par le signal. Dans cet exemple le signal est identique sur chaque trame, c'est pour cela qu'on retrouve exactement le même signal sur chaque courbe. 

La courbe en noir du graphe en bas à droite est la même que le graphe en haut à gauche, il s'agit du signal $x_n$ représenté en fonction du temps. Sur ce graphe, il y a en plus des traits horizontaux de couleurs et de hauteurs différentes
qui permettent d'identifier chaque trame. Ce sont ces traits qui permettent de lire 
les instants associés au début et à la fin de chaque trame en trouvant l'abscisse 
du début et de la fin du trait horizontal. 

\subsection{Notations pour définir les trames}

On utilise ici les notations suivantes. Ces notations ne sont pas 
universelles, il est donc nécessaire de les redéfinir quand on les utilise. 
\begin{itemize}
\item $K$ désigne le nombre de trames. 
\item $T_K$ est la durée d'une trame. 
\item $N_K$ est le nombre d'échantillons dans une trame, il est identique pour toutes les trames d'un même son.
\item $k\in \{0\ldots K-1\}$ est un indice qui identifie la trame. 
\item $t_k^\de$ instant associé au premier échantillon de la trame $k$.
\item $t_k^\der$ instant associé au dernier échantillon de la trame $k$. 
\item $t_k^\ce$ instant associé au centre de la trame $k$. 
\item $t_{k,n}$ échelle de temps associée à la trame $k$ donnant 
les instants associées aux échantillons $n=0$ jusqu'à $n=N_K-1$. 
\end{itemize}

Du fait qu'il n'y a pas de chevauchement, on a
\beqn\label{eq:N:T_K}
\boxed{
T_K=\frac{T}{K}\mbox{ et }N_K=\frac{N}{K}
}
\eeqn

D'une façon générale, le début, le centre et la fin d'une trame 
$k$
sont définies par
\beqn\label{eq:N:t_k_de}
\boxed{
\mbox{Pour }k\in\{0\ldots K-1\},\quad\left \{
\begin{array}{l}
t_k^\de=k\frac{T}{K}\\[0.2cm]
 t_k^\der=t_k^\de+T_K-T_e\\[0.2cm]
t_k^\ce=\frac{1}{2}\left (t_k^\de+t_k^\der\right )
\end{array}
\right. 
}\eeqn

Avec ces définitions et pour une trame $k$, on peut définir une échelle de temps et déterminer les valeurs du signal
\beqn\label{eq:N:ech_temps_trame}
\boxed{
\begin{array}{c}
\mbox{Pour }k\in\{0\ldots\}\mbox{ et }n\in \{0\ldots N_K-1\}\\[0.5cm]
t_{k,n}=t_k^\de+nT_e \mbox{ et }x_{k,n}=x(t_{k,n})=x\left[\frac{t_{k,n}}{T_e}\right ]
\end{array}
}
\eeqn
Dans la dernière expression en bas à droite de l'équation~(\ref{eq:N:ech_temps_trame}), l'expression entre crochet est un indice 
\beqns
n'=\frac{t_{k,n}}{T_e}=k\frac{N}{K}+n
\eeqns
et cet indice est utilisé pour retrouver dans le signal $x_n$ la valeur recherchée 
$x_{k,n}=x_{n'}$. 


\subsection{Découpage en trames avec chevauchement}

\begin{figure}
\begin{center}
\begin{tabular}{c}
\includegraphics[width=0.8\linewidth]{son_trames_chevauchement.png}
\end{tabular}
\end{center}
\caption{Découpage d'une sinusoïde en trames qui se chevauchent.}
\label{fig:N:son_trames_chevauchement}
\end{figure}


\`Etant donné un nombre total d'échantillons $N$, un nombre de trames $K$ et 
du choix de chevauchement utilisé, on a les deux propriétés suivantes. 
\begin{itemize}
\item Les instants de débuts des trames ne sont pas modifiées.
\beqn
\boxed{
t_k^\de=k\frac{T}{K}
}
\eeqn
\item La longueur des trames est augmenté d'un facteur $\frac{1}{1-\alpha}$. 
\beqn\label{eq:N:T_K_alpha}
\boxed{
T_K=\frac{T}{K}\frac{1}{1-\alpha}\mbox{ et }N_K=\frac{N}{K}\frac{1}{1-\alpha}
}
\eeqn
\item Hormis la première trame, toutes les trames partagent avec la précédente
$\alpha N_K$ échantillons. Et hormis la dernière trame, toutes les trames partagent avec la suivante $\alpha N_K$ échantillons. 
\end{itemize}


La dernière affirmation se calcule ainsi pour $k\in\{0\ldots K-1\}$
\beqns
t_k^\der-t_{k+1}^\de+T_e=\left (k\frac{T}{K}+\frac{T}{K}\frac{1}{1-\alpha}-T_e\right ) -(k+1)\frac{T}{K}+T_e=\frac{T}{K}\left (\frac{1}{1-\alpha}-1\right )
=\alpha T_K
\eeqns


Ainsi les équations (\ref{eq:N:t_k_de}) et (\ref{eq:N:ech_temps_trame})
ne sont pas modifiées quand on met un chevauchement. En revanche l'équation~(\ref{eq:N:T_K})
est remplacée par l'équation~(\ref{eq:N:T_K_alpha}).

Lors de l'implémentation, ces formules ont été un peu modifiées pour tenir 
compte de ce que le découpage en trames ne tombe pas exactement sur un échantillon 
et qu'il faut donc commencer à partir de l'échantillon le plus proche. 

\section{Signaux sonores et silences}
\label{sec:detection_silence}
\subsection{Puissance moyenne à court terme}
\label{ssec:PMCT}


\begin{figure}
\begin{center}
\begin{tabular}{c}
\includegraphics[width=0.8\linewidth]{son_puissance.png}
\end{tabular}
\end{center}
\caption{Signal temps discret représentant un signal sonore commençant et terminant par un silence.}
\label{fig:N:son_puissance}
\end{figure}

En traitement du signal, on définit une puissance moyenne qui évolue dans le temps
qui est appelée puissance moyenne à court terme. 
Cela se fait en introduisant une fenêtre notée $w_T$ qui est un signal temps 
continu de durée $T$ centré en zéro. 
La notion de fenêtre a déjà été présentée lors du cours sur la 
synthèse des filtres numérique à réponse impulsionnelle finie avec notamment la fenêtre rectangulaire et triangulaire. 
\`A temps continu, la fenêtre rectangulaire de largeur $T$ est ainsi définie.
\beqns
w_T(\tau)=\1_{\left [-\frac{T}{2},\frac{T}{2}\right]}(\tau)
\eeqns
La fenêtre triangulaire de largeur $T$ est ainsi définie.
\beqns
w'_T(\tau)=\left (1-\frac{2t}{T}\right)\1_{\left [-\frac{T}{2},\frac{T}{2}\right]}(\tau)
\eeqns
Ici la fenêtre est utilisée, non pour modifier une réponse impulsionnelle mais un signal, ici $x^2(t)$. L'action de la fenêtre 
porte sur l'intervalle de temps centré en $t$. Aussi elle est d'abord centrée en $t$ puis normalisée.
\beqns
w_T(\tau)\mapsto w_T(t-\tau)\mapsto \frac{1}{\int_\Rr w_T(t-\tau)\,d\tau}\,w_T(t-\tau)
\eeqns
Ainsi modifiée la fenêtre est ensuite multipliée par $x^2(\tau)$
\beqns
x^2(\tau)\mapsto x^2(\tau)\frac{1}{\int_\Rr w_T(t-\tau)\,d\tau}\,w_T(t-\tau)
\eeqns

Cette puissance moyenne à court terme, notée $\sm{PMCT}$~\footnote{{\tt PMCT}
est défini dans \cite{Camastra07} p.~41-42.}~\footnote{Une interprétation en terme d'énergie
existe dans page~3, section~2.1 dans~\cite{Peeters04}.}
 est 
\beqn\label{eq:PMCT_TC}
P(t)=\frac{{\int_\Rr {x^2(\tau)w_T(t-\tau)\,d\tau }}}{{\int_\Rr w_T(\tau)\,d\tau}}
\eeqn
Avec une fenêtre rectangulaire, $P(t)$ devient 
\beqn\label{eq:PMCT_TC_rect}
\boxed{
P(t)=\frac{1}{T}{\int_{t-\frac{T}{2}}^{t-\frac{T}{2}} x^2(\tau)\,d\tau}
}
\eeqn


Ici le découpage en trame du signal se prête justement à un calcul très similaire.
\begin{itemize}
\item $T$ est remplacée par la longueur de la trame $T_K$ qui compte $N_K$ échantillons. 
\item $t$ est remplacée par $t_k^\ce$, le milieu de la trame $k$ qui se trouve à peu près à l'échantillon $\frac{N_K}{2}$ de 
la trame $k$. 
\end{itemize} 
 Cela permet ainsi d'approcher la  discrétisation de l'équation~(\ref{eq:PMCT_TC}).
\beqn
\PMCT_k=\frac{{\sum_{n=0}^{N_K-1} x_k^2[n]w_{N_K}[n-\frac{N_K}{2}]}}{{\sum_{n=0}^{N_K-1} w_{N_K}[n-\frac{N_K}{2}]}}
\eeqn
où $w_{N_K}[n]$ est une fenêtre de support $\{-\frac{N_K}{2}\ldots \frac{N_K}{2}\}$ {\bf mais} avec des indices allant de $0$ à $N_K-1$.  

Avec une fenêtre rectangulaire, 
\beqn
\boxed{
\PMCT_k=\frac{1}{N_K}
{\sum_{n=0}^{N_K-1} x_k^2[n]}
}
\eeqn


\subsection{Détection du début et de la fin d'un signal sonore.}
\label{ssec:det_deb_fin_son}

La figure~\ref{fig:N:son_puissance} montre un exemple de signal sonore commençant et terminant par un silence. 
On souhaite dans cet exemple retrouver l'instant à partir duquel le signal sonore commence et l'instant auquel ce
 signal sonore s'arrête. 


On se donne un seuil, il est ici fixé à $10\%$ de la valeur maximale.
\beqn\label{eq:seuil}
\boxed{
s_e=\frac{1}{10}\max_k({\PMCT_k})
}
\eeqn
Ce seuil est utilisé pour déterminer deux numéros de trames~: $k^\de$ la première trame pour laquelle la puissance $\PMCT_k$ est supérieure 
$s_e$ et $k^\der$ la dernière  pour laquelle ceci est vrai. 
\beqn
\boxed{
k^{\de}=\underset{k}{\min}\,\{k|\,\PMCT_k>s_e\}
\mbox{ et }
k^{\der}=\underset{k}{\max}\,\{k|\,\PMCT_k>s_e\}
}
\eeqn
Les instants $t^\de$ et $t^\der$ associés au début et à la fin du signal sonore sont les centres des trames $k^\de$ et $k^\der$. 
\beqn
\boxed{
\left\{\begin{array}{l}
t^{\de}=t_{k}^{\ce}\mbox{ avec }k=k^{\de}\\[0.3cm]
t^{\der}=t_k^{\ce}\mbox{ avec }k=k^{\der}
\end{array}
\right . 
}
\eeqn
où $t_k^{\ce}$ désigne l'instant associé au centre de la trame $k$. 

\subsection{Normalisation d'un signal sonore}

La normalisation du signal a pour but de rendre comparable 
un son qui serait prononcé de façon forte et un son prononcé à voix plus basse. 
Cette normalisation consiste à imposer que la puissance moyenne soit fixe et en l'occurrence égale à $1$, mais 
cette étape se fait après avoir retiré les silences du signal.~\footnote{Si on effectuait cette normalisation du 
signal avant de retirer les silences, un son avec beaucoup de silences 
que l'on aurait normalisé  avec ses silences, aurait une 
puissance moyenne plus forte, une fois retirés les silences.}


Pour comparer les signaux, il est souhaitable que les signaux soient comparable en terme de puissance moyenne. Cette moyenne étant calculée sans considérer les silences. 
Pour obtenir que les signaux soient comparés, on effectue une {\em normalisation}, c'est-à-dire qu'on chacun des signaux par une valeur appropriée. 
Cette valeur est déterminée avec les étapes suivantes. 
\begin{itemize}
\item On utilise la technique de détection du début et de fin du signal sonore présentée en section~\ref{ssec:det_deb_fin_son}. 
\item On calcule la puissance moyenne en ne considérant que les trames qui se situent entre la première et la dernière des trames associées au signal sonore. 
On note $\bb{K}$ l'ensemble des trames où le son est plus fort que le seuil fixé par l'équation~(\ref{eq:seuil})
et $|\bb{K}|$ le nombre de ces trames. 
\beqns
\boxed{
P_\moy=\frac{1}{|\bb{K}|}{\sum\limits_{k\in \bb{K}} \sm{PMCT}_k}
}
\eeqns
\item La normalisation consiste à multiplier le signal par $\frac{1}{\sqrt{P_\moy}}$. 
\beqn
\boxed{
x_n\mapsto \frac{1}{\sqrt{P_\moy}} x_n
}
\eeqn
\end{itemize}


\section{Indications sur l'implémentation proposée}
\label{sec:implementation}

\begin{figure}
\begin{center}
\begin{tabular}{c}
\includegraphics[width=0.6\linewidth]{projet_son1.png}
\end{tabular}
\end{center}
\caption{Organisation des données dans l'implémentation}
\label{fig:N:projet_son1}
\end{figure}

Dans la simulation proposée, le répertoire principal est subdivisé en {\tt prg} contenant les programmes Matlab (fichiers {\tt .m} ou {\tt .p}) et {\tt donnee} qui contient 
les fichiers audio répartis en trois répertoires  {\tt un},  {\tt deux } et {\tt trois}. 
Cette organisation est schématisée sur la figure~\ref{fig:N:projet_son1}.


\chapter{Obtenir une classification grâce à des descripteurs}
\label{ch:classification_par_descripteurs}

L'objectif au cours de la séance de TP correspondante est de classer les sons à partir de descripteurs. Un descripteur peut 
soit être une valeur pour l'ensemble du signal, soit un ensemble de valeurs, une pour chaque trame.
On suppose dans cette partie qu'on dispose d'un certain nombre de descripteurs qui nous donnent des valeurs, une valeur par trame. 
La classification des sons est alors exposée en trois parties. 
La section~\ref{sec:distance_entre_sons} permet à partir de descripteurs d'évaluer numériquement 
une similarité entre deux sons. En fait on parle plutôt de distance entre sons, la distance correspondant ici à un défaut de similarité. 
une distance entre deux sons. 
La section~\ref{sec:knn} permet à partir de distances entre sons de prédire l'identité d'un son quelconque, 
c'est-à-dire s'il ressemble plus à un son de type {\tt un}, {\tt deux} ou {\tt trois}. 
Enfin la section~\ref{sec:evaluation_classification} montre comment on évalue généralement un classifieur. 


%\fbox{\begin{minipage}{0.8\linewidth}
%\imp
%Des descripteurs sont disponibles en utilisant la fonction {\tt traitement}. 
%\end{minipage}}

\section{Calcul d'une distance entre deux sons}
\label{sec:distance_entre_sons}



\begin{figure}
\begin{center}
\begin{tabular}{c}
\begin{tikzpicture}
[node distance = 10mm,thick, main/.style = {draw, circle},
  rect/.style={draw,rectangle,fill=green!50},rect_y/.style={draw,rectangle},
  minimum size=0mm]
	\node (H1) {};
	\node (L1)[below of=H1] {};
	\node (L11) [below of=L1] {};
		\node (L12) [below of=L11] {};
		\node (L13) [below of=L12] {};
		\node (L14) [below of=L13] {};
	  \node (sons) [right of=L1] {sons}; 
		\node[rect_y] (xn) [below of=sons] {$x_a[n]$};   
		\node (xmn) [below of=xn] {};  
		\node[rect_y] (xpn) [below of=xmn] {$x_b[n]$};  
		\node (L2) [right of=sons] {};
	  \node (trames) [right of=L2] {trames}; 
		\node[rect_y] (xkn) [below of=trames] {$x_a[k,n]$};   
		\node (xmkn) [below of=xkn] {};  
		\node[rect_y] (xpkn) [below of=xmkn] {$x_b[k,n]$};  
		\node (L3) [right of=trames] {};
		\node (sans_silence) [right of=L3] {$\begin{array}{c}\mbox{sans le}\\ \mbox{silence}\end{array}$}; 
		\node[rect_y] (xkn1) [below of=sans_silence] {$x_a[k,n]$};   
		\node (xmkn1) [below of=xkn1] {};  
		\node[rect_y] (xpkn1) [below of=xmkn1] {$x_b[k,n]$};  
		\node (L4) [right of=sans_silence] {};
		\node (normalisation) [right of=L4] {$\begin{array}{c}\mbox{normali-}\\ \mbox{sation}\end{array}$}; 
		\node[rect_y] (xkn2) [below of=normalisation] {$x_a[k,n]$};   
		\node (xmkn2) [below of=xkn2] {};  
		\node[rect_y] (xpkn2) [below of=xmkn2] {$x_b[k,n]$};  
		\node (L5) [right of=normalisation] {};
		\node (H5) [above of=L5] {};
		\node (L51) [below of=L5] {};
		\node (L52) [below of=L51] {};
		\node (L53) [below of=L52] {};
		\node (L54) [below of=L53] {};
		\node (descripteur) [right of=L5] {$\begin{array}{c}\mbox{calcul des}\\ \mbox{descripteurs}\end{array}$}; 
		\node[rect_y] (zkj) [below of=descripteur] {$z_{a}^{(j)}[k]$};   
		\node (zmkj) [below of=zkj] {};  
		\node[rect_y] (zpkj) [below of=zmkj] {${z}_{b}^{(j)}[k]$};  		
		\node (L6) [right of=descripteur] {};
		\node (distance) [right of=L6] {$\begin{array}{c}\mbox{calcul de la}\\ \mbox{distance}\end{array}$}; 
		\node (L67l) [below of=distance] {}; 
		\node[rect_y] (d) [below of=L67l] {$d(x_a,x_b)$};   
		
		\begin{scope}[-latex]
\draw[thick,->,blue] (xn) to   (xkn);
\draw[thick,->,blue] (xkn) to   (xkn1);
\draw[thick,->,blue] (xkn1) to   (xkn2);
\draw[thick,->,green] (xkn2) to   (zkj);
\draw[thick,->,blue] (xpn) to   (xpkn);
\draw[thick,->,blue] (xpkn) to   (xpkn1);
\draw[thick,->,blue] (xpkn1) to   (xpkn2);
\draw[thick,->,green] (xpkn2) to   (zpkj);
\draw[thick,->,red] (zpkj) to   (d);
\draw[thick,->,red] (zkj) to   (d);
\draw[gray,dashed,-] (H1) to   (H5);
\draw[gray,dashed,-] (H5) to   (L54);
\draw[gray,dashed,-] (L14) to   (L54);
\draw[gray,dashed,-] (H1) to   (L14);
\end{scope}
\end{tikzpicture}
\end{tabular}
\end{center}
\caption{Schéma décrivant la mise en oeuvre du calcul de la distance entre deux sons noté $x$ et $x'$. 
La partie encadrée en pointillé est la préparation des signaux
transformant $x_a[n]$ et $x_b[n]$ en $x_a[k,n]$ et $x_b[k,n]$, $n$ étant dans $x_a[n]$ et $x_b[n]$ l'indice de l'échantillon pour  l'ensemble du son 
et pour $x_a[k,n]$ et $x_b[k,n]$, l'indice dans la trame $k$. La lettre $j$ désigne un type de descripteur et celui-ci est calculé pour les deux sons et pour chaque 
%trame $k$, les valeurs obtenues sont rangées dans $z_{k}^{(j)}$ et ${z'}_{k}^{(j)}$. 
$d(x_a,x_b)$ désigne la valeur de la distance entre les deux sons.  }
\label{fig:dist_sons}
\end{figure}
 %\beqns
%\begin{array}{c@{}c@{}c@{}c@{}c@{}c@{}c}
%\mbox{sons} &  & \mbox{trames} && \hspace{-1cm}\mbox{descripteurs}\hspace{-1cm} && \mbox{distance}\\[0.3cm]
%\fr{$x_n$} &\arr{0}& \fr{$x_{k,n}$}& \arr{0}& \fr{$z_{k,j}$}\\[-0.4cm]
%&& && &\arr{-30} \\[-0.3cm]
%&& && &  &\fr{d(x,x')}\\[-0.3cm]
%&& && &\arr{+30} \\[-0.4cm]
%\fr{$x'_n$} &\arr{0}& \fr{$x'_{k,n}$}& \arr{0}& \fr{$z'_{k,j}$}\\[0.3cm]
%\end{array}
%\eeqns


La figure~\ref{fig:dist_sons} schématise la façon de calculer une distance (i.e. une non-similarité) entre deux sons. 
La partie encadrée en pointillé figure la préparation des signaux avec les tâches suivantes. 

\begin{minipage}{0.95\linewidth}
\begin{itemize}
\item Chaque signal sonore est décrit avec $x_a[n]$ et $x_b[n]$ par un signal temps discret échantillonné à la même fréquence d'échantillonnage, mais 
pas forcément de même durée. 
\item Chaque signal est découpé en trames, de longueur et de chevauchement identique, le nombre de trames est a priori différent d'un signal à l'autre. 
\item Les trames silencieuses en début et fin de son sont retirées. 
\item Les valeurs des signaux au sein de chaque trames sont normalisées globalement au niveau du son, c'est-à-dire que si une trame est 
en moyenne deux fois plus forte qu'une autre trame du même son, elle reste deux fois plus forte après la normalisation. 
Par contre quand on compare deux sons, le fait de multiplier par deux toutes les valeurs d'un des deux sons, ne modifie pas la distance entre les 
deux sons. 
\end{itemize}
\end{minipage}

On rajoute les notations suivantes~: 

\begin{minipage}{0.95\linewidth}
\begin{itemize}
\item $x_a$ et~$x_b$ désignent les sons~$a$ et~$b$. 
\item $x_a[n]$ et~$x_b[n]$ désignent les~$N_a$ et~$N_b$ valeurs des signaux associés aux sons~$a$ et~$b$. 
\item $x_a[kn]$ et~$x_b[kn]$ désignent les~$N_k$ valeurs des sons $a$ et $b$ pour la trame~$k$, c'est l'équivalent pour le son~$a$ de ce qui était noté précédemment~$x_k[n]$. 
\item $J$ désigne le nombre total de descripteur. 
\item $j\in\{1\ldots J\}$ désigne un descripteur spécifique. $\PMCT$ est un exemple de descripteur, les autres seront décrits dans le 
chapitre~\ref{ch:desc}. 
\item ${z}_a^{(j)}[k]$ et~${z}_b^{(j)}[k]$  désigne la valeur du descripteur~$j$ pour la trame~$k$ et les sons~$a$ et~$b$. 
\end{itemize}
\end{minipage}

Les calculs figurés par les flèches vertes joignant $x_a[kn]$ et $x_b[kn]$ à  ${z}_a^{(j)}[k]$ et ${z}^{(j)}_b[k]$ correspondent aux 
calculs des valeurs des descripteurs, 
Les flèches rouges joignant  ${z}_{a}^{(j)}[k]$ et ${z}_{b}^{(j)}[k]$ à $d(x_a,x_b)$ figurent les calculs permettant d'évaluer la distance à partir 
des valeurs des descripteurs, trois techniques sont proposées dans cette section. 

\subsection{Les descripteurs par trames sont transformés en descripteurs par son}
\label{ssec:mu_sigma}
On rajoute ici un autre sens au mot descripteur. Précédemment, il s'agissait d'un descripteur par trame, ici il s'agit d'un descripteur 
pour l'ensemble d'un son. Ce descripteur est identifié par $j$ correspondant aux valeurs du descripteur par trame qui sont 
résumés dans une seule valeur. Ce descripteur est aussi identifié par la façon de faire ce résumé~: $\mu$ pour la moyenne, $\sigma$ 
pour l'écart-type, $\gamma_1$ et $\gamma_2$ pour les coefficients d'asymétrie et d'aplatissement.

Ces quatre descripteurs de sons sont calculés à partir des valeurs d'un descripteur obtenu pour chaque trame d'un son. 

\begin{minipage}{0.95\linewidth}
\begin{itemize}
\item La moyenne d'un descripteur $j$ est la moyenne des valeurs de $z_k^{(j)}$ pour chaque trame $k$. 
\beqn\label{eq:mu}
\boxed{
\mu^{(j)}=\frac{1}{K}{\sum_{k=0}^{K-1} z_k^{(j)}}
}
\eeqn
\item 
L'écart-type d'un descripteur $j$ est la racine carré de la moyenne des variances.
\beqn\label{eq:sigma}
\boxed{
\sigma^{(j)}=\sqrt{\frac{1}{K}{\sum_{k=1}^K \left (z_k^{(j)} -\mu^{(j)}\right)^2}}
}
\eeqn
\item Le coefficient d'asymétrie d'un descripteur $j$ est 
\beqn
\gamma_1^{(j)}=\frac{1}{(\sigma^{(j)})^3}{\frac{1}{K}{\sum_{k=1}^K \left (z_k^{(j)} -\mu^{(j)}\right)^3}}
\eeqn
\item Le coefficient d'aplatissement d'un descripteur $j$ est 
\beqn
\gamma_2^{(j)}=\frac{1}{(\sigma^{(j)})^4}{\frac{1}{K}{\sum_{k=1}^K \left (z_k^{(j)} -\mu^{(j)}\right)^4}}
\eeqn
\end{itemize}
 \end{minipage}

Ces quatre descripteur de sons permettent de définir différentes distances entre sons suivant ce qui est pris en compte. 
Par exemple en prenant en compte la moyenne et l'écart-type des descripteur $j\in\{1\ldots J\}$, on a la distance suivante~: 
\beqn
\boxed{
d(x_a,x_b)=\sqrt{{\sum_{j=1}^J \left( \mu_a^{(j)}-\mu_b^{(j)}\right )^2+\left( \sigma_a^{(j)}-\sigma_b^{(j)}\right )^2}}
}
\eeqn

\subsection{La distance entre deux sons est obtenue en comparant trame par trame, les valeurs des descripteurs.}
\label{ssec:dist_trames}

Les sons $a$ et $b$ n'ont pas a priori la même durée et donc pas le même nombre de trames. On note $\min(K_a,K_b)$ le nombre de trames du son 
le plus court. On définit la distance comme la moyenne des distances entre les descripteurs trame par trame. Cette distance est 
en fait la racine carré de la somme des carrés des différences. Chaque son est décrit par $J{\times}K_a$ et $J{\times}K_b$ valeurs, 
on arrive à la définition suivante. 
\beqn
\boxed{
d(x_a,x_b)=\sqrt{\frac{1}{\min(K_a,K_b)}
{\sum_{k=0}^{\min(K_a,K_b)-1}{\sum_{j=1}^J\left (z_a^{(j)}[k]-z_b^{(j)}[k]\right )^2}}}
}
\eeqn

Un important défaut de cette technique est qu'elle amène à considérer un son comme différent, lorsqu'il est prononcé avec une vitesse différente ou simplement une vitesse qui varie différemment. 

\subsection{La distance entre deux sons est obtenue en cherchant la déformation temporelle minimisant la différence entre les deux sons.}
\label{ssec:dist_def_temp}

\subsubsection{Notion de déformation temporelle dynamique }


\begin{figure}
\begin{center}
\begin{tabular}{cc}
\includegraphics[width=0.5\linewidth]{fig_def_temp1.png}
\includegraphics[width=0.5\linewidth]{fig_def_temp2.png}\\
\includegraphics[width=0.5\linewidth]{fig_def_temp4.png}
\includegraphics[width=0.5\linewidth]{fig_def_temp3.png}
\end{tabular}
\end{center}
\caption{Quatre déformations possibles d'un même signal sinusoïdal représenté sur les quatre figures en vert. 
Le temps est représenté sur l'axe horizontal et les valeurs des signaux sont représentées sur l'axe vertical. En haut à gauche, le signal bleu 
est perturbé par un bruit additif, en haut à droite, il est perturbé par une bruit additif de moindre ampleur ajouté à la fois sur les valeurs du signal 
et celles du temps~; en bas à gauche, il est perturbé par un bruit additif ajouté seulement sur les valeurs de temps~; en bas à droite, le bruit 
additif ajouté seulement sur les valeurs de temps est corrigé par le fait qu'un évènement postérieur à un autre évènement doit rester postérieur après 
la perturbation.}
\label{fig:def_temp_1}
\end{figure}

La figure~\ref{fig:def_temp_1} représente un même signal sinusoïdal colorié en vert $x_v(t)$ et 
différentes déformations de ce signal sinusoïdal, $x_b(t)$, colorées en 
bleu. 

Il est d'usage lorsqu'on évalue la distance entre deux courbes définies sur un même intervalle de temps $[0,T]$, de calculer la 
moyenne quadratique de la différence entre $x_v(t)$ et $x_b(t)$. 
\beqn
\boxed{
d_1(x_v,x_b)=\sqrt{\frac{1}{T}{\int_0^T \left(x_v(t)-x_b(t)\right )^2\,dt}}
}
\eeqn
Cette évaluation est souvent choisie pour sa simplicité, elle a une interprétation pertinente lorsque le signal déformé $x_b(t)$ resulte 
d'un bruit blanc gaussien centré additif, car dans ce cas $d_1(x_v,x_b)$ est une estimation de l'écart-type de cette gaussienne. Le graphe en haut à gauche 
de la figure~\ref{fig:def_temp_1} montre en bleu un signal déformé par un bruit blanc additif, on y observe que parfois la courbe bleue est au dessus 
de la courbe verte et parfois elle est en dessous. 

Il existe dans la littérature scientifique une technique permettant d'évaluer la distance avec les différences en hauteur entre les signaux mais
avec les distances euclidienne entre les courbes, c'est-à-dire pour chaque point de la courbe $x_b(t)$, on utilise la distance entre ce point et 
le point le plus proche de $x_v(t)$. Cette évaluation est pertinente lorsqu'on considère que la déformation de $x_b(t)$ résulte d'une part 
d'un variation de  la valeur du signal $x_b(t^b_n)-x_v(t^v_n)$ mais aussi une variation de la base de temps $t^b_n-t^v_n$. Le graphe en haut à droite est obtenu en ajoutant deux bruits blancs 
gaussiens centrés additifs indépendants sur les valeurs du signal et sur les instants associés à ces valeurs. 

Le graphe en bas à gauche est obtenu en ne modifiant que les bases de temps $t^b_n$ par rapport à $t^v_n$, il s'agit d'un bruit blanc gaussien centré 
additif. C'est-à-dire qu'on a l'égalité entre les valeurs des signaux $x_b$ et $x_v$ mais les valeurs ont lieu à des instants différents. 
\beqns
x_b(t^b_n)=x_v(t^v_n)
\eeqns
Sur ce graphe, la courbe bleue présente des boucles suggérant que le temps s'inverse parfois. Ceci n'est pas une modélisation réaliste. 

Le graphe en bas à droite est obtenu aussi en ne modifiant que les bases de temps $t^b_n$ par rapport à $t^v_n$, mais pour plus de réalisme, l'ordre des 
évènements est respecté, il n'y a donc plus de boucles.
\beqns
t^v_n\leq t^v_{n'}\quad\Rightarrow\quad t^b_n\leq t^b_{n'}
\eeqns
Concrètement, les variations de $t^b_n$ sont limitées par la contrainte que $t^b_{n}\leq t^b_{n+1}$ doit toujours être vrai. 
C'est ce type de  déformation du signal que l'on cherche à prendre en compte. Quand on prononce un son plus lentement pour plus rapidement ou 
avec une vitesse qui varie au cours de la prononciation du son, il s'agit du même son. La distance devrait théoriquement ne pas 
être sensible à ce type de déformation. 
On appelle cette déformation, une déformation temporelle dynamique.~\footnote{Cette notion est présentée en détail dans~\cite{Cassisi12}.} 


\subsubsection{Table d'indexation}

\begin{figure}
\begin{center}
\begin{tabular}{c}
\includegraphics[width=0.5\linewidth]{fig_7.png}
\end{tabular}
\end{center}
\caption{En vert et bleu, deux signaux sont définis sur des intervalles de temps différents $(t_n,x_n)$, $(t'_n,y_n)$.
En rouge, le signal $(t_n,x_n)$ est transformé par une table d'indexation en 
$(t'_{\Phi_{y}[n]},x_{\Phi_x[n]})$ de façon à approcher le signal $(t'_n,y_n)$.}
\label{fig7}
\end{figure}

La figure~\ref{fig7} illustre ce que l'on cherche à faire avec deux tables d'indexation. 
Le trait bleu associé à $x_n$ est défini sur l'intervalle de temps $[0,20]$, tandis que la courbe verte associée à $y_n$ 
est définie sur l'intervalle de 
temps $[0,15]$. Le signal $x_{\Phi_x[n]}$ est défini pour les entiers $\{0\ldots 21\}$ et est à valeurs parmi les 
valeurs de $\{x_0\ldots x_{20}\}$, ce sont des points qui sont sur la courbe rouge. La courbe rouge est en fait 
obtenue avec reliant les points $(t_{\Phi_y[n]},x_{\Phi_x[n]})$.
\beqns
\begin{array}{llcl}
\Phi_x[0]=0 & \Phi_y[0]=0 & (t_{\Phi_y[0]},x_{\Phi_x[0]})=(t_0,x_0)=(0,0) & \mbox{position initiale en bas à gauche}\\
& & \vdots& \\
\Phi_x[3]=3 & \Phi_y[1]=0 & (t_{\Phi_y[3]},x_{\Phi_x[3]})=(t_0,x_3)=(0,3) & \mbox{déplacement vertical {\bf V}}\\
\Phi_x[4]=3 & \Phi_y[4]=1 & (t_{\Phi_y[4]},x_{\Phi_x[4]})=(t_1,x_3)=(1,3) & \mbox{déplacement horizontal {\bf H}}\\
\Phi_x[5]=4 & \Phi_y[5]=2 & (t_{\Phi_y[5]},x_{\Phi_x[5]})=(t_2,x_4)=(2,4) & \mbox{déplacement diagonal {\bf D}}\\
&&\vdots &
\end{array}
\eeqns 
Cet exemple illustre le fait que deux tables d'indexation permettent de modéliser un déplacement horizontal et vertical. 

En pratique, on n'utilise pas la base de temps, on modifie juste les indices avec les deux tables 
d'indexation de façon à minimiser le carré des différences entre $x_{\Phi_x[n]}$ et $y_{\Phi_y[n]}$. 
\beqn
y_{\Phi_y[n]}\approx x_{\Phi_x[n]}
\eeqn

On introduit de nouvelles notations. 
\begin{itemize}
\item $N_\Phi$: Les tables d'indexation sont définies sur une plage d'indices communs 
\beqns
n\in\{0\ldots N_\Phi-1\}
\eeqns
\item $N_x$ et $N_y$ sont le nombre d'indices pour $x_n$ et $y_n$. 
Chaque table d'indexation est à valeurs dans les indices sur lesquels $x_n$ et $y_n$ sont définis
\beqns
\Phi_x[n]\in \{0\ldots N_x-1\} \mbox{ et }\Phi_y[n]\in \{0\ldots N_y-1\}
\eeqns
\end{itemize}


En pratique, on impose que le premier indice de $\Phi_x$ corresponde au point de départ de $x_n$, le dernier de $\Phi_x$
avec le point d'arrivée de $x_n$ et de même pour $\Phi_y$ avec $y_n$. 
\beqn\label{eq:phi_contr1}
\left \{
\begin{array}{ll}
\Phi_x[0]=0,\,&\Phi_x[N_{\Phi}-1]=N_x-1\\[0.2cm]
\Phi_{y}[0]=0,\,&\Phi_{y}[N_{\Phi}-1]=N_y-1\\[0.2cm]
\end{array}
\right . 
\eeqn

On introduit la contrainte modélisant le non-retournement du temps 
\beqn\label{eq:phi_contr2}
\Phi_x[n]\leq \Phi_x[n+1] \mbox{ et }\Phi_{y}[n]\leq \Phi_{y}[n+1]
\eeqn


On rajoute une autre contrainte qui indique que la différence de temporalité entre les deux signaux ne doit pas 
être trop grande. 
Cette contrainte a aussi l'avantage de diminuer la complexité numérique de l'algorithme utilisé pour calculer cette nouvelle distance. 
\beqn\label{eq:phi_contr3}
\left |\Phi_x[n]-\Phi_{y}[n]\right |\leq \delta
\eeqn
$\delta$ étant un paramètre à définir pour calculer cette distance. 

\subsubsection{Distance définie au moyen d'un problème d'optimisation}


Pour chaque choix de $\Phi_x$ et $\Phi_y$, on a une valeur de distance qui est obtenue classiquement avec la moyenne quadratique. 
\beqn
\label{eq:tw_d1}
\boxed{
d_{\Phi_x,\Phi_{y}}(x,y)=\sqrt{\frac{1}{N_x+N_y}{\sum_{n=0}^{N_{\Phi}-1} \left(x_{\Phi_x[n]}-y_{\Phi_{y}[n]} \right )^2}}
}
\eeqn
La distance prenant  en compte de la déformation temporelle dynamique est alors défini en choisissant 
$\Phi_x$ et $\Phi_y$ de façon à respecter les contraintes définies par les équations~(\ref{eq:phi_contr1}),~(\ref{eq:phi_contr2}) et~(\ref{eq:phi_contr3}). 
et à minimiser $d_{\Phi_x,\Phi_{y}}(x,y)$.
\beqn\label{eq:prob_min}
\boxed{
d_\delta(x,y)=\underset{\Phi_x,\Phi_y}{\min}\,d_{\Phi_x,\Phi_{y}}(x,y)
}
\eeqn

\subsubsection{Algorithme résolvant ce problème d'optimisation}

\begin{figure}
\begin{center}
\begin{tabular}{c}
\includegraphics[width=0.5\linewidth]{fig_8c.png}
\includegraphics[width=0.5\linewidth]{fig_8d.png}
\end{tabular}
\end{center}
\caption{\`A gauche~: représentation temporelle des signaux $x_n$, $y_n$ et $x_n$ transformés par déformation temporelle. 
\`A droite~: représentation des tables d'indexation permettant de générer la déformation temporelle du signal $x_n$. 
}
\label{fig8}
\end{figure}

La gauche de la figure~\ref{fig8} est similaire à la figure~\ref{fig7} avec en bleu et vert deux signaux $(t_n,x_n)$ et $(t_n,y_n)$ et 
en rouge, la déformation du premier signal pour se rapprocher du second~: $(t_{\Phi_y[n]},x_{\Phi_x[n]})$. 
La droite de cette figure montre les valeurs prises par~$\Phi_x[n]$ et~$\Phi_y[n]$ en représentant ces deux tables 
comme une succession de points formant un chemin reliant au départ~$(0,0)$ au point d'arrivée~$(N_x,N_y)=(5,3)$.
Ces contraintes correspondent à  l'équation~(\ref{eq:phi_contr1}). 
On satisfait la contrainte de l'équation~(\ref{eq:phi_contr2}) en imposant que le chemin soit composé seulement de 
déplacement verticaux, horizontaux ou diagonaux et en l'occurrence seulement d'un pas à la fois. 
La contrainte indiquée par l'équation~(\ref{eq:phi_contr3}) est indiquée par les traits noirs hachurés à l'extérieur de la zone autorisée sur la 
droite de la figure~\ref{fig8}. 
 


Les valeurs utilisées pour les signaux représentés sur la figure~\ref{fig8} sont 
\beqns
\begin{array}{llllll}
x_0=0 & x_1=1 & x_2=2 & x_3=3 & x_4=4 & x_5=5\\[0.2cm]
y_0=0 & y_1=2 & y_2=4 & y_3=5\\[0.2cm]
\end{array}
\eeqns
Les tables d'indexations créées sont~: 
\beqns
\begin{array}{llllll}
\Phi_x[0]=0 & \Phi_x[1]=1 & \Phi_x[2]=2 & \Phi_x[3]=3 & \Phi_x[4]=4 & \Phi_x[5]=5 \\[0.2cm]
\Phi_y[0]=0 & \Phi_y[1]=0 & \Phi_y[2]=0 & \Phi_y[3]=1 & \Phi_y[4]=2 & \Phi_y[5]=3 \\[0.2cm]
\end{array}
\eeqns

On appelle arête ({\em edge}) les traits associés au déplacement sur le graphe de droite. On appelle noeud ({\em node}, {\em vertice}) les 
points indiqués par des ronds bleus sur le graphe de droite. 
La localisation du point $n$ est déterminé par $\Phi_x[n]$ et $\Phi_y[n]$, il se trouve que ces valeurs déterminent aussi 
\beqns
(x_{\Phi_x[n]}-y_{\Phi_y[n]})^2
\eeqns
Les nombres en bleus situés à côté de chaque noeud donnent la valeur de cette quantité. 
Ce sont les valeurs de $x_n$ et $y_n$ qui donnent à chaque point du graphe de droite une valeur pour $(x_{\Phi_x[n]}-y_{\Phi_y[n]})^2$
dépendant uniquement de la position du point. 
La distance entre les deux signaux telle que définie dans l'équation est à la somme des quantités inscrites à côté de chaque noeud. 
L'équation~(\ref{eq:prob_min}) indiquant que la distance est obtenue à partir du chemin minimisant $d_{\Phi_x,\Phi_y}(x,y)$
 définie par l'équation~(\ref{eq:tw_d1}). Il se trouve que le graphe à droite de la figure~\ref{fig8} donne une interprétation de cette minimisation. 
$d_{\Phi_x,\Phi_y}(x,y)$ est la somme des valeurs associées à chaque point et qui ne dépend que de la position des points. 
La minimisation consiste donc à trouver le chemin minisant la somme des valeurs de chaque noeud en utilisant que des déplacements verticaux, horizontaux ou diagonaux et menant d'un point de départ à un point d'arrivée tout en restant dans le domaine délimité par les zones hachurées. 

L'algorithme permettant cette minimisation s'appelle l'algorithme de Dijkstra. 
Il consiste dans un premier temps à découvrir tous les noeuds possibles.
\begin{itemize}
\item Le premier noeud regardé est le point de départ et on lui affecte la valeur associée $(x_0-y_0)^2$. 
\item On répète la tâche suivante
\begin{enumerate}
\item\label{it:vois} Aller au voisin et lui donner la valeur de la distance entre le point de départ et ce voisin. 
\item On indique aussi à ce voisin le noeud précédent où l'on était. 
\item Si sur ce voisin il y a déjà une valeur, alors cette valeur doit être diminuée si la distance trouvée est moindre et 
on lui change l'origine que si l'on change sa valeur. 
\item Revenir au noeud précédent. 
\item Aller à l'étape~\ref{it:vois} s'il y a un voisin disponible et non-exploré dans cette tâche. 
\item Revenir au premier voisin et s'autoriser à aller à une profondeur supplémentaire. 
\end{enumerate}
\end{itemize}
Lorsque ces tâches ne peuvent plus être répétés parce qu'on a été au maximum de la profondeur possible, alors 
on part du point d'arrivée et on remonte au point de départ en suivant les indications laissées à chaque noeud. 




\begin{figure}
\begin{center}
\begin{tabular}{c}
\includegraphics[width=\linewidth]{fig_dist_temp_bis.png}
\end{tabular}
\end{center}
\caption{\`A gauche~: représentation temporelle des signaux $x_n$, $y_n$ et $x_n$ transformés par déformation temporelle. 
\`A droite~: représentation des tables d'indexation permettant de générer la déformation temporelle du signal $x_n$. 
}
\label{fig8bis}
\end{figure}

La figure~\ref{fig8bis} est assez similaire à la figure~\ref{fig8} mais avec d'autres valeurs pour les signaux $x_n$, $y_n$, $\Phi_x[n]$ et $\Phi_y[n]$. 



\section{Prédiction par le plus proche voisin}
\label{sec:knn}
\subsection{Principe}

\begin{figure}
\begin{center}
\begin{tabular}{c}
\includegraphics[width=\linewidth]{knn_ex1.png}
\end{tabular}
\end{center}
\caption{Visualisation de sons à travers les valeurs des indicateurs $\mu_\sm{PMCT}$ et $\sigma_\sm{PMCT}$}
\label{fig_knn}
\end{figure}

On appelle {\bf classifieur} le programme ou le procédé par lequel il est estimé que le son appartient à telle classe. 

On appelle {\bf prédiction} le fait pour un classifieur d'estimer qu'un son appartient à une classe en utilisant uniquement les données 
numériques disponible pour ce son. 

La prédiction par le plus proche voisin est un cas particulier d'un classifieur appelé $k$-NN pour {\em Nearest Neighbor} ce qui signifie 
justement les $k$ plus proche voisins. Ce classifieur est performant mais très coûteux en terme de complexité numérique dès lors que la 
base de donnée est assez importante. Il est aussi particulièrement simple à implémenter, ce qui est la raison principal de son choix ici. 
Il est utilisé ici dans le cas où $k=1$. 

Ce classifieur consiste pour chaque son inconnu appelé requête, de parcourir tous les sons de la base de données et pour chaque son de 
calculer sa distance avec la requête. Le classifieur détermine la classe comme étant celle du son ayant la plus petite distance avec la requête. 
Cette classe est appelée la prédiction faite par le classifieur pour cette requête. 
Il est intéressant de remarquer que ce choix de faire une classification en fonction d'un seul élément (ou de $k$ éléments dans la version plus 
générale de cet algorithme) permet de s'adapter à une situation ou une classe regrouperait des éléments très hétérogènes. 


La figure~\ref{fig_knn} montre comment une vingtaine de sons peuvent être visualisés sur un graphe. Chaque point correspond à un son, sa couleur 
(bleu pour {\tt un}, vert pour {\tt deux}, rouge pour {\tt trois}) indique le mot que ce son vocalise. Cette information est ce que l'on cherche à prédire avec 
la prédiction par le plus proche voisin. La localisation de chaque point dépend des valeurs de deux indicateurs, $\mu_{\sm{PMCT}}$ et $\sigma_{\sm{PMCT}}$. 
Ces indicateurs ont été présentés dans les sections~\ref{ssec:PMCT} et~\ref{ssec:mu_sigma}, c'est un programme informatique qui à partir des
données enregistrées permet de calculer ces deux valeurs et ainsi de positionner ces points sur ce graphique.
Pour illustrer le fonctionnement de cette technique de prédiction, voici son fonctionnement. 
\begin{enumerate}
\item  Sélectionnez dix points que vous numérotez de $1$ à $10$. 
\item Considérer un autre 
point qui ne figure pas parmi ces points. Ce point est appelé requête. 
\item Mesurez avec une règle la distance entre ce point requête et chacun de ces 10 points numérotés. 
\item Regardez la couleur du point qui a la distance avec le point requête la plus faible (et qui est donc sur le graphique 
le plus proche du point requête parmi les 10 points numérotés).
\item La prédiction consiste à attribuer au point requête la couleur du point le plus proche et par suite la classe, {\tt un}, {\tt deux} ou 
{\tt trois} suivant la 
couleur observée. 
\end{enumerate}

\subsection{Formalisation de la technique du plus proche voisin}

 Pour formaliser cette technique du plus proche voisin, on adopte les notations suivantes. 
\begin{itemize}
\item $x$ désigne en général un son défini pour plus de généralité par ses valeurs  $x_n$. 
\item $\chi$ désigne un ensemble de sons. 
\item $y$ désigne la classe à laquelle le son $x$ appartient, ({\tt un}, {\tt deux} ou {\tt trois}), est indiqué par son appartenance respective à $\chi_1, \chi_2,\chi_3$. 
\item $\br{d}(x_a,x_b)$ est une valeur positive correspondant à 
la distance entre les sons $x_a$ et $x_b$. En fait pour plus de généralité, ce calcul repose sur la réalisation des 
étapes suvantes. 
\begin{itemize}
\item Découpage de $x_a$ et $x_b$ en trames décrit à la section~\ref{sec:N:son_trames}.
\item Calcul d'un indicateur par trame pour $x_a$ et $x_b$, illustré par $\sm{PMCT}$ décrite à la section~\ref{ssec:PMCT}.
\item Mise en  oeuvre d'une des trois distance présentées dans les sections~\ref{ssec:mu_sigma},~\ref{ssec:dist_trames},~\ref{ssec:dist_def_temp}. 
\end{itemize}
\item $\br{d}(x,\chi)$ désigne la distance entre le son $x$ et un ensemble de sons regroupés dans $\chi$. 
Du fait du choix de la technique du plus proche voisin, cette distance est ici définie par 
\beqn
\boxed{
\br{d}(x,\chi)=\min\limits_{x'\in \chi} \br{d}(x,x')
}
\eeqn
où $\min\limits_{x'\in \chi} \br{d}(x,x')$ désigne la valeur la plus faible parmi les distances mesurées entre un son donné $x$ et 
tous les sons $x'$ contenus dans $\chi$. 
\item $\ww{x}$ désigne la classe prédite. Cette classe est prédite de cette façon. 
\beqn
\boxed{
\ww{x}=\argmin_{c\in\{1,2,3\}}\br{d}(x,\chi_c)
}
\eeqn
où $\chi_1,\chi_2,\chi_3$ regroupent des sons dont on sait qu'ils sont respectivement associés à {\tt un}, {\tt deux} et {\tt trois}. 
et $\argmin\limits_{c\in\{1,2,3\}}\br{d}(x,\chi_c)$ est ainsi défini. 
\beqns
\argmin\limits_{c\in\{1,2,3\}}\br{d}(x,\chi_c)=\left \{
\begin{array}{lclcl}
1 & \mbox{si} & \br{d}(x,\chi_1)\leq \br{d}(x,\chi_2) &\mbox{et}& \br{d}(x,\chi_1)\leq \br{d}(x,\chi_3)\\
2 & \mbox{si} & \br{d}(x,\chi_2)\leq \br{d}(x,\chi_1) &\mbox{et}& \br{d}(x,\chi_2)\leq \br{d}(x,\chi_3)\\
3 & \mbox{si} & \br{d}(x,\chi_3)\leq \br{d}(x,\chi_1) &\mbox{et}& \br{d}(x,\chi_3)\leq \br{d}(x,\chi_2)\\
\end{array}
\right . 
\eeqns

\end{itemize}


\subsection{Illustration avec l'implémentation proposée en TP}

\begin{figure}
\begin{center}
\begin{tabular}{c}
\includegraphics[width=\linewidth]{fig_rep_req.png}
\end{tabular}
\end{center}
\caption{Schéma correspondant aux différents dossiers existant et créés pour réaliser la prédiction en utilisant la technique du plus proche voisin. 
}
\label{fig9bis}
\end{figure}

La figure~\ref{fig9bis} illustre la façon  dont l'algorithme est ici implémenté. Chaque bloc représente un répertoire 
contenant des fichiers. 
Les sons que l'on utilise pour tester et évaluer la performance d'un classifieur sont en réalité issus de la base de données. 
Il faudrait donc s'assurer qu'ils ne sont pas utilisés aussi pour l'apprentissage. 
La partie qui n'est pas encadré en pointillé n'est pas modifiée lors de la mise en oeuvre de la classification. Cette
mise en oeuvre consiste à tirer aléatoirement une partie des sons des répertoires {\tt un}, {\tt deux} et {\tt trois}, 
de les placer dans le
répertoire {\tt requête}, les autres sons sont placés dans trois nouveaux répertoires contenus dans le répertoire 
{\tt simulation} et appelé {\tt un}, {\tt deux} et {\tt trois}. 
L'information selon laquelle les sons placés dans {\tt requête} n'est pas disponible sur les fichiers sons, mais elle 
est stockée pour être utilisée ultérieurement lors de l'évaluation de l'algorithme. 

\section{\'Evaluation de la performance d'un classifieur}
\label{sec:evaluation_classification}

En pratique quand on utilise un procédé de reconnaissance vocal, on a besoin de savoir dans quelle mesure on peut lui faire confiance. 
Cette mesure est ce qu'on appelle l'{\bf évaluation de la performance}. Pour se faire, on utilise des sons dont on connaît la classe à laquelle 
ils appartiennent et on compare cette classe avec ce que le classifieur prédit. Il existe un très grand nombre de mesures de performance, on en présente 
trois types~: la sensibilité globale, la précision et le rappel. 

\subsection{Matrice de confusion}

Le rôle de la matrice de confusion est de résumer sous la forme d'une matrice les données utiles au calcul de l'évaluation de la performance. 
Ces données utiles consistent en le fait de connaître le nombre d'expérience où le son requête appartenait à telle classe et où la classe prédite est 
celle-là. Dans le cadre de cette étude, il s'agit d'une matrice $3{\times}3$ puisqu'il y a trois sons possibles. 

\begin{itemize}
\item Chaque {\bf ligne} est associée aux expérimentations sur les sons qui en réalité appartiennent à telle classe. 
\item Chaque {\bf colonne} est associée aux expérimentations sur les sons qui ont été prédit comme étant de telle classe. 
\item La somme de toutes les cases est égale au nombre total d'expérimentations. 
\item \`A la case $i,j$, il y a le nombre d'expérimentations pour lesquelles le son appartient en réalité à la classe~$i$ et 
le classifieur l'a prédit comme étant de la classe~$j$. 
\item $m$ est un indice faisant référence à un son $x$. 
\item $M$ est le nombre total de sons utilisés pour les différentes requêtes. 
\item $\1(\ldots)$ est la fonction caractéristique, elle prend la valeur $1$ si les trois points de suspension sont remplacés par 
une affirmation exacte et par $0$ si l'affirmation est fausse. 
\item $\1(y_m=c)$ vaut $1$ si  le son numéro $m$ est de la classe $c$ et $\1(y_m=c)$ vaut $0$ si ce n'est pas le cas. 
\item $\1(\ww{x}_m=c)$ vaut $1$ si le son numéro $m$ est prédit par le classifieur comme étant de classe $c$ et $\1(\ww{x}_m=c)$ vaut $0$ 
si ce n'est pas le cas. 
\item $\1(y_m=i)\1(\ww{x}_m=j)$ vaut $1$ is le son numéro $m$ est d'une part de la classe $i$ et d'autre part a été prédit par le classifieur 
comme étant de la classe $j$. 
\end{itemize}

Les composantes de la matrices de confusion sont~: 
\beqn\label{eq:matrice_confusion}
\boxed{
C_{ij}={\sum_{m=1}^M\1(y_m=i)\1(\ww{x}_m=j)}
}
\eeqn


\subsection{Sensibilité globale}

La sensibilité globale, notée $\OA$ pour {\em Overall Assessment}, est 
le rapport entre le nombre de classifications correctes sur le nombre totales de requêtes, noté $M$. 
Les classifications correctes sont celles pour lesquelles $y_m=\ww{x}_m$. 

\beqn
\label{eq:OA}
\boxed{
\OA=\frac{C_{11}+C_{22}+C_{33}}{3}
}
\eeqn

\subsection{Précision et rappel}

La précision et le rappel sont des notions très utilisées pour les classifieurs binaires, c'est-à-dire pour lesquels, il n'y a que deux classes. 
Mais ces notions sont parfois étendues au cas plus général où on considère un nombre plus important de classes, c'est ce que nous utilisons ici. 

Pour chaque classe~$c$, on calcule deux indicateurs. La {\bf précision} $\p{P}_c$ est le rapport entre le nombre de requête correctement attribuées à la classe~$c$
et le nombre de requêtes que le classifieur évalué a prédit comme étant de la classe~$c$. 
Le {\bf rappel} $\p{R}_c$  est le rapport entre le nombre de requête correctement attribué à la classe~$c$ 
et le nombre de requêtes qui dans la réalité correspondent à la classe~$c$. 
\beqn
\boxed{
\left\{
\begin{array}{l}
\p{P}_1=\frac{C_{11}}{C_{11}+C_{21}+C_{31}}\\[0.3cm]
\p{P}_2=\frac{C_{22}}{C_{12}+C_{22}+C_{32}}\\[0.3cm]
\p{P}_3=\frac{C_{33}}{C_{13}+C_{23}+C_{33}}\\[0.3cm]
\end{array}
\right.
\quad
\mbox{et} \quad 
\left\{
\begin{array}{l}
\p{R}_1=\frac{C_{11}}{C_{11}+C_{12}+C_{13}}\\[0.3cm]
\p{R}_2=\frac{C_{22}}{C_{21}+C_{22}+C_{23}}\\[0.3cm]
\p{R}_3=\frac{C_{33}}{C_{31}+C_{32}+C_{33}}\\[0.3cm]
\end{array}
\right.
}
\eeqn
Ainsi la précision indique la probabilité  qu'un échantillon, dont le classeur évalué indique qu'il s'agit de la classe~$i$, 
soit effectivement de la classe~$i$. 
Par contre,  le rappel indique la probabilité pour qu'un échantillon dont on sait qu'il est de la classe~$i$, soit détecté 
comme tel par le classifieur évalué. 


\subsection{Validation croisée}

\begin{figure}
\begin{center}
\begin{tabular}{c}
\includegraphics[width=0.8\linewidth]{illustration_validation_croisee.png}
\end{tabular}
\end{center}
\caption{Schéma décrivant ce qu'est une validation croisée.}
\label{fig:O:valid_croisee}
\end{figure}


La {\bf validation croisée} est une technique souvent utilisée pour la mise en oeuvre d'un algorithme de classification, 
elle n'est pas destinée à améliorer l'efficacité d'un classifieur, elle est destinée à évaluer plus précisément sa 
performance vis-à-vis d'une base de données en particulier  lorsqu'il est compliqué d'augmenter le nombre de sons dont on connaît la
classe à laquelle chacun appartient. 
La figure~\ref{fig:O:valid_croisee} illustre le fonctionnement de la validation croisée avec un schéma. 
En haut de cette figure se trouve 12 sons figurés par $x_1\ldots x_{12}$ et $12$ valeurs notées $y_1\ldots y_{12}$ indiquant les véritables classes à laquelle chaque son appartient.
Ici il s'agit d'une validation croisée en quatre blocs, ce qui amène à réaliser quatre apprentissages de classifieurs. 
{\tt Exp1} désigne en haut la première expérience avec le premier apprentissage. Les trois premiers sons de la base 
d'apprentissage $(x_1,y_1),(x_2,y_2),(x_3,y_3)$ servent de base pour tester le classifieur et sont affichés sur fond rouge. Le classifieur testé est entraîné 
en utilisant tous les autres sons $(x_4,y_4),\ldots,(x_{12},y_{12})$ qui sont eux affichés sur fond bleu. Le test du classifieur permet de calculer une matrice 
de confusion spécifique à {\tt Exp1} et celle-ci permet de calculer la sensibilité globale $\sm{OA}_1$.
Les trois autres expériences sont fait de la même façon, mais en utilisant successivement comme sons tests les 
sons $(x_4,y_4),(x_5,y_5),(x_6,y_6)$, puis $(x_4,y_4),(x_5,y_5),(x_6,y_6)$ et enfin $(x_4,y_4),(x_5,y_5),(x_{12},y_{12})$.





\chapter{Descripteurs de trames}
\label{ch:desc}

La partie précédente ayant montrée comment un descripteur par trame permet de définir une technique de classification, cette 
partie traite de la détermination d'un descripteur par trame. 
L'inspiration qui a guidé l'élaboration des descripteurs provient de l'étude des caractéristiques des ondes sonores émises par un individu,
c'est ce qui constitue la section~\ref{sec:model_parole} et qui montre l'intérêt de trouver la fréquence fondamentale et la plage de fréquences présentes
dans le son émis. 
La section~\ref{sec:estimation_spectrale} présente différentes heuristiques permettant de décrire ce contenu spectral en indiquant la fréquence fondamentale, la 
fréquence moyenne et la largeur de spectre. 
La section~\ref{sec:banc_filtres} présente une technique plus systématique pour décrire le contenu spectral, c'est en utilisant un banc de filtres, chaque 
filtre constitue une heuristique donnant une information partielle sur le contenu spectral du son. 


\section{Modélisation de la production de la parole}
\label{sec:model_parole}

La présentation de la modélisation de la façon dont un humain produit un son est 
faite en trois parties. La section~\ref{ssec:onde_stationnaire} décrit le phénomène physique 
permettant de transformer une source sonore en un son dont le caractère plus ou moins aigü du son 
peut être déterminé assez précisément au moyen d'une note. 
La section~\ref{ssec:appareil_phonatoire} décrit brièvement les organes humains intervenant pour 
la production d'un son. 
Enfin la section~\ref{ssec:spectrogramme} présente la notion d'analyse temps-fréquence illustré 
avec la présentation d'un spectrogramme.

\subsection{Onde stationnaire}
\label{ssec:onde_stationnaire}

On dit qu'une onde est stationnaire si en chaque point, on observe que  la surpression évolue dans le temps comme une sinusoïde. 
Par exemple l'équation suivante décrit une évolution sinusoïdale dont l'amplitude crête à crête dépend de l'indice $x$ et vaut 
$\cos(2\pi \frac{x}{\lambda_0})$. 
\beqns
P(x,t)=\Delta P_0\cos(2\pi f_0t)\cos(2\pi \frac{x}{\lambda_0})
\eeqns
où $\lambda$ et $f_0$ sont 
Cette onde peut approximativement correspondre à un cas particulier de l'équation~(\ref{eq:propag_onde}) lorsque le coefficient $\frac{1}{r}$ est 
supposé approximativement constant et~$r$ est remplacé par~$x$. 
La trigonométrie nous indique
que le produit de deux cosinus est une différence entre deux sinus,
 $\cos(a)\cos(b)=\frac{1}{2}\cos(a-b)+\frac{1}{2}\cos(a+b)$. 
Cela permet de voir qu'une onde stationnaire est la somme d'une onde se propageant dans le sens des $x$ croissants et 
une autre dans le sens des $x$ décroissants.
\beqn\label{eq:onde_stationnaire}
P(x,t)=\frac{\Delta P_0}{2}\cos\left (2\pi f_0(t-\frac{x}{c})\right )
+\frac{\Delta P_0}{2}\cos\left (2\pi f_0(t+\frac{x}{c})\right )
\eeqn
où $c=\lambda_0 f_0$ est la vitesse de propagation du son dans l'air. 
Cette modélisation correspond à $g_1=g_2$ dans l'équation~(\ref{eq:propag_onde}). 




\begin{figure}[htbp]
\begin{center}
\begin{tabular}{c}
\includegraphics[width=0.5\linewidth]{onde_stationnaire.png}
\end{tabular}
\end{center}
\caption{Pour une même taille donnée, un même obstacle peut être le siège de trois ondes stationnaires. 
La vitesse moyenne des particules d'air doit être nulle aux deux extrémités de la caisse de résonnance. }
\label{fig:onde_stationnaire}
\end{figure}

La figure~\ref{fig:onde_stationnaire} illustre de manière simplifiée la façon dont la forme géométrique d'une caisse de 
résonance détermine une fréquence de résonance. 
Le haut de la figure schématise al caisse de résonance qui est un pavé. La coupe est un rectangle. La zone colorée 
en bleu schématise une onde stationnaire qui consiste en une variation spatiale et temporelle avec une relation 
entre la longueur d'onde et la fréquence de la vibration indiquée dans l'équation~\ref{eq:long_onde} ($\lambda=c/f$ où 
$c$ est ici la vitesse de propagation du son dans l'air, approximativement 1km toutes les $3$~secondes). Les trois dessins 
illustrent qu'avec une même forme géométrique (un pavé de longueur $d$), $3$ longueurs d'onde sont montrés. 
\begin{center}
\begin{tabular}{|c|c|c|}
\hline 
$\lambda=2d$ & $f=\frac{c}{2d}$ & $d=\frac{\lambda}{2}$\\[0.1cm]
\hline
$\lambda=d$ & $f=2\frac{c}{2d}$ & $d={\lambda}$\\[0.1cm]
\hline
$\lambda=\frac{2}{3}d$ & $f=3\frac{c}{2d}$ & $d=\frac{3\lambda}{2}$\\[0.1cm]
\hline
\end{tabular} 
\end{center}

Cette schématisation illustre un phénomène plus général, à savoir que l'émission d'un son à une certaine fréquence de base
produit généralement des harmoniques qui sont des vibrations à des fréquences qui sont multiples de cette fréquence de base. 
La relation entre longueur du rectangle et longueur d'onde est ici déterminé par le fait que la vibration 
du son est nul sur la paroi (i.e. la paroi est fixe). Dans une onde stationnaire modélisée par l'équation~(\ref{eq:onde_stationnaire}),
c'est à cet endroit que la pression est soit maximale soit minimale.
L'annexe~\ref{app:onde_stationnaire_1D} formalise cette description de manière plus précise.  

Une onde stationnaire peut aussi exister avec un rectangle ouvert sur un côté. Dans ce cas c'est la pression qui est fixée et la vibration 
qui est maximale à l'endroit où le rectangle est ouvert. Les relations entre longueurs d'onde, fréquences et longueur du rectangle sont alors modifiées. 
\begin{center}
\begin{tabular}{|c|c|c|}
\hline 
$\lambda=4d$ & $f=\frac{c}{4d}$ & $d=\frac{\lambda}{4}$\\[0.1cm]
\hline
$\lambda=\frac{4}{3}d$ & $f=3\frac{c}{4d}$ & $d=\frac{3\lambda}{4}$\\[0.1cm]
\hline
$\lambda=\frac{4}{5}d$ & $f=5\frac{c}{4d}$ & $d=\frac{5\lambda}{4}$\\[0.1cm]
\hline
\end{tabular} 
\end{center}



\subsection{Modélisation de l'appareil phonatoire}
\label{ssec:appareil_phonatoire}


\begin{figure}[htbp]
\begin{center}
\begin{tabular}{c}
\includegraphics[width=0.5\linewidth]{parole_formation.jpg}
\end{tabular}
\end{center}
\caption{Diagramme représentant les organes de la parole }
\label{fig:parole_formation}
\end{figure}

On appelle appareil phonatoire l'ensemble des organes humains permettant de produire un son. 
L'objet de cette partie est une brève description de son fonctionnement. 

La figure~\ref{fig:parole_formation} représente une coupe de la tête d'une personne, (coupe dite sagittale), avec la gorge en bas à droite, la bouche au milieu à gauche, les dents le long d'une ligne horizontale placée légèrement au dessus de la bouche. 
Cette figure permet de modéliser la façon dont un son est formé. 
\begin{itemize}
\item Le son est produit par la vibration d'un organe musculaire appelé corde vocale ou plis vocaux. Cet organe musculaire 
permet un contrôle de la fréquence du son émis à ce niveau.  
\item L'intensité du son est modulé par l'intensité du flux d'air sortant du poumon situé plus bas. 
\item Une première caisse de résonance est localisée dans la bouche et sa forme géométrique est modulée notamment par 
la position de la langue et l'ouverture de la bouche. Cette forme géométrique entraîne la formation de vibrations. 
\item Une deuxième caisse de résonance est localisée dans un espace libre au dessus de la bouche au niveau du nez, espace 
appelé cavité nasale. Cette deuxième caisse de résonance entraîne la formation d'un son avec une certaine fréquence. 
\end{itemize}

Ainsi l'anatomie du corps humain permet de modifier l'intensité d'un son et la différence entre deux fréquences 
de résonance. 




%\begin{figure}[htbp]
%\begin{center}
%\begin{tabular}{c}
%\includegraphics[width=0.5\linewidth]{coupe_schematique_parole.png}
%\end{tabular}
%\end{center}
%\caption{Diagramme représentant les organes de la parole, extraite de~\cite{KhederW17} }
%\label{fig:coupe_schematique_parole}
%\end{figure}
%\section{Estimation spectrale}

\subsection{Spectrogramme et notion de description temps-fréquence}
\label{ssec:spectrogramme}

\begin{figure}[htbp]
\begin{center}
\begin{tabular}{c}
\includegraphics[width=0.5\linewidth]{spectrogramme.png}
\end{tabular}
\end{center}
\caption{spectrogramme d'un signal sonore.}
\label{fig:spectrogramme}
\end{figure}

La figure~\ref{fig:spectrogramme} est un exemple de spectrogramme, c'est une visualisation d'un son, ici 
constitué d'une partie parlée à gauche, un silence au milieu, et de nouveau une partie parlée à droite. 
L'axe horizontal est le temps en seconde. L'axe vertical est la fréquence en Hertz. 
Il s'agit d'une représentation temps-fréquence, ce qui peut paraître contradictoire dans le cadre de ce cours. 
En effet une description temporelle d'un signal ne dépend pas de la fréquence et une description fréquentielle d'un signal 
au moyen de son spectre ne dépend pas du temps. En fait la position latérale d'un point détermine une portion du signal sur un intervalle
de temps. Tous les points d'une même verticale concernent la même portion du signal. 
Cette portion de signal est transformée en un spectre qui permet d'indiquer comment l'énergie de cette portion du signal est décomposée en 
une somme  de signaux sinusoïdaux. Chaque point de cette verticale représente une de ces sinusoïdes, c'est la hauteur de ce point qui en déterminant 
une fréquence détermine aussi la sinusoïde. Et un point 
 est d'autant plus sombre ou rouge que l'amplitude du signal sinusoïdal est plus importante. Sur ce spectrogramme, on observe une alternance de 
bandes sombres/rouges horizontales qui sont à la fois régulièrement espacées et avec des intensités qui diminues lorsque la fréquence augmente. 
Ce phénomène est lié au caisses de résonance qui produisent des sons avec une fréquence de base et des harmoniques qui sont des multiples 
de la fréquence de base.

Historiquement la recherche en reconnaissance de la parole s'est d'abord donnée comme guide le fait 
de modéliser les organes qui produisent ou reconnaissent la parole. En pratique la complexité numérique 
et la difficulté à modéliser limitaient la précision des modèles obtenues et par suite la performance. 
Il semble aujourd'hui admis que les techniques de machine learning permettent plus facilement d'obtenir 
des techniques efficaces. Il reste cependant de toutes ces études l'importance apportée à l'utilisation 
d'un certain type de descripteurs et par exemple l'importance d'estimer la fréquence fondamentale. 
L'utilité de s'intéresser à la fréquence fondamentale pour reconnaître une voyelle est 
expliquée en détail dans~\cite{Meunier07}.











\section{Estimation spectrale}
\label{sec:estimation_spectrale}

L'objet de cette partie est de définir 
une application transformant les valeurs sur une trame~$k$ en une valeur donnée, appelée valeur du 
descripteur. 
La section~\ref{ssec:estimation_frequence_fondamentale} présente des techniques permettant 
d'estimer la fréquence fondamentale. 
La section~\ref{sec:descripteur_spectre} presente d'autres techniques permettant d'estimer 
d'autre caractéristiques du spectre, par exemple sa largeur. 

\subsection{Estimation de la fréquence fondamentale}
\label{ssec:estimation_frequence_fondamentale}

Dans cette partie, les deux indicateurs présentés ont pour objectif d'estimer la fréquence fondamentale.~\footnote{Pour un son musical assez simple, cette 
fréquence correspond au {\em pitch} défini section~C.3, p.~215-217 de~\cite{Rocchesso03}.} 

Une autre technique existe pour mesurer la fréquence fondamentale en s'appuyant sur l'autocorrélation.~\footnote{Cette 
technique est brièvement présentée p.~45-46 dans~\cite{Camastra07}.}


\subsubsection{Zero Crossing Rate}

\begin{figure}[htbp]
\begin{center}
\begin{tabular}{c}
\includegraphics[width=0.5\linewidth]{zero_crossing_rate.png}
\end{tabular}
\end{center}
\caption{Graphe illustrant le fonctionnement de l'indicateur $\mb{ZCR}$. }
\label{fig:zero_crossing_rate}
\end{figure}


La figure~\ref{fig:zero_crossing_rate} montre l'évolution de deux signaux en fonction du temps. 
Le premier en trait plus foncé/bleu est la superposition de 2 sinusoïdes. Le deuxième 
 en trait plus clair/vert est une sinusoïde.  Le descripteur~\footnote{Cette technique 
appelée {\em zero crossing rate} est évoquée dans la section~2.4 p.~12 de~\cite{Peeters04}, 
et définie dans~\cite{Camastra07} p.~43-44.} 
$\mb{ZCR}$ détermine le nombre de fois où la courbe traverse l'axe horizontal par une unité de temps. 
Ici il y a deux traversées toutes les secondes. 

Le nombre de passage par zéro n'est en fait pas une notion qui se prête à une formalisation 
utilisant le temps continu. 
Le nombre moyen de passages par zéro pour la trame $k$ est donnée par
\beqn
\label{eq:ZCR}
\boxed{
Z_k=\frac{1}{N_K}{\sum_{n=0}^{N_K-1} \1\left (\signe(x_k[n+1])\neq \signe(x_k[n])\right)}
}
\eeqn
Le fait de normaliser par la longueur de la trame ($N_K$) fait que $Z_k$ n'est pas augmenté lorsque 
les trames sont plus longues. 

Ce nombre moyen de passage par zéro est utilisé pour estimer la fréquence fondamentale, c'est la fréquence 
de la sinusoïde qui aurait ce nombre moyen de passages par zéros. 
\beqn
\label{eq:f_ZCR}
\boxed{
f^{(\sm{ZCR})}_k=\frac{Z_k f_e}{2}
}
\eeqn
En effet, pour une sinusoïde de fréquence $f^{(\sm{ZCR})}_k$, sa période est $T=\frac{1}{f^{(\sm{ZCR})}_k}$ 
et le nombre moyen de passages par zéros est $2$ divisé par le nombre de points sur une période $Tf_e$, 
aussi 
\beqns
f^{(\sm{ZCR})}_k=\frac{1}{T}=\left(\frac{2}{T f_e}\right ) \frac{f_e}{2}=\frac{Z_k f_e}{2}
\eeqns


\subsubsection{Fréquence moyenne du spectre}

\begin{figure}[htbp]
\begin{center}
\begin{tabular}{c}
\includegraphics[width=0.5\linewidth]{illustration_frequence_moyenne.png}
\end{tabular}
\end{center}
\caption{Illustration du calcul de la fréquence moyenne et 
de sa signification comme séparant en deux parties 
égales la surface sous la courbe.}
\label{fig:illustration_frequence_moyenne}
\end{figure}

La notion de temps-fréquence évoquée lors de la description du spectrogramme dans la section~\ref{ssec:spectrogramme}
permet de définir une densité spectrale d'énergie qui dépend du temps. Ici cela se fait en 
appliquant une fenêtre rectangulaire avec l'intervalle $\left [t-\frac{T}{2},t-\frac{T}{2}\right]$
sur le signal $x(t)$. 
\beqn
\label{eq:DSP_t}
\boxed{
\left|\ww{X}_t(f)\right|^2=\left |\mb{TF}\left [x(t)\1_{\left [t-\frac{T}{2},t-\frac{T}{2}\right]}(t)\right](f)
\right|^2
}
\eeqn
Ensuite cette densité spectrale dépendant du temps et de la fréquence est une utilisée 
comme pondération dans $\mu(t)$ qui est appelée la fréquence moyenne (son unité est bien le Hertz). 
\beqn\label{eq:mu_t}
\boxed{
\mu(t)=\frac{{\int\limits_0^{+\infty} f\left |\ww{X}(f)\right |^2\,df}}
{{\int\limits_0^{+\infty} \left |\ww{X}(f)\right |^2\,df}}
}
\eeqn
On peut voir ce calcul de moyenne comme assez similaire au calcul de l'espérance 
d'une variable aléatoire à partir de la densité de probabilité d'une variable aléatoire~: 
$E[T]={\int_\bb{R} tf_T(t)\,dt}$ où ici $f$ jouerait le rôle de $t$ et 
$\frac{\left |\ww{X}(f)\right |^2}{{\int\limits_0^{+\infty} \left |\ww{X}(f)\right |^2\,df}}$
jouerait le rôle de $f_T(t)$.

La figure~\ref{fig:illustration_frequence_moyenne} donne une justification 
de la définition de $\mu(t)$ dans l'équation~(\ref{eq:mu_t}).
La courbe en noir notée $P(f)$,
correspondant en réalité à $|\ww{X}_t(f)|^2$, 
est la densité spectrale d'énergie d'une portion du signal 
$x(t)\1_{[t-\frac{T}{2},t+\frac{T}{2}]}(t)$. 
Le trait semi-pointillé vertical est positionné 
%à la fréquence $\mu(t)$. On considère maintenant 
%la surface sous la courbe à gauche de $\mu(t)$, 
%elle est égale au terme de gauche de la deuxième 
%égalité
%\beqns
%{\int_{0}^{\mu(t)}(\mu(t)-f)P(f)\,df}
%\eeqns
%La surface sous la courbe à droite de $\mu(t)$ 
%est égale au terme de droite de la deuxième égalité
%\beqns
%{\int_{\mu(t)}^{+\infty}(f-\mu(t))P(f)\,df}
%\eeqns
%Ainsi qu'il est indiqué à gauche de la figure, 
%l'égalité de ces deux dernières équations conduit 
%à la définition de $\mu(t)$ donnée dans l'équation~(\ref{eq:mu_t}). 
%Ainsi on peut dire que cette moyenne temporelle est 
%la fréquence qui divise en deux parties égales la surface 
%sous la courbe de la densité spectrale d'énergie de la portion 
%de signal. 
%de signal. 

Cette notion est adaptée aux signaux à temps discret en 
considérant la portion du signal~\footnote{Cette application 
de la transformée de Fourier discrète sur 
le signal découpé peut être vu comme 
l'utilisation d'une transformée 
de Fourier à court terme, p.~99 de~\cite{Rocchesso03}.} 
 sur une trame $x_k[n]$ et en lui calculant la transformée de Fourier discrète considérant 
que la longueur de la trame est suffisante pour que cette transformée de Fourier discrète
soit une bonne approximation de la transformée de Fourier de cette portion de signal. 
On utilise ici un indice $l$ pour les fréquences et on ne considère que la première 
moitié des $N_K$ indices parce que la deuxième moitié des indices correspond aux fréquences 
négatives qui n'est pas prise en compte dans l'équation~(\ref{eq:mu_t}).
Cette première moitié des indices est notée 
\beqn\label{eq:N_K_2}
\boxed{
N_K^{\deux}=\left \lfloor \frac{N_K}{2} \right\rfloor
}
\eeqn
où $\lfloor\ldots \rfloor$ désigne l'arrondi par en dessous. 
Les $N_K^{\deux}$ premières fréquences sont 
$\left [0\ldots \frac{N_K^{\deux}f_e}{N_K}\right]$. 
Ces différentes valeurs sont écrites au moyen d'un nouvel indice $l$ dont dépend la fréquence. 
\beqn\label{eq:f_l}
\boxed{
f_l=\frac{lf_e}{N_K}\mbox{ pour }l\in \{0\ldots N_K^{\deux}
}
\eeqn
La pondération utilisée est la densité spectrale de puissance de la trame $k$.
\beqn
\boxed{
\left |\ww{X}_k[l]\right |^2= \left |
\sm{TFD}\left [x_k[n]\right][l]\right |^2
}
\eeqn
Un estimateur de la fréquence moyenne du spectre $\mu_k$~\footnote{Cet estimateur 
est défini dans la section~6.1.1 p.~13 de~\cite{Peeters04}.}
 est  
\beqn\label{eq:mu_sp}
\boxed{
\mu_k=\frac{{\sum_{l=0}^{N_K^{\deux}}\,\,f_l\,\,\left |\widehat{X}_k[l]\right |^2}}
{{\sum_{l'=0}^{N_K^{\deux}}\left |\widehat{X}_k[l']\right |^2}}
}
\eeqn 
% où $\widehat{X}_k[l]$ est la transformée de Fourier discrète à $k$ fixé de $x_k[n]$ définie par 
% $\widehat{X}_k[l]=\frac{1}{N_K}{\sum_{n=0}^{N_K-1}x_k[n]e^{-j2\pi\frac{ln}{N_K}}}$~;
% et ${\lfloor \frac{N_K}{2}\rfloor}$ signifie le plus grand entier inférieur à $N_K/2$. 
Un indice $l'$ est utilisé parce qu'il n'y a en fait aucun lien entre le compteur utilisé dans la sommation au niveau du numérateur et
le compteur utilisé dans la sommation au niveau du dénominateur. 

\subsection{Autre descripteurs du spectre}
\label{sec:descripteur_spectre}

\subsubsection{Largeur du spectre}

\begin{figure}[htbp]
\begin{center}
\begin{tabular}{c}
\includegraphics[width=0.5\linewidth]{illustration_largeur_spectre.png}
\end{tabular}
\end{center}
\caption{Illustration graphique sur un exemple du sens donné à la notion d'estimation de la largeur d'un spectre.}
\label{fig:illustration_largeur_spectre}
\end{figure}


La largeur du spectre est estimée connaissant $\mu(t)$ avec 
\beqn
\label{eq:largeur_spectre}
\boxed{
\sigma(t)=\frac{\sqrt{{\int\limits_{\bb{R}_+}\left(f-\mu(t)\right)^2\left |\ww{X}_t(f)\right|^2\,df}}}{\sqrt{{\int\limits_{\bb{R}_+}\left |\ww{X}_t(f)\right|^2\,df}}}
}
\eeqn

La figure~\ref{fig:illustration_largeur_spectre} représente l'exemple d'un spectre d'une porte. 
La fréquence est en abscisse. Ce spectre a pour équation un sinus cardinal avec un demi-lobe principal de $3000$Hz. 
Cette figure illustre deux descripteurs $\mu$ et $\sigma$. $\mu$ est la fréquence moyenne et $\sigma$ est l'écart-type. 
Les deux sont calculés comme si les spectres étaient nuls pour les fréquences négatives (s'ils étaient calculés sur les 
vrais spectres, comme leur module est symétrique, la moyenne serait nulle. 
$\mu$ est indiqué par un trait vertical en pointillé. $\sigma$ est représenté par deux traits verticaux autour de celui associé à $\mu$. 
Ces deux traits verticaux indiquent que si le spectre était une gaussienne (courbe en traits pointillés), $66\%$ de sa surface serait incluse dans ces deux traits
verticaux en pointillés. Ce graphe n'est en fait pas tout à fait exact, d'une part la proportion de $66\%$ et l'axe de symétrie au centre de la gaussienne n'est 
ici pas valable puisqu'on ne considère que les fréquences positives, d'autre part la moyenne et le calcul de la largeur se fait en considérant 
la densité spectrale et non le module de la transformée de Fourier et cette densité spectrale n'est donc pas exactement un sinus cardinal.

De même pour le calcul de la moyenne temporelle, l'équation~(\ref{eq:largeur_spectre}) décrivant l'estimation de la largeur du spectre peut 
se voir comme l'estimation de l'écart-type d'une variable aléatoire positive de densité de probabilité $f_T(t)$
\beqns
\sqrt{\mb{var}(T)}=\sqrt{E[(T-E[T])^2]}=\sqrt{{\int\limits_{\bb{R}_+}(t-E[T])^2f_T(t)\,dt}}
\eeqns
où ce qui remplace ici la variable $t$ est $f$ et la densité de probabilité $f_T(t)$ est 
\beqns
\frac{1}{{\int\limits_{\bb{R}_+}\left |\ww{X}_t(f)\right|^2\,df}}\, \left |\ww{X}_t(f)\right|^2
\eeqns



En utilisant les mêmes notations que pour (\ref{eq:mu_sp}), une estimation de la largeur du spectre~\footnote{Cet estimateur est défini dans la section~6.1.2 p.~13 de~\cite{Peeters04}.} est
\beqn
\label{eq:sigma_sp}
\boxed{
\sigma_k=\sqrt{\frac{{\sum_{l=0}^{N_K^\deux}\,\,\left (f_l-\mu_k\right )^2\,\,
\left |\ww{X}_k[l]\right |^2}}{{\sum_{l'=0}^{N_K^\deux}\left |\widehat{X}_k[l']\right |^2}}}
}
\eeqn

%En reprenant les notations utilisée pour (\ref{eq:mu_pl}), cet estimateur de la largeur du spectre peut s'écrire ainsi. 
%\beqn
%\sigma=\sqrt{
%{\sum_{l=0}^{l_{\max{}}}(f_l-\mu)^2 \frac{p_l}{{\sum_{l'=0}^{l_{\max{}}} p_{l'}}}}
%}
%\eeqn
%Ainsi $\sigma$ peut s'interpréter comme la racine carré de la variance d'une variable aléatoire discrète $F$ dont les probabilités sont 
%données par $\frac{p_l}{{\sum_{l'=0}^{l_{\max{}}} p_{l'}}}$. 


\subsubsection{Coefficient d'asymétrie du spectre}

Un estimateur du coefficient d'asymétrie ({\em skewness})~\footnote{Cet estimateur est défini dans la section~6.1.3 p.~13 de~\cite{Peeters04}.} est donné 
par 
\beqns
\gamma_1(t)=\frac{1}{\sigma^3(t)}\frac{{\int\limits_{\bb{R}_+}\left(f-\mu(t)\right)^3\left |\ww{X}_t(f)\right|^2\,df}}{{\int\limits_{\bb{R}_+}\left |\ww{X}_t(f)\right|^2\,df}}
\eeqns
qui devient avec les notations utilisées dans (\ref{eq:sigma_sp}).
\beqn
\gamma_1[k]=\frac{1}{\sigma_k^3}{\frac{{\sum_{l=0}^{N_K^\deux}\,\,\left (f_l-\mu_k\right )^3\,\,
\left |\ww{X}_k[l]\right |^2}}{{\sum_{l'=0}^{N_K^\deux}\left |\widehat{X}_k[l']\right |^2}}}
\eeqn
De même, un estimateur du coefficient d'aplatissement ({\em kurtosis})~\footnote{Cet estimateur est défini dans la section~6.1.4 p.~14 de~\cite{Peeters04}.} est donné par
\beqns
\gamma_1(t)=\frac{1}{\sigma^4(t)}\frac{{\int\limits_{\bb{R}_+}\left(f-\mu(t)\right)^4\left |\ww{X}_t(f)\right|^2\,df}}{{\int\limits_{\bb{R}_+}\left |\ww{X}_t(f)\right|^2\,df}}
\eeqns
qui devient avec les notations utilisées dans (\ref{eq:sigma_sp}).
\beqn
\gamma_2[k]=\frac{1}{\sigma_k^4}{\frac{{\sum_{l=0}^{N_K^\deux}\,\,\left (f_l-\mu_k\right )^4\,
\,\left |\widehat{X}_k[l]\right |^2}}{{\sum_{l'=0}^{N_K^\deux}\left |\widehat{X}_k[l']\right |^2}}}
\eeqn


\section{Utilisation de bancs de filtres}
\label{sec:banc_filtres}


\begin{figure}[htbp]
\begin{center}
\begin{tabular}{c}
\includegraphics[width=0.5\linewidth]{banc_de_filtre.png}
\end{tabular}
\end{center}
\caption{Schéma d'un banc de filtres }
\label{fig:banc_de_filtre}
\end{figure}

On introduit de nouvelles notations pour décrire un banc de filtres. 
\begin{itemize}
\item $l$ est un indice qui compte les raies du spectre des trames. 
\item $f_l$ est la valeur de la fréquence associée à la raie~$l$. 
\item $m$ est un indice qui numérote les filtres utilisés dans le banc de filtres. 
\item $\ww{H}_m(f)$ est la réponse fréquentielle du filtre numéro $m$. 
\end{itemize}


La figure~\ref{fig:banc_de_filtre} schématise un banc de filtres. Le bas de la figure montre les réponses fréquentielles de $4$~filtres notés~$\ww{H}_1(f)$, 
$\ww{H}_2(f)$, $\ww{H}_3(f)$ et $\ww{H}_4(f)$. Le filtre~$\ww{H}_1$ est un passe-bas. Les filtres $\ww{H}_2(f)$ et~$\ww{H}_3(f)$ sont des filtres passe-bande.
Le filtre $\ww{H}_4(f)$ est un filtre passe-haut. Une particularité de ces filtres est que la somme de leur réponses fréquentielles est un filtre passe-tout 
généralement un simple filtre à retard dont le module de la réponse fréquentielle vaut~$1$. 

Dans la partie supérieure de la figure~\ref{fig:banc_de_filtre}, on retrouve à gauche les~$4$ filtres $\ww{H}_1(f)$, 
$\ww{H}_2(f)$, $\ww{H}_3(f)$ et $\ww{H}_4(f)$. Ces filtres reçoivent tous en entrée le signal $x(t)$, celui-ci est visualisé en haut à droite en noir. 
Le signal en bleu représenté juste en dessous est $y_1(t)$, c'est la sortie du filtre de réponse fréquentielle $\ww{H}_1(f)$. On observe que ce signal 
présente des variations de moindre amplitudes, c'est la conséquence de ce que $\ww{H}_1(f)$ est un passe-bas. 
Les signaux représentés en dessous en vert, rouge et cyan, sont notés $y_2(t), y_3(t), y_4(t)$. Ce sont respectivement les sorties des filtres
$\ww{H}_2(f)$, $\ww{H}_3(f)$ et $\ww{H}_4(f)$. On y retrouve des variations parfois significativement plus importantes. 
La décomposition du signal $x(t)$ en $4$ signaux $y_1(t), y_2(t), y_3(t), y_4(t)$ est appelé {\em analyse}, terme indiqué en bas à gauche de la figure~\ref{fig:banc_de_filtre}. Ces signaux, $y_1(t), y_2(t), y_3(t), y_4(t)$ sont ensuite additionnés pour former le signal visualisé en bas à droite en violet et noté 
$y_1(t)+y_2(t)+y_3(t)+y_4(t)$. Tel qu'on peut l'observer, ce signal est identique à $x(t)$. En réalité, ce dernier signal est généralement retardé par rapport 
à $x(t)$. Il est en effet impossible de réaliser une décomposition en banc de filtres avec des filtres causaux sans introduire un retard. 
La formation d'une reconstruction retardée de $x(t)$ à partir des signaux $y_1(t), y_2(t), y_3(t), y_4(t)$ s'appelle {\em synthèse}, ce qui est indiqué en 
bas du deuxième bloc. 

En regardant plus attentivement le bas de la figure~\ref{fig:banc_de_filtre}, on peut observer que les supports~\footnote{Par support, on entend ici l'intervalle sur lequel une fonction ici la réponse fréquentielle est non nulle.} des réponses 
fréquentielles des différents filtres ne sont pas disjoints, on dit que ces filtres se chevauchent. En fait l'allure même du signal $y_1(t)$ avec ces variations atténuées mais existantes laisse penser qu'il y a probablement un chevauchement assez important. Et en effet la notion de banc de filtre 
n'est pas du tout contradictoire avec un chevauchement même assez important. 
Pour la suite de ce document et pour plus de simplicité, on va considérer des bancs de filtres sans chevauchement où les réponses
fréquentielles sont en fait des portes définies par $\1_{[f_1,f_2]}(f)$. 

On dit qu'un banc de filtres suit une échelle linéaire lorsque les intervalles associés aux différentes portes caractérisant les réponses fréquentielles 
des filtres $\ww{H}_m(f)$ sont de longueur identiques. 
\beqn\boxed{
[f_{\min},f_{\max}]=\bigcup_{m}[f_m,f_{m+1}]\quad\mbox{où}\quad 
\left \{ \begin{array}{l}
f_{\min}=f_1,\,\,f_{\max}=f_{M+1}\\[0.3cm]
f_m=f_{\min}+(m-1)\frac{f_{\max}-f_{\min}}{M}\\[0.3cm]
\ww{H}_m(f)=\1_{[f_m,f_{m+1}]}(f)
\end{array}
\right. 
}
\eeqn

\begin{figure}
\begin{center}
\begin{tabular}{cc}
\includegraphics[width=0.5\linewidth]{fig9a.png}&
 \includegraphics[width=0.5\linewidth]{fig9b.png}
\end{tabular}
\end{center}
\caption{\`A gauche~: les courbes $\widehat{H}_m(f)$ en fonction de $f$ pour $m\in\{1,\ldots,8\}$ sont superposées
sur un même graphe.
 \`A droite~: ces courbes ont chacune leur abscisse.}
\label{fig9}
\end{figure}

La sensibilité de l'oreille humaine vis-à-vis de la décomposition fréquentielle d'un son et la façon dont les sons sont produits 
par les organes humains amènent à choisir pour les intervalles caractérisant les filtres $\ww{H}_m(f)$ une échelle logarithmique. 
Ce terme d'échelle logarithmique signifie que les intervalles sont de longueurs {\em croissantes} et que les bornes des ces intervalles 
suivent une loi {\em géométriques}. 
\beqn\boxed{
[f_{\min},f_{\max}]=\bigcup_{m}[f_m,f_{m+1}]\quad\mbox{où}\quad 
\left \{ \begin{array}{l}
f_{\min}=f_1,\,\,f_{\max}=f_{M+1}\\[0.3cm]
f_m=f_{\min}\left (\frac{f_{\max}}{f_{\min}}\right)^{\frac{m-1}{M}}\\[0.3cm]
%r=e^{\frac{\ln(f_{\max})-\ln(f_{\min})}{M}}=\left (\frac{f_{\max}}{f_{\min}}\right)^{\frac{1}{M}}\\[0.3cm]
\ww{H}_m(f)=\1_{[f_m,f_{m+1}]}(f)
\end{array}
\right. 
}
\eeqn

En pratique pour un banc de filtre suivant une échelle linéaire, on peut choisir $f_{\min}=0$ et $f_{\max}=\frac{f_e}{2}$, 
et pour une échelle logarithmique, il faut que $f_{\min}>0$, on peut choisir $f_{\min}=\frac{1}{T_K}$ et $f_{\max}=\frac{f_e}{2}$,
$T$ étant la durée de la trame.  

La figure~\ref{fig9} montre les réponses fréquentielles de huit filtres $\ww{H}_m$ qui suivent une échelle logarithmique, à gauche 
en les superposant sur un même graphe 2D et à droite en mettant chaque courbe le long d'un axe différent. 

\begin{figure}
\begin{center}
\begin{tabular}{cc}
\includegraphics[width=0.5\linewidth]{fig10a.png} &\includegraphics[width=0.5\linewidth]{fig10b.png}
\end{tabular}
\end{center}
\caption{\`A gauche~: superposition de l'évolution des descripteurs en fonction du temps. Chaque courbe
est associée à un filtre en particulier dont la légende indique la fréquence centrale associée à ce filtre.
\`A droite~: représentation séparée de l'évolution de chaque descripteur en fonction du temps.Dans les 
deux graphes, l'échelle en temps indique les instants associés aux milieux de chaque trame.}
\label{fig10}
\end{figure}

La figure~\ref{fig10} représente un exemple de représentation de ce descripteur temps-fréquence, 
il s'agit à gauche et à droite des courbes qui dans la figure~\ref{fig9} sont appelées $y_1(t), y_2(t), y_3(t), 
y_4(t)$. La différence est qu'ici il y en a $5$ et que les filtres utilisés ici ne se chevauchent pas. 
On observe des variations d'amplitudes plus faibles pour les quatre  premières 
par rapport à la dernière associées au fréquences plus élevées. 
Cependant il est significatif que la courbe bleue foncée, associée au filtre passe-bas et située au milieu sur le graphe de gauche et en 
haut à gauche sur le graphe de droite, a des variations qui sont d'une amplitude assez significatives, là 
on aurait pu s'attendre à des variations moins importantes. Cela traduit le fait que le signal 
sonore étudié présente des variations temporelles importantes d'une trame à une autre. 

Ces bancs de filtres servent à définir des descripteurs, un par filtre du banc de filtre.
De multiples descripteurs sont proposés dans la littérature scientifique. 
On aurait pu s'attendre à définir un descripteur comme la puissance sur une portion du signal en 
sortie du filtre $\ww{H}_m(f)$
autour de l'instant $t$.
\beqn\label{eq:desc_bf}
\boxed{
D_m(t)=\frac{1}{T}{\int_{-\frac{T}{2}}^{\frac{T}{2}} |h_m(\tau)\ast x_t(\tau)|^2\,d\tau}
\quad \mbox{ où }\quad \left \{ \begin{array}{l}
h_m(\tau)\mbox{ est la réponse impulsionnelle du filtre }\ww{H}_m(f)\\[0.3cm]
x_t(\tau)=x(\tau+t)\1_{\left [-\frac{T}{2},\frac{T}{2}\right]}(\tau)
\end{array}
\right . 
}
\eeqn

Mais comme la perception de l'intensité sonore est mieux corrélée à une intensité mesurée en décibel et donc 
suivant une échelle logarithmique vis-à-vis de la puissance, il convient d'ajouter un logarithme dans l'équation~(\ref{eq:desc_bf}).
La littérature scientifique a fait le choix d'utiliser un autre descripteur dont une version en temps continu serait 
\beqn
\sm{D\_LOG}_m(t)=\frac{1}{f_{m+1}-f_m}\,{\int_{f_m}^{f_{m+1}} 10\log_{10} \left |\ww{H}_m(f) \ww{X}_t(f)\right|^2\,df}
\eeqn
Et en pratique, le descripteur utilisé, dépend de deux paramètres, $m$ pour le filtre et par 
suite la fréquence associée à ce filtre, et $k$ pour la trame considérée. 

Le descripteur utilisé dans les travaux pratiques 
a pour nom {\tt LOG\_MAG\_FB\_LOG}~\footnote{La signification du nom se retrouve en lisant 
l'expression de droite à gauche. {\tt LOG} en dernier signifie qu'on considère une échelle logarithme, puis 
que cette échelle permet de définir un banc de filtre ({\em filter bank}), qu'on calcule ensuite le module ({\em magnitude}) 
et qu'avant de considérer la moyenne on considère le logarithme des modules.}

En pratique, le descripteur est ainsi défini.
\beqn
\boxed{
\sm{LOG\_MAG\_FB\_LOG}(m,k)=
\frac{1}{\left |\bb{L}_m\right |}
{\sum_{l\in \bb{L}_m} 10\log_{10}\left |\widehat{H}_{m,l}\widehat{X}_{k,l}\right|^2}
}
\eeqn
où $\bb{L}_m$ désigne les indices $l$ pour lesquels $\widehat{H}_{m}\left(\frac{lf_e}{N_K}\right)$ est non-nul, 
ce sont a priori les indices $l$ pour lesquels la fréquence $\frac{lf_e}{N_K}$ sont contenus dans 
$\left [f_m,f_{m+1}\right]$. 
$|\bb{L}_m|$ désigne le nombre d'indices $l$ contenus dans $\bb{L}_m$. 

Remarquons que le fait de modifier un descripteur en le multipliant par une certaine constante ou 
en lui ajoutant une constante n'a aucune incidence sur la classification qui en résulte. 


%\section{Conclusion}

D'autres suggestions de descripteurs pour la reconnaissance de la parole se trouvent dans~\cite{Rabiner93}.



